Software Solutions for Newcomers' Onboarding in Software Projects: A Systematic Literature Review

[Context] Newcomers joining an unfamiliar software project face numerous barriers; therefore, effective onboarding is essential to help them engage with the team and develop the behaviors, attitudes, and skills needed to excel in their roles. However, onboarding can be a lengthy, costly, and error-prone process. Software solutions can help mitigate these barriers and streamline the process without overloading senior members. [Objective] This study aims to identify the state-of-the-art software solutions for onboarding newcomers. [Method] We conducted a systematic literature review (SLR) to answer six research questions. [Results] We analyzed 32 studies about software solutions for onboarding newcomers and yielded several key findings: (1) a range of strategies exists, with recommendation systems being the most prevalent; (2) most solutions are web-based; (3) solutions target a variety of onboarding aspects, with a focus on process; (4) many onboarding barriers remain unaddressed by existing solutions; (5) laboratory experiments are the most commonly used method for evaluating these solutions; and (6) diversity and inclusion aspects primarily address experience level. [Conclusion] We shed light on current technological support and identify research opportunities to develop more inclusive software solutions for onboarding. These insights may also guide practitioners in refining existing platforms and onboarding programs to promote smoother integration of newcomers into software projects.

==> Conduction/conduction-Example.tex <==
%%%SLR results
%This document is based on ``Kitchenham, B. SEGRESS: Software Engineering Guidelines for REporting Secondary Studies. IEEE Transactions on Software Engineering, Vol. 49, NO. 3, March 2023.''

%######################################
An SLR begins with a planning phase, which includes formulating research questions (RQs) and defining inclusion and exclusion criteria, followed by searching and selecting relevant studies. 

This SLR aims to identify studies that have proposed software solutions to enhance the onboarding processes for newcomers in software projects. Based on these goals, the questions we intend to clarify and the rationale for considering them are presented in Table \ref{table:conductionRQ}.

\begin{table*}[ht!]
	\caption{Research questions and their rationales} \label{table:conductionRQ}
	\vskip 0.3cm
	\centering
	\begin{tabular}{p{0.7cm}||p{7cm}|p{9cm}}
		\hline
		\textbf{N$^{o}$} & \textbf{Research question} & \textbf{Rationale} \\ \hline \hline

		\textbf{RQ1} & \textit{What software solutions are proposed in the literature to improve the onboarding of newcomers to software projects?} & We intend to highlight the existing software solutions for onboarding that can be explored to improve newcomers' onboarding research practices. \\ 
		\hline

		\textbf{RQ2} & \textit{How do the software solutions were implemented?} & We intend to provide implementation details of how the software solutions were implemented to guide new solutions that want to create or improve the existing software solutions. \\ 
		\hline	

            \textbf{RQ3} & \textit{How do the software solutions improve newcomers' onboarding?} & We intend to deliver empirical evidence of the outcomes achieved by the software solutions to highlight the benefits of using each software solution.  \\ 
		\hline

            \textbf{RQ4} & \textit{What research strategies were employed to assess the software solutions?} & We intend to understand the research strategies used to evaluate the proposed software solutions to highlight the context in which they were implemented. \\ 
		\hline

            \textbf{RQ5} & \textit{How do the software solutions mitigate newcomers' barriers to joining software projects?} & We intend to comprehend which of the proposed software solutions mitigated contribution barriers to explore possible research gaps. \\ 
		\hline

            \textbf{RQ6} & \textit{How do the software solutions prioritize increasing diversity and inclusion among newcomers?} & We intend to investigate which diversity and inclusion aspects are explored to include more diversity in OSS projects and make software solutions for onboarding more inclusive. \\ 
		\hline
	\end{tabular}
\end{table*}

The strategy used by us to identify and select relevant studies is described as follows.

%-----------------------------
\vspace{0.1cm}
\subsection{Search strategy and Selection process} 


We systematically searched for relevant studies, as illustrated in Figure \ref{fig:searchSelection}. The search process included eight stages, applied sequentially, as follows.

\begin{enumerate}
    \item \textbf{Stage 1 --} The first researcher (R1) used a set of keywords and their respective synonyms to construct our search string (presented in Table \ref{tab:conductionString}), as detailed in Table~\ref{tab:searchterms}. The selection of these synonyms was carried out with the assistance of domain experts, and we also drew upon relevant SLR primary studies, which served as control references for our study~\cite{steinmacher2015systematic, kaur2022understanding}, to enrich our collection of synonyms further. Moreover, R1 applied the search string in the most commonly used publications databases in Computer Science, including IEEE xplore~\footnote{http://ieeexplore.ieee.org}, ACM digital library~\footnote{http://portal.acm.org}, Scopus~\footnote{http://www.scopus.com}, Springer link~\footnote{https://link.springer.com/}, and Web of science~\footnote{https://www.webofscience.com/wos/woscc/basic-search}. Our search across the five selected digital libraries yielded 9,732 candidate studies. Subsequently, we removed 2,243 duplicate candidate studies, resulting in an initial set of 7,489 unique candidate studies to commence the selection process.

    \item \textbf{Stage 2 --} R1 reviewed the candidate studies' titles, abstracts, and keywords to assess their adherence to the inclusion and exclusion criteria. At this stage, 1049 studies were included. 

    \item \textbf{Stage 3 --} R1 evaluated the introduction section of the studies selected in the previous stage to examine their motivation and contributions, and 314 candidate studies were included.
     
    \item \textbf{Stage 4 --} At this stage, R1 applied the selection criteria by reading each paper's conclusion section, and 43 candidate studies were included. 

    \item \textbf{Stage 5 --} At this stage, another researcher (R2) applied the selection criteria in the previously selected candidate studies. The R1 and R2 jointly conducted a consensus decision-making meeting. They reached 88\% of agreement, resulting in 25 studies.
    
    \item \textbf{Stage 6 --} This study selection phase comprised two stages: initial and final selection. During the initial selection stage, screening of titles and abstracts for the candidate studies was performed by R1 against the inclusion/exclusion criteria, resulting in seven (7) studies. The final selection involved examining full papers to make the decision. After performing this stage, 5 (five) studies were included.

    \item \textbf{Stage 7 --} The main weakness of this review is that the databases should not return all studies related to our investigated topic. We included backward and forward snowballing to mitigate the risk of missing studies. Thus, the overall risk of bias due to missing data should be considered Low. R1 performed three rounds of full snowballing. It identifies new studies based on the start set, followed by backward and forward snowballing. R1 conducted this complimentary search strategy according to the guidelines for snowballing proposed in~\cite{wohlin2014guidelines}. Thirty primary studies formed the start set. The backward snowballing had 1048 references, and the forward generated 1294 citations. R1 applied the selection criteria, including six (6) studies meeting the inclusion criteria. In round 2, R1 used the 6 (six) previous studies selected and applied the backward finding of 146 and 259 studies from forward. Only one (1) study was included. In round 3, R1, no studies were included. 
    
    \item \textbf{Stage 8 --} Finally, at the last stage, all researchers carefully read all 37 full-text papers and jointly conducted a consensus meeting with 100\% agreement, resulting in 32 studies. In summary, these studies developed a more general discussion on software solutions for newcomer onboarding in software projects (Table \ref{tab:includedStudies}).

    We considered the studies published until 2023. 
\end{enumerate}

\begin{table}[!ht]
\centering
\caption{Final Search String}
\label{tab:conductionString}
\begin{tabular}{l}
\hline

(``open source''  \textbf{OR}  ``open-source''  \textbf{OR}  ``free software''  \textbf{OR} \\ FOSS  \textbf{OR}  FLOSS  \textbf{OR}  OSS \textbf{OR}  ``OSS projects''  \textbf{OR}  ``open \\ source software''  \textbf{OR}  ``software project''  \textbf{OR}  ``software \\engineering''  \textbf{OR}  ``software development'') \textbf{AND} (``joining \\process''  \textbf{OR}  onboarding  \textbf{OR}  onboard  \textbf{OR}  joining  \textbf{OR}  \\engagement  \textbf{OR}  newcomer  \textbf{OR}  novice  \textbf{OR}  newbie  \textbf{OR}\\  ``new developer''  \textbf{OR}  ``early career''  \textbf{OR}  ``new member'' \\ \textbf{OR}  ``new contributor''  \textbf{OR}  beginner  \textbf{OR}  ``potential \\ participant''  \textbf{OR}  joiner  \textbf{OR}  entrance)

\\ \hline

\end{tabular}
\end{table}

\begin{table}[!ht]\scriptsize
\centering
\caption{Keyword and synonyms used to build search string terms}
\label{tab:searchterms}
\begin{tabular}{l|l}
\hline
\textbf{Keyword}  & \textbf{Synonyms}\\
\hline \hline
OSS & \begin{tabular}[c]{@{}l@{}} OSS, ``open source'', ``open-source'', ``free software'', FOSS, FLOSS, \\``OSS projects'', ``open source software''  \end{tabular} \\
\hline

SE & \begin{tabular}[c]{@{}l@{}} ``Software project'', ``software engineering'', ``software development''\end{tabular} \\
\hline

Onboard & \begin{tabular}[c]{@{}l@{}} Onboarding, onboard, joining, engagement \end{tabular} \\
\hline

Newcomers & \begin{tabular}[c]{@{}l@{}} Newcomer, contributors, novice, newbie,  ``new developer'', \\``early career'', ``new member'', ``new contributor'', ``new people'',\\ beginner, ``potential participant'', joiner, ``new committer'' \end{tabular} \\
\hline
\hline
\end{tabular}
\end{table}





\begin{figure*}[ht!]
    \centering
    \includegraphics[width=1.01\textwidth]{Conduction/images/newselectionprocessnewupdated2.pdf}
    \caption{Search and selection process}
    \label{fig:searchSelection}
\end{figure*}

For the selection criteria, we established one Inclusion Criteria (IC) and five Exclusion Criteria (EC), detailed below: 

\begin{itemize}
    \item \textbf{IC1:} -- The primary study proposes software solutions for newcomers' onboarding in software projects; 
    
    \item \textbf{EC1} -- The study does not have an abstract; 
    
    \item \textbf{EC2} -- The study is just published as an abstract; 
    
    \item \textbf{EC3} -- The study is not written in English; 
    
    \item \textbf{EC4} -- The study is an older version of another study already considered; 
    
    \item \textbf{EC5:} -- The study is not a scientific study, such as editorials, summaries of keynotes, workshops, and tutorials.
\end{itemize}



\begin{table*}[!ht]\scriptsize
\centering
\caption{List of included studies}
\label{tab:includedStudies}
\begin{tabular}{cllc}
\hline
\textbf{ID} & \textbf{Reference} & \textbf{Title} & \textbf{\begin{tabular}[c]{@{}c@{}}Public. \\year\end{tabular}}\\
\hline \hline

PS01 & \begin{tabular}[c]{@{}l@{}}\citet{PS01azanza2021onboarding}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Onboarding in Software Product Lines: Concept Maps as Welcome Guides \end{tabular} & 2021 \\ \hline

PS02 & \begin{tabular}[c]{@{}l@{}}\citet{PS02canfora2012going}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Who is Going to Mentor Newcomers in Open Source Projects? \end{tabular} & 2012 \\ \hline

PS03 & \begin{tabular}[c]{@{}l@{}}\citet{PS03cubranic2003hipikat}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Hipikat: Recommending pertinent software development artifacts \end{tabular} & 2003 \\ \hline

PS04 & \begin{tabular}[c]{@{}l@{}}\citet{PS04diniz2017using}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Using Gamification to Orient and Motivate Students to Contribute to OSSprojects \end{tabular} & 2017 \\ \hline

PS05 & \begin{tabular}[c]{@{}l@{}}\citet{PS05dominic2020conversational}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Conversational Bot for Newcomers Onboarding to Open Source Projects \end{tabular} & 2020 \\ \hline

PS06 & \begin{tabular}[c]{@{}l@{}}\citet{PS06fu2017expert}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Expert Recommendation in OSS Projects Based on Knowledge Embedding \end{tabular} & 2017 \\ \hline

PS07 & \begin{tabular}[c]{@{}l@{}}\citet{PS07guizani2022attracting}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Attracting and Retaining OSS Contributors with a Maintainer Dashboard \end{tabular} & 2022 \\ \hline

PS08 & \begin{tabular}[c]{@{}l@{}}\citet{PS08he2022gfi}\end{tabular} & \begin{tabular}[c]{@{}l@{}} GFI-bot: automated good first issue recommendation on GitHub \end{tabular} & 2022 \\ \hline

PS09 & \begin{tabular}[c]{@{}l@{}}\citet{PS09kagdi2008can}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Who can help me with this source code change? \end{tabular} & 2008 \\ \hline

PS10 & \begin{tabular}[c]{@{}l@{}}\citet{PS10medeiros2022assisting}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Assisting Mentors in Selecting Newcomers' Next Task in Software ProductLines: A Recommender System Approach \end{tabular} & 2022 \\ \hline

PS11 & \begin{tabular}[c]{@{}l@{}}\citet{PS11nagel2021ontology}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Ontology-Based Software Graphs for Supporting Code Comprehension During Onboarding \end{tabular} & 2021 \\ \hline

PS12 & \begin{tabular}[c]{@{}l@{}}\citet{PS12sarma2016training}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Training the Future Workforce through Task Curation in an OSS Ecosystem \end{tabular} & 2016 \\ \hline

PS13 & \begin{tabular}[c]{@{}l@{}}\citet{PS13serrano2022find}\end{tabular} & \begin{tabular}[c]{@{}l@{}} How to Find My Task? Chatbot to Assist Newcomers in Choosing Tasks inOSS Projects \end{tabular} & 2022 \\ \hline

PS14 & \begin{tabular}[c]{@{}l@{}}\citet{PS14stanik2018simple}\end{tabular} & \begin{tabular}[c]{@{}l@{}} A Simple NLP-Based Approach to Support Onboarding and Retention in Open Source Communities \end{tabular} & 2018 \\ \hline

PS15 & \begin{tabular}[c]{@{}l@{}}\citet{PS15steinmacher2016overcoming}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Overcoming Open Source Project Entry Barriers with a Portal for Newcomers \end{tabular} & 2016 \\ \hline

PS16 & \begin{tabular}[c]{@{}l@{}}\citet{PS16steinmacher2012recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending Mentors to Software Project Newcomers \end{tabular} & 2012 \\ \hline

PS17 & \begin{tabular}[c]{@{}l@{}}\citet{PS17toscani2018gamification}\end{tabular} & \begin{tabular}[c]{@{}l@{}} A Gamification Proposal to Support the Onboarding of Newcomers in the FLOSScoach Portal \end{tabular} & 2015 \\ \hline

PS18 & \begin{tabular}[c]{@{}l@{}}\citet{PS18wang2011bug}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Which bug should I fix: Helping new developers onboard a new project \end{tabular} & 2011 \\ \hline

PS19 & \begin{tabular}[c]{@{}l@{}}\citet{PS19xiao2022recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending Good First Issues in GitHub OSS Projects \end{tabular} & 2022 \\ \hline

PS20 & \begin{tabular}[c]{@{}l@{}}\citet{PS20yin2021automatic}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Automatic learning path recommendation for open source projects using deep learning on knowledge graphs \end{tabular} & 2021 \\ \hline

PS21 & \begin{tabular}[c]{@{}l@{}}\citet{PS21ford2022reboc}\end{tabular} & \begin{tabular}[c]{@{}l@{}} ReBOC: Recommending Bespoke Open Source Software Projects to Contributors \end{tabular} & 2022 \\ \hline

PS22 & \begin{tabular}[c]{@{}l@{}}\citet{PS22liu2018recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending GitHub Projects for Developer Onboarding \end{tabular} & 2018 \\ \hline

PS23 & \begin{tabular}[c]{@{}l@{}}\citet{PS23santos2023designing}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Designing for Cognitive Diversity: Improving the GitHub Experience for Newcomers \end{tabular} & 2023 \\ \hline

PS24 & \begin{tabular}[c]{@{}l@{}}\citet{PS24santos2021can}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Can i solve it? identifying apis required to complete oss tasks \end{tabular} & 2021 \\ \hline

PS25 & \begin{tabular}[c]{@{}l@{}}\citet{PS25minto2007recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending Emergent Teams \end{tabular} & 2007 \\ \hline

PS26 & \begin{tabular}[c]{@{}l@{}}\citet{PS26heimburger2020gamifying}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Gamifying onboarding: How to increase both engagement and integration of new employees \end{tabular} & 2020 \\ \hline

PS27 & \begin{tabular}[c]{@{}l@{}}\citet{PS27malheiros2012source}\end{tabular} & \begin{tabular}[c]{@{}l@{}} A source code recommender system to support newcomers \end{tabular} & 2012 \\ \hline

PS28 & \begin{tabular}[c]{@{}l@{}}\citet{PS28yang2016repolike}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Repolike: personal repositories recommendation in social coding communities \end{tabular} & 2016 \\ \hline

PS29 & \begin{tabular}[c]{@{}l@{}}\citet{PS29zhou2021ghtrec}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Ghtrec: a personalized service to recommend github trending repositories for developers \end{tabular} & 2021 \\ \hline

PS30 & \begin{tabular}[c]{@{}l@{}}\citet{PS30venigalla2022gitq}\end{tabular} & \begin{tabular}[c]{@{}l@{}} GitQ-towards using badges as visual cues for GitHub projects \end{tabular} & 2022 \\ \hline

PS31 & \begin{tabular}[c]{@{}l@{}}\citet{PS31sun2018personalized}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Personalized project recommendation on GitHub \end{tabular} & 2018 \\ \hline

PS32 & \begin{tabular}[c]{@{}l@{}}\citet{PS32sarma2009tesseract}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Tesseract: Interactive Visual Exploration of Socio-Technical Relationships in Software Development \end{tabular} & 2009 \\ \hline

\end{tabular}
\end{table*}

%-----------------------------


\begin{comment}
    
%-----------------------------
The risk of bias (RoB) for each Study is shown in Table \ref{tab:tab:RoB}. The RoB starting point for each Study is Low because none of the studies
... %However, because ..., we have revised our initial assessment to Moderate. 

Although Sx ...., it ..., therefore we provide only one risk of methodological RoB assessment for that Study.

We excluded Sx and Sx from our synthesis because both studies were duplicated by other studies (Sx and Sx respectively).

Study x ... Sx ... Neither Study reported .... which was reported by all other studies.

The Sx, although it might appear to meet the inclusion criteria, was excluded because ...

\begin{table*}[!ht]
\centering
\caption{Risk of Bias Assessment (RoB) in Studies}
\label{tab:RoB}
\begin{tabular}{p{8cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}|p{0.5cm}} \hline

{\textbf{RoB question}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} & {\textbf{Sx}} \\ \hline

\textbf{....} & Low & Low & Low & Low & Low & Low & Low & Low & Low & Low   \\ \hline

\textbf{....} & ... & ... & ... & ... & ... & ... & ... & ... & ... & ...   \\ \hline

\end{tabular}
\end{table*}

If we had selected Sx for inclusion  .... Therefore, excluded Sx is consistent with our protocol. The consequence of exclude Sx is that ... this suggests that ...

\end{comment}

%-----------------------------
\vspace{0.1cm}
\subsection{Data Collection Process} 

 
With the final set of studies decided upon, we carried out the data extraction activity on all included papers. One researcher was responsible for extracting the data and completing the associated forms. For validation purposes, a sample comprising 20\% of the total number of studies was selected randomly and had their data extracted by another researcher. The level of agreement between the researchers was 100\%). 


%-----------------------------
\vspace{0.1cm}
\subsection{Data Synthesis Process} 

The data synthesis activity involved compiling the data extracted from each study included in our SLR. Most of the selected primary studies were conference primary studies, accounting for 30 primary studies (94\%), while there were two (2) journal studies (6\%). Table~\ref{tab:studiesvenue} provides a comprehensive list of the conferences and journals where these primary studies have been published. This information can be valuable for practitioners and researchers interested in this topic, as it helps identify relevant conferences for future publication opportunities. Notably, ICSE, one of the prominent software engineering conferences, had the highest number of published primary studies, followed by the FSE conference. The journals that featured publications were IEEE Access and Science China Information Sciences.

\begin{table}[!ht]\scriptsize
\centering
\caption{Selected studies published by venue}
\label{tab:studiesvenue}
\begin{tabular}{l|c|c|c}
\hline
\multicolumn{1}{c|}{\textbf{Venue}} & \textbf{\# of studies} & \textbf{ID} & \textbf{\%} \\ \hline \hline

ICSE & 7 & \begin{tabular}[c]{@{}c@{}}PS01, PS03, \\PS07, PS15, \\PS19, PS23, PS32\end{tabular} & 22\% \\ \hline
FSE & 3 & PS02, PS08, PS12 & 9\% \\ \hline
CHASE & 2 & PS04, PS18 & 6\% \\ \hline
ICSME & 2 & PS09, PS14 & 6\% \\ \hline
COMPSAC & 2 & PS20, PS27 & 6\% \\ \hline
MSR & 2 & PS24, PS25 & 6\% \\ \hline
BotSE & 1 & PS05 & 3\% \\ \hline
IWCSN & 1 & PS06 & 3\% \\ \hline
CAiSE & 1 & PS10 & 3\% \\ \hline
SEAA & 1 & PS11 & 3\% \\ \hline
CONVERSATIONS & 1 & PS13 & 3\% \\ \hline
RSSE & 1 & PS16 & 3\% \\ \hline
IHC & 1 & PS17 & 3\% \\ \hline
VL/HCC & 1 & PS21 & 3\% \\ \hline
AHFE & 1 & PS26 & 3\% \\ \hline
ICWS & 1 & PS29 & 3\% \\ \hline
ICPC & 1 & PS30 & 3\% \\ \hline
IEEE Access & 1 & PS22 & 3\% \\ \hline
Internetware & 1 & PS28 & 3\% \\ \hline
\begin{tabular}[c]{@{}l@{}}Science China \\ Information Sciences\end{tabular} & 1 & PS31 & 3\% \\ \hline \hline

\end{tabular}
\end{table}

Table~\ref{tab:selectedstudiescountry} presents the geographic distribution of the selected primary studies, which originate from five continents and nine different countries. Notably, many primary studies involved collaboration among authors from multiple countries, thus contributing to the inclusion of more than one country. The majority of publications were from the USA (34\%), followed by Brazil (28\%) and China (25\%). The remaining countries contributed with approximately 1 to 3 publications each.


\begin{table}[!ht]\scriptsize
\centering
\caption{Selected studies per country}
\label{tab:selectedstudiescountry}
\begin{tabular}{l|l|c|c}
\hline
\multicolumn{1}{c|}{\textbf{Continent}} & \multicolumn{1}{c|}{\textbf{Country}} & \textbf{\# of studies} & \textbf{\%} \\ \hline \hline

\multirow{2}{*}{\textbf{Asia}} & \textbf{China} & 8 & 25\% \\ \cline{2-4} 
 & \textbf{India} & 1 & 3\% \\ \hline \hline
 
\multirow{3}{*}{\textbf{Europe}} & \textbf{Germany} & 3 & 9\% \\ \cline{2-4} 
 & \textbf{Italy} & 1 & 3\% \\ \cline{2-4} 
 & \textbf{Spain} & 2 & 6\% \\ \hline \hline
 
\multirow{2}{*}{\textbf{North America}} & \textbf{Canada} & 2 & 6\% \\ \cline{2-4} 
 & \textbf{USA} & 11 & 34\% \\ \hline \hline
\textbf{South America} & \textbf{Brazil} & 9 & 28\% \\ \hline \hline
\textbf{Oceania} & \textbf{Australia} & 1 & 3\% \\ \hline \hline
\end{tabular}
\end{table}

Figure~\ref{fig:publiyear} illustrates the annual distribution of primary studies published over time. The analysis reveals that the earliest paper in the dataset was published in 2003. From 2003 to 2011, there was a consistent trend of one paper published per year. Furthermore, starting in 2012, there was a notable increase in published primary studies, with the count rising from 3 to 7. This growth suggests a heightened interest and research activity in the field during the subsequent years.

\begin{figure}[h]
    \centering
    \includegraphics[width=8.5cm]{images/bargraphnew.pdf}
    \caption{Publication years and relevant paper counts.}
    \label{fig:publiyear}
\end{figure}


We created a word cloud by aggregating the keywords extracted from the 32 chosen primary studies, as illustrated in Figure~\ref{fig:wordcloud}. Word clouds have gained popularity as a simple yet visually captivating method for representing textual information. They are widely employed in various domains to provide an overview by highlighting the most frequently occurring words, serving as a concise textual summary~\cite{heimerl2014word}. 
%In our word cloud, prominent terms include open source, software, onboarding, and newcomers. 
Generating this word cloud based on the selected studies' keywords validates the search string's effectiveness in retrieving relevant results from the targeted data sources.

\begin{figure}[h]
    \centering
    \includegraphics[width=8.5cm]{images/WordArt.png}
    \caption{Keywords wordcloud.}
    \label{fig:wordcloud}
\end{figure}


\begin{comment}
We performed the data synthesis for our RQs using ..., %classification schemes, tables (totals and summaries), and visual representations (graphs), ...,
with details following. 

A closer inspection shows that our data can be structured into x linked categories. The first category contains ... The second contains
factors that ... 

Regarding analysis and synthesis of bias assessment, it is clear that Sx ... However, the ... used by Sx was unclear, while Sx always used ... . For this reason, we kept Sx in the data synthesis and omitted Sx. The ... seems well-founded and unbiased for all studies. However, only S4 used ...

X studies (Sx, Sx, ... and Sx) found ... while x studies (Sx, Sx, ... and Sx) found ... The remaining x studies (Sx, Sx, ... and Sx) had ... A problem with this assessment is that .... Comparing .... with ... 

We also considered the relationship between ... and ... This analysis was
not planned when the study protocol was developed, but observing
our data, it seemed that, in contrast to .... 

Regarding heterogeneity, the majority of the studies (x) were based on providing ..., which is what happens ... %in real-life software development contexts. 

Only x studies provided the same information to the ... Hence, it is difficult to conclude about ....


%-----------------------------
\vspace{0.1cm}
\textbf{SLR's results} 
% Presenting resulting following MOCC (Motivators, Outcomes, Characteristics and Context) model.

Based on the extraction %and categorization/summarization results, 
it was possible to answer the RQs proposed in this SLR, which will be discussed following.

{\textbf{RQ1:} \textit{...?}}

With this question, we investigated ...

{\textbf{RQ2:} \textit{...?}}

With this question, we ...

Our investigation resulted in x findings:
\begin{itemize}
    \item \textbf{F1 --} ....
    \item \textbf{F2 --} ....
    \item \textbf{Fx --} ....

\end{itemize}

In general, our findings suggest that ...

Table \ref{tab:certainty} shows our assessment of the quality of the evidence supporting our individual findings. 

\begin{table*}[!ht]
\centering
\caption{Assessment of Certainty in the Body of Evidence for x Findings }
\label{tab:certainty}
\begin{tabular}{l|p{11cm}|l} \hline

{\textbf{Issue}} & {\textbf{Comment}} & {\textbf{Assessment}} \\ \hline
%F1 -- Study RoB & ...  & Low RoB \\ \hline
\textbf{F1} -- Missing data & The first search process was very rigorous, and the second included snowballing. & Low RoB \\ \hline
\textbf{F1} -- Inconsistency & Initial inconsistencies in results were substantially reduced by comparing the .... & Low Inconsistency \\ \hline
\textbf{F1} -- Coherence & X of x studies ... Also x studies reported ... Thus, x of the x sources of evidence supported the finding. & Minor Concerns \\ \hline
\textbf{F1} -- Relevance & This issue is extremely important for companies & No Concerns \\ \hline
\multicolumn{2}{l}{\textbf{F1 -- Overal quality of evidence}} & \textbf{Moderate Quality} \\ \hline

\textbf{F2} -- Methodology & ...  & ... \\ \hline
\textbf{F2} -- Adequacy & In terms of Data Adequacy, x studies compared ... with ..., so we
have more evidence about .... However, ...., which also support Fx. Only one of the studies (Sx) .... We conclude there are Minor concerns about
Data Adequacy.  & Minor Concerns \\ \hline
\textbf{F2} -- ... & ...  & ... \\ \hline
\multicolumn{2}{l}{\textbf{F2 -- Overal quality of evidence}} & \textbf{...} \\ \hline

\end{tabular}
\end{table*}

For F1, ... In terms of ..., we have x ...
For F2, ... Overall, we rate confidence in the quality of the evidence
supporting F2 to be Moderate, meaning that ``It is likely that the
review finding is a reasonable representation of the phenomenon of
interest''.

%-----------------------------
\vspace{0.1cm}
\textbf{Discussion and Limitations}

Overall none of our findings supported the idea that ... In particular, there was no ...

Summarising the limitations of this SLR, we identified x issues that might impact the certainty of the evidence:
\begin{itemize}
    \item Few studies that investigated ....
    \item ...
    \item The studies only included formal experiments, i.e., no industry case studies.  
\end{itemize}

...

%-----------------------------
\vspace{0.1cm}
\textbf{Applications for Practice and Future Research}

... we, therefore, recommend that ... Further research on this topic should consider ...

%-----------------------------
\vspace{0.1cm}
\textbf{Availability Of Protocol, Data and Other Materials}
Supplementary material related to this article can be found online
at https:...

\end{comment}

%-----------------------------
%\vspace{0.1cm}
%\subsection{Declaration of competing interest}

%No author associated with this paper has disclosed any potential or pertinent conflicts which may be perceived to have an impending conflict with this work. For full disclosure statements, refer to https://doi.org/10.1016/j.infsof.2021.106783.



==> OLD_Sections/olddiscussion.tex <==


\textbf{Technological interventions for newcomer onboarding.} We have explored the different types of technological interventions for newcomer onboarding in software projects presented in the literature. Our findings reveal that these interventions encompass a range of approaches, including recommending suitable projects (PS05, PS07, PS21, PS22, PS28, PS29, PS31) or newcomers support tool (PS15), redesigning the OSS environment to influence newcomer interaction (PS04, PS11, PS17, PS23, PS30), facilitating interaction between newcomers and experienced mentors (PS02, PS06, PS09, PS16, PS25), and community initiatives for guidance and assistance (PS07, PS09, PS16, PS25).


There is a rise in recommendation systems designed to aid developers in a diverse array of activities. These systems assist developers in finding relevant information and evaluating alternative decisions, thereby covering a broad spectrum of software engineering tasks~\cite{robillard2009recommendation, dagenais2011recommending}. Moreover, these  systems have the potential to handle vast amounts of development data, offering practical support to developers. One notable approach that emerged related to newcomers' onboarding interventions is the integration of recommendation mechanisms in supporting newcomers. Recommendation of source files (PS03, PS10, PS20, PS27), tasks (PS12, PS13, PS14, PS18), and issue labels (PS08, PS19, PS24) are some examples. These mechanisms aim to guide newcomers in exploring and integrating source code files, suggesting relevant tasks or bugs, and recommending initial tasks or issues for engagement. 

Machine learning has emerged as a thriving discipline with a wide range of practical applications and ongoing research areas. Notably, the intersection of machine learning and software engineering has become increasingly prominent~\cite{meinke2018, kotti2023machine}. By harnessing machine learning techniques, we gain the ability to tackle software engineering problems that are challenging to model purely through algorithms or lack satisfactory solutions using traditional approaches~\cite{zheng2006value}. This integration allows for innovative solutions and advancements in the field. Among the selected studies, machine learning techniques have been employed in many studies (PS06, PS08, PS14, PS19, PS24, PS28, PS29) to improve the effectiveness of these recommendation systems, enabling personalized and automated suggestions.

Gamification aims to enhance user engagement, motivation, and performance by integrating game mechanics and elements into a specific task, thereby increasing its appeal. The application of gamification in software engineering has garnered significant research attention, with the goal of improving developer engagement and outcomes~\cite{pedreira2015gamification}. There is a growing interest in utilizing gamification (PS04, PS17, PS26) and modifying the OSS environment (PS04, PS17, PS23, PS30) to enhance newcomer engagement and motivation.  \citet{PS04diniz2017using}~(PS04), applied gamification elements such as rankings, quests, points, and levels have been introduced to orient and motivate newcomers. Additionally, the redesign of the OSS environment, including the use of plugins and web portals, aims to address inclusivity bugs (PS23), provide assistance and resources (PS17), and offer visual cues related to project architecture and maintenance (PS30).

Recommendation systems play a crucial role in supporting newcomer onboarding, covering various categories such as community support (PS09, PS16, PS25), mentor/expert recommendation (PS02, PS06, PS09, PS16, PS25), issue label recommendation (PS08, PS19, PS24), project recommendation (PS05, PS21, PS22, PS28, PS29, PS31), SPL feature recommendation (PS10), and source files recommendation (PS10, PS27). These systems leverage historical data, social connections, and machine learning algorithms to recommend suitable mentors, projects, or specific resources to newcomers. Finally, support tools specifically designed for newcomer onboarding have been developed. These tools focus on tasks such as recommending source files (PS03), suggesting relevant tasks or bugs (PS12, PS18), providing assistance and resources (PS15), and integrating gamification elements to enhance motivation and engagement (PS26).

By comprehensively organizing and categorizing these interventions, our paper aims to provide a comprehensive overview of the available approaches that effectively support newcomers in their transition and integration into software projects. The findings highlight the diverse applications of technological interventions and provide insights into potential areas for further exploration and improvement in newcomer onboarding.

\textbf{Impact of technology interventions.} We examined the impact of technology interventions on newcomers' onboarding in software projects. The researchers categorized the selected studies into five distinct categories, each representing a different aspect of the impact. The category with the highest number of studies, comprising 14 studies (45\%), focused on the contribution process and orientation. Newcomers need proper orientation to navigate the project and correctly make contributions~\cite{PS15steinmacher2016overcoming}. Motivating, engaging, and retaining new developers in a project is essential to sustain a healthy OSS community~\cite{qureshi2011socialization}.By introducing and guiding newcomers through the contribution process, these approaches aimed to facilitate their integration and active participation in OSS projects (PS07, PS10, PS11, PS13, PS15, PS17, PS21, PS22, PS23, PS26, PS28, PS29, PS30, PS31).

According to~\cite{balali2020recommending} labeling/tagging is a widespread practice for providing support in task selection in software projects. Some studies (23\%) highlighted the importance of categorizing and labeling tasks within the project to assist newcomers in identifying tasks that align with their skill levels and interests. By marking tasks with appropriate labels and providing clear descriptions and instructions, these approaches aimed to enable newcomers to easily select and engage with tasks that are suitable for their capabilities (PS08, PS12, PS13, PS14, PS18, PS19, PS24).

\citet{begel2008novice} discuss the importance, advantages and challenges of mentoring for novices in the software industry. The impact of mentoring in the onboarding process was also evident, with seven studies (23\%) focusing on this aspect. Mentoring plays a crucial role in pairing experienced contributors with newcomers to provide guidance, support, and knowledge transfer. By establishing constructive learning relationships between mentors and mentees, these approaches fostered the growth and integration of newcomers into the OSS community (PS02, PS06, PS09, PS12, PS13, PS16, PS25).

Furthermore, the researchers identified approaches (19\%) that aimed to enhance newcomers' experience within software projects (PS04, PS05, PS17, PS20, PS23, PS26). Other studies (13\%) focused on improving productivity through technology interventions. By adopting these initiatives, software projects aimed to optimize newcomers' productivity and facilitate their seamless integration into the development process (PS01, PS03, PS20, PS27). In conclusion, the findings of this study highlight the diverse impact of technology interventions on newcomers' onboarding in software projects. By focusing on aspects such as the contribution process, labeling and task selection, mentoring, enhancing newcomers' experience, and improving productivity, these interventions contribute to facilitating the integration and effectiveness of newcomers in software development communities.

\textbf{Evaluation measures and metrics.} Software engineering is a dynamic and interdisciplinary domain that encompasses various social and technological aspects. To gain comprehensive insights it is crucial to investigate not only the tools and processes employed but also the social and cognitive dimensions that surround them. This necessitates a deep understanding of human activities to explore how individual software engineers engage in software development and how teams and organizations coordinate their efforts to achieve success. By studying these aspects, researchers can gain a holistic understanding of software engineering practices and enhance the ability to support effective software development processes~\cite{easterbrook2008selecting}. The analysis of the selected primary studies revealed several types of evaluations. Most studies (52\%) applied qualitative analysis allowing researchers to delve into the nuances of the onboarding process and capture valuable insights from the participants (PS01, PS02, PS03, PS04, PS07, PS10, PS13, PS14, PS15, PS17, PS20, PS21, PS23, PS26, PS29, PS31). In addition, 35\% of the studies opted for quantitative analysis to quantify the impact and effectiveness of the technological interventions, providing concrete evidence of their outcomes (PS01, PS02, PS06, PS13, PS14, PS15, PS19, PS22, PS23, PS24, PS30).

Among the studies, computer evaluations were conducted in 32\% (PS08, PS09, PS10, PS19, PS20, PS24, PS25, PS27, PS28, PS29). Computer-based evaluations offer an objective and systematic approach to evaluating the effectiveness of onboarding interventions, allowing for precise measurement and analysis of various parameters. Moreover, empirical evaluations were carried out in 10\% of the studies (PS11, PS22, PS23). These evaluations involved observing, collecting, and analyzing real-world data from users in software projects. By directly engaging with actual users, researchers could assess the impact, effectiveness, and user experience of different onboarding interventions in practical settings. 

Overall, the findings highlight the diverse range of evaluation methods employed to assess the effectiveness of technology interventions for newcomers' onboarding. The inclusion of empirical evaluation was prominent in the selected studies, signifying its importance in understanding the practical implications of onboarding approaches. By employing a combination of evaluation methods, researchers can gain a comprehensive understanding of the impact and effectiveness of technological interventions for newcomers' onboarding in software projects.


%&&&&&&

%%%%% Include in the new discussion

\textbf{Newcomers' orientation.}

The following onboarding barriers do not have any specific onboarding intervention approaches proposed in the literature, due to that we highlight them as research opportunities that emerge to be further investigated by the software engineering community, these barriers are related to newcomers' orientation such as: \textbf{\textit{(i) outdated list of bugs:}} other opportunities would be developing interventions to ensure that bug lists or issue repositories are regularly updated, providing newcomers with up-to-date and relevant tasks. This may involve implementing mechanisms for tracking the status and activity of reported issues; \textbf{\textit{(ii) reproducing issues:}} Another interesting point would be to explore techniques and tools to assist newcomers in reproducing reported issues, enabling them to understand and address problems effectively. This may involve creating reproducibility guidelines, providing virtualized or sandboxed environments, or offering step-by-step debugging support;


\textbf{Newcomers' characteristics.}

Despite the progress made in developing onboarding interventions for mitigating barriers related to newcomers' characteristics, there are some barriers that can be seen as research opportunities that require further exploration. Among the opportunities we have the following: \textbf{\textit{(i) lack of proactivity:}} investigating approaches to encourage newcomers to take a proactive stance in their onboarding process. This may involve designing interventions, creating platforms for collaboration and engagement, and providing incentives to motivate newcomers to actively seek knowledge and participate in project activities; \textbf{\textit{(ii) lack of commitment:}} exploring interventions to enhance newcomers' commitment levels throughout the onboarding journey. This could involve developing personalized onboarding plans, setting clear goals and expectations, and providing regular feedback and recognition to foster a sense of commitment and accountability; \textbf{\textit{(iii) underestimating the challenge:}} Understanding and addressing the issue of newcomers underestimating the challenges they may face during the onboarding process. This may involve providing realistic expectations, highlighting the learning curve, and offering support mechanisms to help newcomers navigate difficulties and setbacks effectively; and \textbf{\textit{(iv) lack of patience:}} investigating approaches to cultivate patience and resilience among newcomers when encountering obstacles or setbacks during their onboarding journey. This could include mentorship programs, peer support networks, and guidance on managing expectations and building a growth mindset.

\textbf{Communication.}

While existing onboarding interventions have made progress in mitigating communication barriers, there are still research opportunities to further enhance the onboarding process. These opportunities include addressing the following areas: \textbf{\textit{(i) answering with too advanced/complex contents:}} exploring methods to ensure that answers provided to newcomers are understandable and suitable for their level of knowledge and expertise. This may involve creating knowledge resources with varying levels of complexity, encouraging community members to provide clear and concise explanations, and promoting effective communication practices; \textbf{\textit{(ii) not sending a meaningful/correct message:}} investigating interventions to improve the quality and accuracy of communication from both newcomers and existing members. This could include providing communication guidelines, offering templates or examples of effective messages, and encouraging constructive feedback and peer review of communication exchanges; \textbf{\textit{(iii) English level:}} addressing language barriers for non-native English speakers. This may involve providing language support resources, facilitating language exchanges or translation assistance, and promoting inclusive and multicultural communication practices within the community; \textbf{\textit{(iv) shyness:}} exploring approaches to support and empower shy or introverted newcomers in their communication efforts. This could include creating safe spaces for interaction, offering communication training, and providing mentorship or peer support specifically tailored to help shy individuals overcome barriers and engage in effective communication; \textbf{\textit{(v) making useless comments in the mailing list/forum:}} investigating methods to foster meaningful and productive discussions by discouraging irrelevant or low-value comments. This may involve community moderation, setting guidelines for constructive participation, and promoting a culture of mutual respect and relevance in communication platforms; \textbf{\textit{(vi) low responsiveness:}} exploring ways to enhance responsiveness from existing members when interacting with newcomers. This could include incentivizing and recognizing responsive behavior, establishing clear expectations for community participation, and implementing systems to track and measure responsiveness levels; \textbf{\textit{(vii) not acknowledging/thanking answers:}} investigating approaches to encourage newcomers to acknowledge and express gratitude for the assistance they receive. This may involve raising awareness about the importance of appreciation in community dynamics, providing guidance on appropriate ways to express gratitude, and fostering a culture of appreciation and recognition.

\textbf{Documentation.}

Those existing onboarding interventions have made progress in mitigating documentation problems, but there are still research opportunities to further enhance the onboarding process. These opportunities include addressing the following areas: \textbf{\textit{(i) unclear documentation:}} investigating methods to improve the clarity and comprehensibility of documentation. This may involve conducting usability studies, employing natural language processing techniques to analyze and enhance documentation readability, and incorporating user feedback and testing to identify and address areas of confusion or ambiguity. \textbf{\textit{(ii) Code comments not clear:}} This includes providing guidelines for writing clear and descriptive comments, encouraging code reviews and feedback, and promoting a culture of code documentation within the development community;

\textbf{Technical Hurdles.}

While existing onboarding interventions have made progress in mitigating technical hurdles, there are still research opportunities to further enhance the onboarding process. These opportunities include addressing the following areas: (i) code characteristics: investigating the characteristics of code that pose challenges for newcomers, such as code quality, complexity, instability, and adherence to coding standards. This may involve conducting code analysis, developing tools for automated code quality assessment, and exploring methods to simplify complex code structures; and (ii) Change request hurdles: This includes creating templates for change requests, specifying the required information and format. Additionally, offering mentorship where experienced members guide newcomers through the change request process can help address this barrier effectively.



%&&&&&&

\textbf{Addressing newcomers' barriers.} A better understanding of the barriers enables communities and researchers to design and produce tools and conceive interventions to better support newcomers~\cite{balali2018newcomers}. In our study, we aim to evaluate existing onboarding interventions proposed in the literature and assess their effectiveness in addressing and mitigating these barriers. One crucial phase in facilitating newcomers' successful integration and contribution is their orientation to the community or organization. However, this phase is hindered by several barriers, including challenges in finding appropriate tasks to start with (PS04, PS05, PS07, PS08, PS12, PS13, PS14, PS15, PS17, PS18, PS19, PS24, PS31) and accessing mentors for guidance and support (PS02, PS05, PS06, PS09, PS12, PS13, PS14, PS15, PS16, PS19, PS31). Mentorship is a widely utilized approach in open collaboration communities to assist newcomers in overcoming the challenges they encounter during their initial stages of participation~\cite{hsieh2013welcome, fagerholm2014role}. Our analysis of the selected studies revealed several onboarding interventions that effectively address these challenges. Approaches such as task recommendation systems, clear guidelines for task selection, and mentorship programs contribute to facilitating newcomers' engagement and meaningful contributions from the beginning.

We also identified the barriers related to newcomers' orientation proposed in~\cite{steinmacher2019overcoming} that lack specific onboarding strategy approaches in the literature. These barriers present valuable research opportunities for the software engineering community. For example, exploring methods to assist newcomers in finding the correct artifacts to fix an issue, improving the availability and accessibility of comprehensive "How to Contribute" resources, ensuring up-to-date bug lists or issue repositories, developing techniques and tools for issue reproduction, and providing clear guidance on the contribution flow are all areas that require further investigation. By addressing these research gaps that focus on newcomers orientation, we can enhance newcomers support and provide a successful integration into software projects.

Another barrier comes from the newcomers' characteristics that pose significant challenges during the onboarding process such as: (i) lack of domain experience (PS01, PS03, PS05, PS07, PS08, PS10, PS11, PS12, PS15, PS20, PS23, PS27, PS29, PS31); (ii) lack of knowledge in project process and practices (PS01, PS02, PS03, PS04, PS05, PS06, PS07, PS08, PS10, PS11, PS15, PS16, PS17, PS20, PS21, PS22, PS23, PS24, PS26, PS27, PS28, PS29, PS30, PS31); and (iii) lack of technical background (PS01, PS03, PS05, PS07, PS08, PS09, PS10, PS11, PS15, PS18, PS20, PS23, PS25, PS27, PS31). By implementing these interventions, organizations and communities can help newcomers acquire domain expertise and contribute effectively within their respective domains and enhance newcomers' technical skills, fill knowledge gaps, and build their confidence to actively contribute to technical projects.

While progress has been made in developing onboarding interventions to address barriers related to newcomers' characteristics, there are still research opportunities that warrant further exploration. These include investigating approaches to encourage newcomers to take a proactive stance in their onboarding process, enhancing newcomers' commitment levels throughout their journey, addressing the issue of newcomers underestimating the challenges they may face, and cultivating patience and resilience among newcomers. By delving into these research opportunities, we can further refine onboarding practices and create a more inclusive and supportive environment for newcomers in various domains.

Literature highlights that newcomers often face challenges related to community protocol, language, and appropriate communication~\cite{steinmacher2019overcoming}. Fortunately, specific approaches have been proposed to mitigate these barriers and enhance communication between newcomers and existing community members addressing the following barriers: (i) not receiving an answer (PS15, PS16, PS25); (ii) sending a message that is considered impolite (PS15, PS16, PS25); and (iii) need to contact a real person (PS02, PS05, PS06, PS09, PS12, PS15, PS16, PS25, PS26). Providing effective communication channels to contact real people, such as mentorship programs, would be beneficial in fostering interaction and support for newcomers.

While existing onboarding interventions have made progress in mitigating communication barriers, there are still research opportunities to enhance the process further. These opportunities include investigating methods to reduce delays in answering newcomers' inquiries, ensuring that answers are understandable and suitable for newcomers' knowledge level, improving the quality and accuracy of communication from both newcomers and existing members, addressing language barriers for non-native English speakers, supporting shy or introverted newcomers in their communication efforts, fostering meaningful and productive discussions, enhancing responsiveness from existing members, encouraging newcomers to acknowledge and express gratitude for assistance, and promoting a culture of appreciation and recognition within the community. By exploring these research opportunities, we can refine communication practices and create a more inclusive and supportive environment that facilitates effective interactions and knowledge exchange between newcomers and the existing community.

Some approaches focused on onboarding interventions to mitigate issues related to documentation problems and enhance its effectiveness and usability for newcomers. To address the barrier of outdated information, it is crucial to prioritize maintaining up-to-date documentation (PS03, PS11, PS15). By actively involving the community in the documentation process, inaccuracies can be identified and addressed more efficiently. Mitigating the barrier of information overload involves organizing and structuring documentation in a user-friendly manner (PS03, PS11, PS15, PS23). By optimizing the usability of documentation, newcomers can find the most relevant information based on their specific needs, thereby improving their understanding and efficiency.

Addressing the barrier of unclear code comments emphasizes the importance of maintaining well-documented code (PS03, PS11, PS15). By promoting comprehensive code documentation practices, newcomers can better comprehend the project code and navigate through it effectively. Concerning the barrier of lack of documentation, it is essential to actively create and improve documentation resources (PS03, PS11, PS15, PS20, PS23). By prioritizing the creation and enhancement of documentation, newcomers can reduce the time spent on studying the project code and improve the accuracy of their learning process.

While existing onboarding interventions have made progress in mitigating documentation problems, there are still research opportunities to enhance the onboarding process. These opportunities include investigating methods to improve the clarity and comprehensibility of documentation through usability studies and natural language processing techniques. Additionally, exploring approaches to consolidate and centralize documentation resources can involve developing unified platforms, implementing knowledge management systems, and establishing clear guidelines for documentation organization and structure to avoid fragmentation and scattered information. By addressing these areas, we can create a more streamlined and user-friendly documentation experience for newcomers, facilitating their integration into the project and enhancing their overall onboarding process.

The onboarding process for newcomers often involves overcoming technical hurdles. Existing interventions aim to facilitate newcomers' understanding and navigation of technical aspects within a project. These interventions include streamlining the local environment setup process (PS01, PS03, PS04, PS10, PS11, PS15, PS20, PS25, PS27), providing comprehensive instructions, and offering pre-configured development environments to ensure a smooth onboarding experience. Additionally, documentation and guidance play a crucial role in helping newcomers overcome code and architecture hurdles (PS01, PS02, PS03, PS04, PS10, PS11, PS15, PS20, PS23, PS25, PS27). Interventions focus on providing code walkthroughs, architectural diagrams, and high-level overviews of the project structure to aid newcomers in navigating the codebase and understanding the project's architecture. Clear guidelines for submitting and handling change requests are also important (PS01, PS03, PS04, PS10, PS11, PS15, PS19, PS20, PS25, PS27, PS30, PS31). Interventions involve creating templates, specifying required information and formats, and establishing communication channels between newcomers and project contributors. Mentorship programs can further support newcomers in navigating the change request process.

While progress has been made in mitigating technical hurdles, there are still research opportunities to enhance the onboarding process. One area of exploration is the investigation of code characteristics that pose challenges for newcomers, such as code quality, complexity, instability, and adherence to coding standards. Analyzing code and developing automated tools for code quality assessment can be valuable in addressing this. Another area to explore is the cognitive aspects of understanding and working with code. Research can focus on studying the cognitive processes involved in code comprehension, developing visualizations or interactive tools to improve code understanding, and identifying common cognitive barriers faced by newcomers. It is important to note that addressing cognitive barriers, as highlighted by \citet{PS23santos2023designing}~(PS23), is a crucial aspect that requires further attention in the onboarding process. The onboarding of newcomers has been studied in different online collective production communities~\cite{jensen2011joining, halfaker2013rise, hannebauer2014exploratory, steinmacher2015social} and it also affects commercial software development settings~\cite{begel2008novice, dagenais2010moving}.

\textbf{Diversity and inclusion in technological interventions.} Newcomers encounter various challenges, which affect underrepresented populations differently and can result in a steeper learning curve, a lack of community support, and difficulties in initiating contributions, all contributing to the existing diversity imbalance in OSS~\cite{steinmacher2015social, padala2020gender, trinkenreich2021women}. Numerous studies have emphasized the positive impact of social diversity on productivity, teamwork, and the quality of contributions. The literature has highlighted concerns regarding the low diversity in OSS, considering factors such as gender, language, and location~\cite{storey2016social, bosu2019diversity, guizani2022debug, trinkenreich2021women}. Previous research has demonstrated that diverse teams tend to be more productive, reinforcing the significance of addressing diversity-related issues in OSS~\cite{vasilescu2015gender}. Our analysis revealed that the majority of the proposed onboarding interventions (97\%) targeted a general newcomer population without considering or evaluating their effectiveness for integrating different user types into software projects. Only one study (3\%) specifically focused on providing tailored support for newcomers with specific cognitive styles (PS23), which often present barriers to programming for certain populations. Regarding the explicit focus on diversity and inclusion, the majority of studies (94\%) did not mention any specific emphasis in this regard, while a small percentage (6\%) explicitly addressed diversity and inclusion concerns (PS07, PS23). These findings underscore the need for more research and the development of inclusive onboarding interventions to promote diversity and inclusion within software communities.

In conclusion, our study highlights the importance of prioritizing diversity and inclusion in technological interventions for newcomers. By addressing the specific needs and barriers faced by underrepresented groups, we can create more inclusive onboarding processes and foster greater diversity within software projects. This research serves as a call to action for the software engineering community to actively work towards creating inclusive environments that welcome individuals from diverse backgrounds and leverage their unique perspectives for the benefit of the entire community.




%%%% old part

\textbf{Addressing newcomers' barriers.} A better understanding of the barriers enables communities and researchers to design and produce tools and conceive interventions to better support newcomers~\cite{balali2018newcomers}. One crucial phase in facilitating newcomers' successful integration and contribution is their orientation to the community or organization. The onboarding of newcomers has been studied in different online collective production communities~\cite{jensen2011joining, halfaker2013rise, hannebauer2014exploratory, steinmacher2015social} and it also affects commercial software development settings~\cite{begel2008novice, dagenais2010moving}.

In our study, we aim to understand existing onboarding interventions proposed in the literature and assess their effectiveness in addressing and mitigating these barriers. Mentorship is a widely utilized approach in open collaboration communities to assist newcomers in overcoming the challenges they encounter during their initial stages of participation~\cite{hsieh2013welcome, fagerholm2014role}. Our analysis of the selected studies revealed onboarding interventions that effectively address these challenges. 

In our investigation, we also pinpointed noteworthy research gaps pertaining to the obstacles encountered by newcomers during the onboarding process, as highlighted by~\citet{steinmacher2019overcoming}. Notably, we observed an absence of technological onboarding interventions designed to tackle these specific barriers. We highlight research opportunities that emerge related to \textit{newcomers' orientation} such as: \textbf{\textit{(i) outdated list of bugs:}} developing interventions to ensure that bug lists or issue repositories are regularly updated, this may involve implementing mechanisms for tracking the status and activity of reported issues; \textbf{\textit{(ii) reproducing issues:}} this may involve creating reproducibility guidelines, providing virtualized or sandboxed environments, or offering step-by-step debugging support tools.

Among the opportunities focused on the barriers related to \textit{newcomers' characteristics}, we have the following: \textbf{\textit{(i) lack of proactivity:}} this may involve designing interventions, creating platforms for collaboration and engagement, and providing incentives to motivate newcomers to actively seek knowledge and participate in project activities; \textbf{\textit{(ii) lack of commitment:}} this could involve developing personalized onboarding plans, setting clear goals and expectations, and providing regular feedback and recognition to foster a sense of commitment and accountability; \textbf{\textit{(iii) underestimating the challenge:}} This may involve providing realistic expectations, highlighting the learning curve, and offering support mechanisms to help newcomers navigate difficulties and setbacks effectively; and \textbf{\textit{(iv) lack of patience:}} this could include mentorship programs, peer support networks, and guidance on managing expectations and building a growth mindset.

While existing onboarding interventions have made progress in mitigating communication barriers, there are still research opportunities to further enhance the onboarding process. These opportunities include: \textbf{\textit{(i) answering with too advanced/complex contents:}} this may involve creating knowledge resources with varying levels of complexity, encouraging community members to provide clear and concise explanations; \textbf{\textit{(ii) not sending a meaningful/correct message:}} this could include providing communication guidelines, offering templates or examples of effective messages, and encouraging constructive feedback and peer review of communication exchanges; \textbf{\textit{(iii) English level:}} this may involve providing language support resources, facilitating language exchanges or translation assistance, and promoting inclusive and multicultural communication practices within the community; \textbf{\textit{(iv) shyness:}} this could include creating safe spaces for interaction, offering communication training, and providing mentorship or peer support specifically tailored to help shy individuals overcome barriers and engage in effective communication; \textbf{\textit{(v) making useless comments in the mailing list/forum:}} this may involve community moderation, setting guidelines for constructive participation, and promoting a culture of mutual respect in communication platforms; \textbf{\textit{(vi) low responsiveness:}} this could include incentives and recognizing responsive behavior, establishing clear expectations for community participation; \textbf{\textit{(vii) not acknowledging/thanking answers:}} this may involve raising awareness about the importance of appreciation in community dynamics, providing guidance on appropriate ways to express gratitude, and fostering a culture of appreciation and recognition.

Some opportunities focused on \textit{documentation} barriers include addressing the following areas: \textbf{\textit{(i) unclear documentation:}} this may involve conducting usability studies, employing natural language processing techniques to analyze and enhance documentation readability, and incorporating user feedback. \textbf{\textit{(ii) Code comments not clear:}} this includes providing guidelines for writing clear and descriptive comments, encouraging code reviews and feedback, and promoting a culture of code documentation within the development community.

While existing onboarding interventions have made progress in mitigating technical hurdles, there are still research opportunities to further enhance this barrier that includes:  \textbf{\textit{(i) code characteristics:}} this may involve conducting code analysis, developing tools for automated code quality assessment, and exploring methods to simplify complex code structures; and  \textbf{\textit{(ii) Change request hurdles:}} this includes creating templates for change requests, specifying the required information and format.

These barriers present valuable research opportunities for the software engineering community. By addressing these research gaps that focus on newcomers onboarding barriers, we can enhance newcomers support and provide a successful integration into software projects.

==> OLD_Sections/oldintro.tex <==
%\boldification{Onboarding software projects}
%Effective onboarding enables new employees to acquire the necessary attitudes, knowledge, skills, and behaviors for effective work~\cite{bauer2011onboarding, cable2013reinventing, klein2015specific}. The onboarding process can assume either a formal or informal structure~\cite{zahhly1989differential, louis1983availability}. 
Within the software development context, several reasons necessitate the onboarding of newcomers, including (i) to replace retired developers, (ii) to replace developers that left or will leave the company, (iii) to scale up the number of developers in response to the growth of the number of customers, (iv) to incorporate new people that may bring new ideas and thus help a company to innovate, or (v) to take over the work from original developers (also a type of replacement) to free up the experienced developers for starting new endeavors~\cite{britto2018onboarding}.

Onboarding encompasses the structured or informal process of assimilating newly hired employees, evolving them from ``outsiders'' to valuable contributors within the organization~\cite{bauer2010maximizing}. Onboarding is the essential process through which new team members acclimate to their unfamiliar work environment, develop the required behaviors, attitudes, and skills needed to excel in their new roles, and effectively integrate into the team~\cite{saks2007socialization}. 

Inadequately designed onboarding processes can lead to substantial squandering of company resources and talent and can be a source of frustration for all involved parties. Project managers deal with reduced productivity and need to allocate senior developers' time to mentor newcomers. Senior team members are tasked with conveying substantial information within a limited timeframe. Simultaneously, newcomers confront the challenge of adapting to an entirely new work environment while being aware that they might occasionally disrupt their senior colleagues' workflow when seeking guidance~\cite{pradel2016quantifying}. 

 %This stress can significantly impact a developer's happiness, job retention, and productivity.
\citet{buchan2019effective} agree that a poor onboarding process can lead to anxiety in new team members due to their perceived lack of team contribution and trust. Additionally, it may result in a decline in the team's overall productivity~\cite{rollag2005getting, ju2021case}. 

%When many developers change teams or embark on new positions annually, their initial productivity lag often lasts for months due to the overwhelming nature of onboarding~\cite{rollag2005getting, ju2021case}.

In software companies, dealing with the frequent onboarding of newcomers becomes essential, especially for those with multiple teams or undergoing rapid growth, as highlighted by~\citet{buchan2019effective}. %The swift and efficient onboarding of newcomers can significantly enhance organizational capacity. 
The duration of the onboarding process varies based on factors such as the newcomer's work experience, attitude, and skills, as noted in previous studies~\cite{bauer2011onboarding, kammeyer2003unwrapping}.

%Additionally, the level of support provided to newcomers during the onboarding period influences its duration. 
%Onboarding individuals possessing the requisite skills and compatible personalities is paramount for the prosperity of software development organizations and their projects, as emphasized by~\citet{hall2008}.

%Software companies are perpetually engaged in the pursuit of hiring highly skilled and accomplished individuals to meet the ever-growing demands of their workforce and to stay competitive in the rapidly evolving global market. This diverse spectrum of new hires includes recent college graduates who may lack prior industry exposure and seasoned professional developers with several years of experience, as noted by~\citet{rastogi2017ramp}. 

%\boldification{Boldification: Describe the growing popularity/importance of open source projects and the importance of effective onboarding for their success.}

%\boldification{Boldification: Describe the research gap, emphasizing the lack of a comprehensive understanding of software solutions for onboarding in the context of open source projects}

Previous studies investigated the barriers encountered by newcomers~\cite{steinmacher2015systematic, balali2018newcomers, kaur2022understanding}. These barriers can be minimized through a well-designed onboarding process. In particular, researchers have concentrated on investigating solutions for new contributors within open-source software (OSS) communities~\cite{steinmacher2015systematic, gharehyazie2015developer}. OSS has emerged as a prominent force in the software industry, garnering significant attention since 2003~\cite{von2003special}. The OSS development model is characterized by open access to source code and the possibility for anyone to contribute~\cite{singh2010small}. This collaborative model, reliant on the involvement of geographically dispersed volunteers, emphasizes the crucial role played by newcomers in ensuring the longevity, success, and continuity of OSS projects. Furthermore, active participation in OSS projects not only provides newcomers with opportunities to establish their reputation within the community~\cite{riehle2015open, cai2016reputation} but also contributes to the creation of widely-used software products that benefit society as a whole~\cite{parra2016making}. Additionally, engaging in OSS projects has enhanced newcomers' prospects of achieving professional success~\cite{riehle2015open, greene2016cvexplorer}. 

Enhancing the onboarding experience for newcomers is of paramount importance~\cite{ko2018mining}. %However, the existent literature is scattered across various sources, making it difficult for practitioners to identify and adopt the onboarding process in their projects~\citet{sharma2020exploring}. 
%This research gap requires a comprehensive examination of current software solutions for onboarding to provide practitioners with insights and enable researchers to identify areas that need further attention. This knowledge gap hinders the ability of practitioners and organizations to implement efficient onboarding practices and limits their understanding of the factors that contribute to a smooth onboarding for newcomers. 

%**** The onboarding process entails transmitting knowledge, skills, protocols, and a deep understanding of the organizational culture, enabling them to collaborate within a team effectively~\cite{britto2018onboarding}. 

%, the literature needs a comprehensive synthesis of the software solutions employed in different settings.
%In the rapidly evolving landscape of OSS projects, the need for a consolidated and comprehensive overview of software solutions for newcomers' onboarding has become a significant challenge for practitioners and researchers. 

%\boldification{Boldification: Describe the study motivation for a systematic literature review to bridge the existing knowledge gap and provide insights into effective software solutions for onboarding, Outline the objectives of the review}

Therefore, this study aims to identify the state-of-the-art related to software solutions for newcomers' onboarding by conducting a Systematic Literature Review (SLR). This paper offers a significant contribution in the form of an in-depth analysis of 32 primary studies published until 2023 to advance knowledge in newcomer onboarding in software projects. The insights gained from this study can inform practitioners and researchers working on improving their understanding of the factors contributing to a smooth onboarding for newcomers and provide a basis for further research in this area. 

%This knowledge gap hinders the ability of practitioners and organizations to implement efficient onboarding practices and limits . 

The remainder of this paper is organized as follows. Section~\ref{sec:methodology} details the SLR planning and its execution. Next, Section~\ref{sec:results} presents the results and answers the study research questions. Section~\ref{sec:discussion} outlines the paper discussion, and we provide the study implications on Section~\ref{sec:implications}. The threats to validity are discussed in Section~\ref{sec:threatstovalidity}. In Section~\ref{sec:relatedwork}, we introduce related work. Finally, Section~\ref{sec:conclusion} concludes the work concerning our main findings and suggests future work.


==> OLD_Sections/oldintro18Dec.tex <==
\section{Introduction}
\label{sec:introduction}

%%%%% NEW %%%%%%
%Software is an integral component of a system solution that can be represented as executable instructions for a computer. It encompasses all the requisite documentation for comprehending, modifying, and employing the solution. Notably, one key feature of the software is that it can be complex to build and complex to understand~\cite{basili2005experimental}. The development of software significantly relies on the integration of pre-existing software components, encompassing software libraries, frameworks, database management systems, and even entire software products~\cite{ilin2022framework}.

%%%%%% old intro %%%%%%%

%Onboarding encompasses the structured or informal process of assimilating newly hired employees, evolving them from ``outsiders'' to valuable contributors within the organization~\cite{talya2014onboarding}. Within the software development context, the onboarding of newcomers becomes essential for (i) replacing retired developers, (ii) replacing developers that left or will leave the company, (iii) scaling up the number of developers in response to the growth of the number of customers, (iv) incorporating new people that may bring new ideas and thus help a company to innovate, or (v) taking over the work from original developers (also a type of replacement) free up the experienced developers for starting new endeavors~\cite{britto2018onboarding}.

%Onboarding is the essential process through which newcomers acclimate to their unfamiliar work environment, develop the required behaviors, attitudes, and skills to excel in their new roles, and effectively integrate into the team~\cite{saks2007socialization}. Inadequately designed onboarding processes can lead to substantial squandering of company resources and talent and can be a source of frustration for all involved parties. \citet{buchan2019effective} agree that a poor onboarding process can lead to anxiety in new team members due to their perceived lack of team contribution and trust. Additionally, it may result in a decline in the team's overall productivity~\cite{ju2021case, rollag2005getting}.  

%Previous studies investigated the barriers encountered by newcomers~\cite{balali2018newcomers, kaur2022understanding, steinmacher2015systematic}. For example, newcomers confront the challenge of adapting to an entirely new work environment while being aware that they might occasionally disrupt their senior colleagues' workflow when seeking guidance~\cite{pradel2016quantifying}. A well-designed onboarding process can minimize the barriers. %The barriers can be minimized through a well-designed onboarding process. 
%In particular, researchers have concentrated on investigating solutions for new contributors within open-source software (OSS) communities~\cite{gharehyazie2015developer, steinmacher2015systematic}. OSS has emerged as a prominent force in the software industry, garnering significant attention since 2003~\cite{von2003special}. The OSS development model features open access to source code and allows anyone to contribute %The OSS development model is characterized by open access to source code and the possibility for anyone to contribute 
%~\cite{singh2010small}. This collaborative model, reliant on the involvement of geographically dispersed volunteers, emphasizes the crucial role played by newcomers in ensuring the longevity, success, and continuity of OSS projects. Furthermore, active participation in OSS projects not only provides newcomers with opportunities to establish their reputation within the community~\cite{cai2016reputation, riehle2015open} but also contributes to the creation of widely-used software products that benefit society as a whole~\cite{parra2016making}. Additionally, engaging in OSS projects has enhanced newcomers' prospects of achieving professional success~\cite{greene2016cvexplorer, riehle2015open}. 

%Enhancing the onboarding experience for newcomers is of paramount importance~\cite{ko2018mining}. Therefore, this study aims to identify studies that propose software solutions that facilitate the onboarding processes for newcomers in software projects. We are interested in solutions that minimize the human-burdened interaction. For example, the cost of taking an experienced developer to his tasks to teach a newcomer is high, and sometimes, it is not possible to allocate a senior as a mentor for a long period of time~\cite{PS27malheiros2012source}. Therefore, we focus on capturing software solutions that can support newcomers. These software solutions should be adopted when newcomers face tasks to learn various aspects of software projects, such as documentation, project architecture, the code review process, and testing practices, among others. Software solutions are integral for newcomers to feel comfortable with the new software platform and project processes to acquire the knowledge and resources to be productive and better comprehend their tasks. We conducted a Systematic Literature Review (SLR) to achieve this goal. This paper contributes significantly to a comprehensive analysis of 32 primary studies published until 2023 to advance knowledge in newcomer onboarding in software projects. The insights from this study can inform practitioners and researchers working on improving their understanding of the factors contributing to a smooth onboarding for newcomers and provide a basis for further research in this area. 

%%%%%%%%%%%%%% NEW INTRO %%%%%%%%%%%%%

%onboarding general

Onboarding refers to incorporating new developers into a software development team~\cite{pham2017onboarding, rastogi2017ramp, steinmacher2015systematic, viviani2019reflections}. Onboarding serves as a way to integrate newcomers into the environment so they can understand how to succeed in their position and integrate with their coworkers to work effectively as a team. During this period, developers become familiar with a new project, its source code, and its team~\cite{bauer2011organizational}.

When joining a new software development team for the first time, newcomers must deal with lots of new information in a short time~\cite{sim1998ramp}. In addition to new tasks, development processes, colleagues, and work environments, large and complex source code structures usually need to be understood. Thus, newcomers need significant time before contributing to the project to the best of their ability~\cite{zhou2010developer}. Companies strive to get the most out of their employees, and new team members look to prove themselves in the new setting~\cite{berlin1993beyond}. Inadequately designed onboarding can lead to substantial squandering of company resources and talent and can be a source of frustration for all involved parties. \citet{buchan2019effective} agree that poor onboarding can lead to anxiety in new team members due to their perceived lack of team contribution and trust. Additionally, it may result in a decline in the team's overall productivity~\cite{ju2021case, rollag2005getting}. Therefore, approaches supporting onboarding are desirable to help newcomers and mitigate these problems.

According to~\cite{PS01azanza2021onboarding}, onboarding is becoming increasingly important with a volatile labor and technological market~\cite{bonar1983uncovering, labuschagne2015onboarding, pham2017onboarding}. In particular, open collaboration communities, such as many open source software (OSS) projects, aim to provide environments with low entry barriers to onboarding and retaining newcomers to maintain project sustainability. However, previous work shows that newcomers have been found to face particularly challenging barriers in the OSS context. Social interaction, previous knowledge, finding a way to start, documentation, and technical hurdles are examples of barriers~\cite{steinmacher2015systematic}. Consequently, these barriers posed during the onboarding may lead newcomers to give up on contributing~\cite{steinmacher2015social}. Therefore, investigating how to attract and retain OSS contributors is crucial~\cite{balali2020recommending, guizani2021long, steinmacher2014attracting, steinmacher2015social, PS15steinmacher2016overcoming, trinkenreich2020hidden, zhou2012make}.

Typical onboarding strategies include courses~\cite{pradel2016quantifying, sim1998ramp}, bootcamps~\cite{pham2017onboarding} or mentors~\cite{balali2018newcomers, britto2018onboarding, fagerholm2014onboarding, pham2017onboarding}, where senior developers are appointed to guide newcomers in their onboarding. However, interviewed mentors reported their tasks are tedious and time-consuming~\cite {britto2018onboarding}. These typical onboarding strategies used to support newcomers during the onboarding are known for being costly in terms of time and money. For example, senior developers pointed out that being mentors can impact their productivity~\cite{pham2017onboarding}. Having new hires read relevant source code without assistance is also costly regarding time investment~\cite{basili1997evolving}, leading to long adjustment periods. %Software solutions (e.g., tools) supporting onboarding present opportunities to help newcomers reach confidence in doing their job~\cite{bauer2011organizational} more efficiently.

%mitigating newcomers’ onboarding barriers is crucial, in this sense, researchers have investigated topics such as what motivates newcomers to contribute~\cite{steinmacher2015social, PS15steinmacher2016overcoming}, how to recommend tasks to newcomers~\cite{balali2020recommending}, understanding the roles and activities that are part of the current OSS landscape and the different career pathways~\cite{trinkenreich2020hidden}. 

%Another topic of investigation is how to attract and retain OSS contributors~\cite{steinmacher2014attracting, guizani2021long, zhou2012make}. In this sense, user-friendly tools, safe spaces for newcomers, and positive interactions between newcomers and established community members are promising tools for newcomer retention. 

%Research has found OSS to be a challenging ecosystem to navigate, both for newcomers~\cite{steinmacher2014attracting, steinmacher2015social} and for experienced OSS contributors in large mature organizations~\cite{guizani2021long}. Onboarding an OSS project is a complex, multi-stage process. Newcomers are expected to learn about the project on their own and can feel lost in the complexity of a project~\cite{ducheneaut2005socialization}, pushing newcomers away from the project~\cite{steinmacher2014attracting}. 

%Incorporating a newcomer into a software development team is lengthy, frustrating, and expensive. While it is considered a necessity, it is also very costly and error prone~\cite{bonar1983uncovering, labuschagne2015onboarding, pham2017onboarding}.

%In software projects, onboarding is costly in terms of time and money~\cite{pham2017onboarding}. 
%As a result, most development teams expect newcomers to explore and understand the source code by 


%Newcomers’ seamless onboarding is also essential for open source software (OSS) projects, particularly those that leverage outsiders’ contributions to remain sustainable~\cite{balali2018newcomers}.



%\citet{PS06fu2017expert} states that the rapid growth of software development practices in recent years has been a bonanza for technology diffusion and commercial advantage. These outstanding successes in OSS have mainly involved the cooperation pattern of social-technical interaction and globally distributed fashion. For an OSS project to sustain itself in the long term, it must be able to attract, onboard, and retain newcomers~\cite{zhou2012make}. 

%onboarding osss
%Research has found OSS to be a challenging ecosystem to navigate, both for newcomers~\cite{steinmacher2014attracting, steinmacher2015social} and for experienced OSS contributors in large mature organizations~\cite{guizani2021long}. Previous work shows that the barriers posed during the onboarding may lead newcomers to give up on contributing~\cite{steinmacher2015social}. Onboarding an OSS project is a complex, multi-stage process. Newcomers are expected to learn about the project on their own and can feel lost in the complexity of a project~\cite{ducheneaut2005socialization}, pushing newcomers away from the project~\cite{steinmacher2014attracting}. The barriers related to newcomers’ orientation play a crucial role, especially in keeping the newcomers confident and motivated to continue with the project~\cite{PS15steinmacher2016overcoming}.

%pq software solutions
Enhancing the onboarding experience for newcomers is of paramount importance~\cite{ko2018mining}. Therefore, this study aims to identify studies that propose software solutions (e.g., tools) that facilitate the onboarding of newcomers in software projects~\cite{bauer2011organizational}. Software solutions are integral for newcomers to feel comfortable with the new software platform and project processes to acquire the knowledge and resources to be productive and better comprehend their tasks. Software solutions can actively support aspects such as reducing onboarding time and cost for companies~\cite{PS01azanza2021onboarding}, support independent learning~\cite{viviani2019reflections}, the need for training newcomers in the project specifics~\cite{PS02canfora2012going}, help newcomers to deal with the high amount of information~\cite{PS03cubranic2003hipikat, zhou2012make}, and to support newcomers in understanding complex source code structures~\cite{britto2018onboarding, fagerholm2014onboarding}. %To this end, we advocate using software solutions for onboarding so that the newcomer can explore the software project independently but in a guided manner, making their onboarding experience more efficient and less daunting.

Since a Systematic Literature Review (SLR) objectively summarizes and critically analyzes the available research, we adopted this method to achieve our goal. This paper presents a comprehensive analysis of 32 primary studies published until 2023 to identify the state-of-the-art related software solutions for newcomers' onboarding and to identify potential gaps that can be addressed by developing new software solutions. The insights from this study can inform practitioners and researchers working on improving their understanding of the factors contributing to a smooth onboarding for newcomers and provide a basis for further research in this area.

We have organized the remainder of this paper as follows. Section~\ref{sec:methodology} details the SLR planning and its execution. Next, Section~\ref{sec:results} presents the results and answers the study research questions. Section~\ref{sec:discussion} outlines the paper discussion, and we provide the study implications on Section~\ref{sec:implications}. The threats to validity are discussed in Section~\ref{sec:threatstovalidity}. In Section~\ref{sec:relatedwork}, we introduce related work. Finally, Section~\ref{sec:conclusion} concludes the work concerning our main findings and suggests future work.


==> OLD_Sections/oldmethod.tex <==
   
In this section, we present the critical aspects of the review design. Subsection~\ref{sec:planning} details the SLR protocol used as the basis to conduct our review, emphasizing our research goal translated to Research Questions (RQs) and describes the searching for evidence, selecting relevant articles, extracting and synthesizing data activities, adopted by us to answer the proposed RQs. Figure~\ref{fig:slrprocess} summarizes our study design.

Subsequently, to fine-tune the search string, a pilot search was performed on Google Scholar, and a control group containing a set of five known studies previously established by the authors was created for search string validation.~\cite{wang2011bug, steinmacher2016overcoming, stanik2018simple, heimburger2020gamifying, azanza2021onboarding}. Inclusion and exclusion criteria were applied to select and ensure the relevance of the collected literature. Finally, data were extracted from the selected studies and analyzed/summarized to answer the RQs. 
         
         
\begin{figure}[ht]
\centering
\includegraphics[width=8.5cm]{images/slrprocess.pdf}
\caption{SLR process -- based on~\cite{kitchenham2013systematic}}
\label{fig:slrprocess}
\end{figure}

%%%Katia - Com relação à Figure 1
%%%Katia Deixei alguns exemplos de figura na pasta images (Figures.pptx)


%%%%Phases:
%Planning SLR
 %- Developing the protocol
%Conduncting SLR
 %- Searching for evidence
 %- Selecting relevant articles/primary studies
 %- Extracting data
 %- Synthesizing the data


\subsection{Planning SLR}
\label{sec:planning}
%%%Katia - An SLR begins with a planning phase, which includes the formulation of Research Questions (RQs) and defining search, selection, and extraction/synthesis procedures. 

%%%%Katia
%Sugestão de estruturação: Não separar o planejamento da execução. Se quiser apresentar o protocolo em um documento separado e inserir o link aqui.

%Objective and research questions
%Searching for evidence
%Selecting relevant primary studies
%Extracting data
%Synthesizing the data

\subsubsection{Objective and research questions}
According to \citet{steinmacher2012recommending}, OSS projects are characterized by their self-organization and dynamic nature, involving volunteers from diverse locations who contribute and collaborate on software development. Furthermore, the continuous influx of newcomers and their active participation in development activities play a vital role in the success of these projects~\cite{park2009beyond}. In this context, this SLR aims to identify studies that have proposed technology support strategies to enhance the onboarding processes for newcomers in software projects. To facilitate understanding, we translated our research goal into the following Research Questions (RQs):


\begin{itemize}
    \item \textbf{RQ1:} What technological support strategies are proposed in the literature to facilitate the onboarding of newcomers to software projects?
\end{itemize}

As the field of software development continually evolves, the challenges faced by newcomers during their onboarding process become more pronounced. By answering \textbf{RQ1}, we aim to provide a comprehensive understanding of the existing strategies in supporting newcomers during the onboarding process. It enables effective onboarding, enhances team collaboration, improves newcomer satisfaction and retention, and facilitates knowledge transfer and innovation. By leveraging existing knowledge and common used onboarding practices, organizations can create a smooth onboarding process, promote productivity, and foster a positive team dynamic.

\begin{itemize}
    \item \textbf{RQ2:} How the technological support strategies proposed in the literature to facilitate the onboarding of newcomers to software projects were implemented?
\end{itemize}

While numerous technological strategies have been proposed to enhance newcomers' integration into software projects, understanding the specific implementation details is essential to assess their feasibility, effectiveness, and real-world impact. By answering \textbf{RQ2}, it allows the software development community to identify successful approaches and avoid potential pitfalls when onboarding newcomers to projects and helps identify areas for improvement in onboarding processes, leading to a smoother and more efficient integration of new contributors. Moreover, it helps in optimizing resource allocation to ensure that the chosen strategies are cost-effective and yield the desired results.
    
\begin{itemize}
    \item \textbf{RQ3:} To what extent does the technology support proposed in the literature impact the newcomers' onboarding?
\end{itemize}

Investigating the impact, researchers and practitioners can determine whether the proposed technology support strategies effectively address the challenges faced by newcomers. By answering \textbf{RQ3}, we aim to provide empirical evidence and insights into these strategies in facilitating the onboarding process for newcomers in various software projects. Understanding this impact allows organizations to optimize their onboarding strategies, create a positive onboarding experience, accelerate newcomers' productivity, and foster satisfaction and retention. Additionally, it contributes to the continuous improvement of onboarding practices by advancing field knowledge.

         
\begin{itemize}
    \item \textbf{RQ4:} What evaluation methods were employed in the literature to assess the technology support strategies?
\end{itemize}
    
As the field of newcomer onboarding strategies continues to evolve, it is crucial to identify and evaluate the methodologies used to assess the success and outcomes of these strategies. By addressing \textbf{RQ4}, we aim to provide a comprehensive understanding of the evaluation methods used in existing studies. These results will contribute to the existing body of knowledge by identifying the methods utilized to assess the impact of technology support strategies.

\begin{itemize}
    \item \textbf{RQ5:} How do literature's technological support strategies mitigate newcomers' barriers to joining software \\projects?
\end{itemize}

There is a need to comprehend the practical impact of technological interventions on addressing the barriers that newcomers commonly encounter when trying to integrate into software projects. By focusing on \textbf{RQ5}, our objective is to gain valuable insights into the specific technological support strategies utilized to overcome the challenges and barriers that newcomers often encounter during the onboarding process. Through this investigation, we aim to identify potential gaps in the proposed newcomers onboarding strategies, thereby highlighting the areas that require attention to effectively mitigate the barriers faced by newcomers.

\begin{itemize}
    \item \textbf{RQ6:} To what extent do the technology support strategies proposed in the literature prioritize increasing diversity and inclusion among newcomers?
\end{itemize}

The growing recognition of the importance of diversity and inclusivity in software development communities, highlights the need to explore how the technological strategies outlined in the literature actively address the barriers that underrepresented groups often face when entering software projects. By addressing \textbf{RQ6}, we aim to explore the various technology support strategies that have been proposed to foster a more diverse and inclusive environment for newcomers. We will analyze the existing literature to identify how existing strategies promote the diversity inclusion of newcomers' onboarding. This research endeavor seeks to identify gaps and opportunities in existing approaches to effectively promote diversity and inclusion among newcomers' onboarding strategies. 

%%%Katia - Seguir a ordem do processo de SLR, primero é feita a busca por estudos candidatos, depois a seleção
%Para as subseções, utilizar os mesmos "nomes" das fases que foram usadas na Figura 1. Isso facilita a leitura e mantém a consistência
\subsubsection{Criteria for selection of studies} 
\label{sec:criteriaforselectionofstudies}

%Uma figura ajudaria a visualizar o processo de busca, não?

The strategy to identify potentially relevant studies to answer our RQs is described as follows, we employed two search process approaches. Initially, we conducted queries in digital libraries. However, as discussed in~\cite{steinmacher2015systematic}, relying solely on this approach for SLRs in software engineering can be inefficient. Therefore, we followed the recommendations of previous studies~\cite{jalali2012systematic, kitchenham2013systematic} and implemented additional techniques to enhance our search process. These techniques included single-step citation analysis (forward and backward snowballing) and single-step author snowballing.

The selection criteria were employed to determine the inclusion of publications in the study. Each study was evaluated based on specific criteria that are relevant to the research question defined in our study. To ensure consistency and accuracy, we established clear criteria for the inclusion and exclusion of studies, which are summarized in Table~\ref{tab:iceccriteria}.

Studies were included in the SLR if they met the following inclusion criteria (IC): IC1: The primary study proposes technology support for newcomers' onboarding in software projects. Concerning the exclusion criteria (EC), studies were excluded if: EC1: The study does not have an abstract; EC2: The study is just published as an abstract; EC3: The study is not written in English; EC4: The study is an older version of another study already considered; and EC5: The study is not a scientific study, such as editorials, summaries of keynotes, workshops, and tutorials.

\begin{table}[!ht]\scriptsize
\centering
\caption{Inclusion and exclusion criteria}
\label{tab:iceccriteria}
\begin{tabular}{l}
\hline
\textbf{Inclusion criteria}\\
\hline \hline

\textbf{IC1} --  The primary study proposes technology support for newcomers' onboarding in \\software projects;  \\ \hline \hline 

\textbf{Exclusion criteria}\\
\hline \hline
\textbf{EC1} -- The study does not have an abstract;  \\ \hline
\textbf{EC2} -- The study is just published as an abstract;  \\ \hline
\textbf{EC3} -- The study is not written in English;  \\ \hline
\textbf{EC4} -- The study is an older version of another study already considered;  \\ \hline
\textbf{EC5} -- The study is not a scientific study, such as editorials, summaries of keynotes, \\workshops, and tutorials;  \\ \hline
\end{tabular}
\end{table}


\subsubsection{Search in digital libraries}
\label{sec:searchdigitallibraries}
%... x phases. First of all, we created our search string. The strategy used to construct search terms was composed of four stages:

%Stage 1: Identify the main terms considering the RQs (see Table x -- Line x);
%Stage 2: Identify synonyms or alternative words or abbreviations for principal terms considering keywords found in primary studies (see Table x -- Line x);
%Stage 3: Use the Boolean OR to incorporate synonyms or alternative words or abbreviations (see Table x -- Line x);
%Stage 4: Finally, use the Boolean AND to link the principal terms (see Table x -- Line x);

%Table x: Search String
%Areas 	Keywords
%OSS		....
%...		...
%("..." OR "..." OR "..." ...)
%Search String: ("..." OR "..." OR "..." ...) AND  ("..." OR "..." OR "..." ...)

We employed an SLR method, adhering to well-established guidelines for the Software Engineering (SE) area as proposed by~\cite{keele2007guidelines, kitchenham2013systematic}. Figure~\ref{fig:slrprocess} illustrates the sequential phases and their respective activities encompassing our method. To ensure a comprehensive and well-rounded approach, a panel of three highly experienced researchers, adept at conducting and publishing various empirical studies such as surveys, SLRs, and others in the SE context with a focus on the OSS environment, as well as research related to onboarding and investigating barriers faced by newcomers, came together for a series of five meetings. Throughout these collaborative sessions, the research protocol was meticulously formulated, critically examined, and refined to ensure the study's robustness and effectiveness. 


Furthermore, to ensure the breadth and depth of our investigation, we selected the databases, followed by the execution of the search string. The backward and forward snowballing approach was also carried out, wherein relevant citations within the retrieved studies were examined, along with a proactive pursuit of recent publications that have cited the identified studies~\cite{wohlin2014guidelines}. 

The delineation of textual search strings utilized in the majority of digital libraries assumes paramount importance~\cite{kitchenham2013systematic}. The effectiveness of the searching phase, and consequently the overall SLR, greatly hinges on this crucial aspect. In light of this, we employed the PICOC components, a widely adopted approach for establishing search strings, as outlined by \citet{biolchini2005systematic}. However, for the purpose of our study, we focused solely on the population and intervention components, while omitting the comparison, outcome, and control components~\cite{kitchenham2013systematic}.

In our search string formulation, the population was defined as OSS projects, whereas the intervention component encompassed onboarding newcomers.

technological support strategies aimed at facilitating the onboarding process of newcomers in software projects. By narrowing down our focus to these specific components, we aimed to enhance the relevance of the retrieved literature, thus enabling us to address the research objectives with greater efficacy.

%%%Katia O uso somente da population and intervention caracteriza Mapeamentos Sistemáticos, assim como questões de pesquisas amplas, iniciadas por "Quais, Quantos, Quem"????
%%%Katia População = software projects -- Não seria open source software projects???
         %Intervenção = component encompassed technological support strategies - É isso mesmo? -- Não seria onboarding???
         %A string é formada por apenas um AND, ou seja, tem 2 termos principais.  

Upon careful analysis of terms associated with the population and intervention components, we formulated a set of keywords and their respective synonyms, as detailed in Table~\ref{tab:searchterms}, to construct our search string. The selection of these synonyms was carried out with the assistance of domain experts, and we also drew upon relevant SLR primary studies, which served as control references for our study~\cite{steinmacher2015systematic, kaur2022understanding}, to further enrich our collection of synonyms.

\begin{table}[!ht]\scriptsize
\centering
\caption{Keyword and synonyms used to build search string terms}
\label{tab:searchterms}
\begin{tabular}{l|l}
\hline
\textbf{Keyword}  & \textbf{Synonyms}\\
\hline \hline
OSS & \begin{tabular}[c]{@{}l@{}} OSS, ``open source'', ``open-source'', ``free software'', FOSS, FLOSS, \\``OSS projects'', ``open source software''  \end{tabular} \\
\hline

SE & \begin{tabular}[c]{@{}l@{}} ``Software project'', ``software engineering'', ``software development''\end{tabular} \\
\hline

Onboard & \begin{tabular}[c]{@{}l@{}} Onboarding, onboard, joining, engagement \end{tabular} \\
\hline

Newcomers & \begin{tabular}[c]{@{}l@{}} Newcomer, contributors, novice, newbie,  ``new developer'', \\``early career'', ``new member'', ``new contributor'', ``new people'',\\ beginner, ``potential participant'', joiner, ``new committer'' \end{tabular} \\
\hline
\hline
\end{tabular}
\end{table}

Based on the terms presented in Table~\ref{tab:searchterms}, a comprehensive and generic search string was formulated as follows: \textit{(``open source''  OR  ``open-source''  OR  ``free software''  OR  FOSS  OR  FLOSS  OR  OSS  OR  ``OSS projects''  OR  ``open source software''  OR  ``software project''  OR  ``software engineering''  OR  ``software development'') AND (``joining process''  OR  onboarding  OR  onboard  OR  joining  OR  engagement  OR  newcomer  OR  novice  OR  newbie  OR  ``new developer''  OR  ``early career''  OR  ``new member''  OR  ``new contributor''  OR  beginner  OR  ``potential participant''  OR  joiner  OR  entrance)}. 

This search string was derived after numerous trials and iterations, taking into account the studies established as the control group. During the refinement process, certain synonyms were excluded, either due to the absence of relevant primary studies associated with those terms or because the search results yielded an excessive number of studies that, upon skimming their titles, were deemed to be outside the scope of this SLR (e.g., ``first steps'', ``initial steps'', attrac*, contributing). Furthermore, the effectiveness of the search string was continuously assessed to ensure its ability to retrieve the studies established as part of the control group. By employing this approach, we aimed to strike a balance between inclusivity and precision, ensuring that the search string captures the relevant literature while avoiding an overwhelming number of irrelevant or tangential studies.

%Once the search string was established, we proceeded to define the criteria for selecting appropriate digital libraries, as recommended in~\cite{steinmacher2015systematic}. These criteria included the following requirements: the digital libraries should index primary studies pertaining to open source software research, be predominantly in the English language, support searching using Boolean expressions, and provide access to the complete texts of the primary studies. Guided by these criteria, we identified and selected four prominent digital libraries to conduct our comprehensive search, namely the ACM Digital Library~\footnote{http://portal.acm.org}, IEEE Digital Library~\footnote{http://ieeexplore.ieee.org}, Scopus~\footnote{http://www.scopus.com}, Springer Link~\footnote{https://link.springer.com/}, and Web of Science~\footnote{https://www.webofscience.com/wos/woscc/basic-search}. These chosen digital libraries not only meet the aforementioned criteria but also possess a rich collection of scholarly works relevant to our research inquiry.
%%%Katia Daria para ampliar os critérios de seleção de fontes?


After defining the search terms, identifying relevant literature was started. We choose the databases based on predefined criteria, such as: (i) coverage (a large number of conferences proceedings, journals, and indexed books); (ii) content update (publications are regularly updated); (iii) availability (full text of the primary studies are available); (iv) quality of results (accuracy of the results obtained by the search); and (v) versatility export (a mechanism to export the results of the search is available). The most commonly used databases in SE area that meet the characteristics described above are: IEEE xplore~\footnote{http://ieeexplore.ieee.org}, ACM digital library~\footnote{http://portal.acm.org}, Scopus~\footnote{http://www.scopus.com}, Springer link~\footnote{https://link.springer.com/}, and Web of science~\footnote{https://www.webofscience.com/wos/woscc/basic-search}.


Table~\ref{tab:searchstring} showcases the search strings employed in each search engine for this study. The data collection process took place during the first semester of 2023, resulting in the retrieval of a substantial number of 9734 primary studies. Specifically, a total of 7489 candidate primary studies were identified and included in our analysis.

 

\begin{table*}[!ht]\scriptsize
\centering
\caption{Search strings}
\label{tab:searchstring}
\begin{tabular}{l|l|l}
\hline
\textbf{Database}  & \textbf{Search string} & \textbf{Total}\\
\hline \hline
ACM & \begin{tabular}[c]{@{}l@{}} Abstract:("open source"  OR  "open-source"  OR  "free software" OR  FOSS  OR  FLOSS  OR  OSS  OR  "OSS projects"  OR  "open source software"  OR\\  "software project"  OR  "software engineering"  OR  "software development") AND Abstract:("joining process"  OR  onboarding  OR  onboard  OR  joining\\  OR  engagement  OR  newcomer  OR  novice  OR  newbie  OR  "new developer"  OR  "early career"  OR  "new member"  OR  "new contributor" OR  beginner  \\OR  "potential participant"  OR  joiner  OR  entrance) \end{tabular} & 1069 \\
\hline

IEEE & \begin{tabular}[c]{@{}l@{}} (("Abstract":"open source" OR "Abstract":"open-source" OR "Abstract":"free software" OR "Abstract":"FOSS" OR "Abstract":"FLOSS" OR \\"Abstract":"OSS" OR "Abstract":"OSS projects" OR "Abstract":"open source software" OR "Abstract":"software project" OR\\ "Abstract":"software engineering" OR "Abstract":"software development") AND ("Abstract":"joining process" OR "Abstract":"onboarding" OR\\ "Abstract":"onboard" OR "Abstract":"joining" OR "Abstract":"engagement" OR "Abstract":"newcomer" OR "Abstract":"novice" OR\\ "Abstract":"newbie" OR "Abstract":"new developer" OR "Abstract":"early career" OR "Abstract":"new member" OR\\ "Abstract":"new contributor" OR "Abstract":"beginner" OR "Abstract":"potential participant" OR "Abstract":"joiner" OR "Abstract":"entrance")) \end{tabular} & 726 \\
\hline

Scopus & \begin{tabular}[c]{@{}l@{}} TITLE-ABS-KEY ( ( "open source"  OR  "open-source"  OR  "free software"  OR  FOSS  OR  FLOSS*  OR  OSS  OR  "OSS projects"  OR  "open source software"\\  OR  "software project"  OR  "software engineering"  OR  "software development" )  AND  ( "joining process"  OR  onboarding  OR  onboard  OR  joining\\  OR engagement  OR  newcomer  OR  novice  OR  newbie  OR  "new developer"  OR  "early career"  OR  "new member"  OR  "new contributor"  OR\\  beginner  OR  "potential participant"  OR  joiner  OR  entrance ) )  AND  ( LIMIT-TO ( SUBJAREA ,  "COMP" ) )  AND\\  ( LIMIT-TO ( LANGUAGE ,  "English" ) ) \end{tabular} & 3019 \\
\hline

Springer link & \begin{tabular}[c]{@{}l@{}} ("open source"  OR  "open-source"  OR  "free software"  OR  FOSS  OR  FLOSS*  OR  OSS  OR  "OSS projects"  OR  "open source software"  OR  "software project"\\  OR  "software engineering"  OR  "software development") AND ("joining process"  OR  onboarding  OR  onboard  OR  joining  OR  engagement  OR\\  newcomer  OR  novice  OR  newbie  OR  "new developer"  OR  "early career"  OR  "new member"  OR  "new contributor"  OR  beginner  OR\\  "potential participant"  OR  joiner  OR  entrance) \end{tabular} & 2554 \\
\hline

Web of science & \begin{tabular}[c]{@{}l@{}} (AB=("open source"  OR  "open-source"  OR  "free software"  OR  FOSS  OR  FLOSS*  OR  OSS  OR  "OSS projects"  OR  "open source software"  OR\\  "software project"  OR  "software engineering"  OR  "software development")) AND AB=("joining process"  OR  onboarding  OR  onboard  OR  joining  OR\\  engagement  OR  newcomer  OR  novice  OR  newbie  OR  "new developer"  OR  "early career"  OR  "new member"  OR  "new contributor"  OR  beginner  OR\\  "potential participant"  OR  joiner  OR  entrance) \end{tabular} & 2364 \\ \hline

 & \begin{tabular}[c]{@{}l@{}} \textbf{TOTAL} \end{tabular} & \textbf{9734} \\ \hline

 & \begin{tabular}[c]{@{}l@{}} \textbf{DUPLICATED} \end{tabular} & \textbf{2243} \\ \hline

 & \begin{tabular}[c]{@{}l@{}} \textbf{INITIAL SET} \end{tabular} & \textbf{7489} \\ \hline

\hline \hline
\end{tabular}
\end{table*}

In addition to our search in the selected digital libraries, we sought the guidance of various experts to identify recommended venues for studies pertinent to our research. These specialists shared valuable insights by suggesting a range of conferences, workshops, journals, and specialized websites known for their relevance in the field. Notably, the majority of these recommended venues were already indexed by the digital libraries we had initially chosen. However, it is important to highlight that certain suggested venues were excluded from our selection due to specific criteria employed for source evaluation. For example, conferences conducted in languages other than English, search engines that did not support searching using Boolean expressions were excluded, as they did not align with our research objectives and grey literature. Consequently, our final selection of sources comprised those that met the predetermined criteria, ensuring the inclusion of high-quality and relevant literature in our analysis.
%%%Katia that certain suggested venues were excluded ... quais?


\subsubsection{Snowballing approach} 

In addition to querying the digital libraries, we utilized an iterative step snowballing approach, implementing two distinct approaches. The first approach involved a thorough investigation of whether the authors of the selected studies had published any additional relevant studies that were not captured by the digital libraries. To identify these additional publications, we extensively examined the authors' profiles within the ACM and IEEE libraries, while also consulting their DBLP~\footnote{https://dblp.org/} profiles and personal homepages, whenever accessible.

The second approach employed backward snowballing approach. We scrutinized the reference lists of all the selected primary studies to identify any other potential studies of relevance. It is worth noting that we did not limited the snowballing approach to a single level; thus, we kept pursuing additional snowballing approach for studies discovered through previous iterations.
%%%Katia 
%Em relação ao snowballing, fiquei com as seguintes dúvidas:
%Como foi conduzido o snowballing?
%1) Pesquisa automatizada (string de pesquisa) seguida por Snowballing para Trás (BS) e Snowballing para Frente (FS) completos? Esse é o snowballing clássico sugerido em Claes Wohlin - Guidelines for Snowballing in Systematic Literature Studies and a Replication in Software Engineering
%2) Pesquisa automatizada (string de pesquisa/Google Scholar?) seguida de BS e FS em paralelo?
%3) Pesquisa automatizada (string de pesquisa) seguida por BS e depois FS?
%4) Pesquisa automatizada (string de pesquisa) seguida por FS e depois BS?
%Quantas rodadas foram realizadas?
%Sugiro a leitura do artigo "Successful Combination of Database Search and Snowballing for Identification of Primary Studies in Systematic Literature Studies" para esclarecimentos.

Both approaches were implemented until reaching saturation, whereby no further paper retrieval was possible. By employing these comprehensive snowballing approach, we aimed to optimize the breadth of our literature search and ensure the inclusion of all pertinent studies in our analysis.


\subsubsection{Control group}
%%%Katia Grupo de controle foi usado na busca automática, essa subseção é sobre snowballing. Não misturar.

In order to validate the keywords utilized in formulating the search string, we performed exploratory searches using Google Scholar. This process allowed us to fine-tune the inclusion and exclusion criteria, refine the research question, identify synonyms for the search string, and establish an information extraction template. Drawing from the insights gained during these exploratory searches and leveraging our expertise in the field, we selected five prominent and pertinent studies to serve as control primary studies~\cite{wang2011bug, steinmacher2016overcoming, stanik2018simple, heimburger2020gamifying, azanza2021onboarding}. During the pilot studies aimed at testing the protocol, all five control primary studies were successfully retrieved:

\begin{itemize}
    \item \citet{wang2011bug} --  Which bug should I fix: helping new developers onboard a new project;
    
    \item \citet{steinmacher2016overcoming} -- Overcoming open source project entry barriers with a portal for newcomers;
    
    \item \citet{stanik2018simple} -- A simple nlp-based approach to support onboarding and retention in open source communities;

    \item \citet{heimburger2020gamifying} -- Gamifying onboarding: How to increase both engagement and integration of new employees;

    \item \citet{azanza2021onboarding} -- Onboarding in software product lines: Concept maps as welcome guides.
\end{itemize}



\subsection{Conducting SLR}

\subsubsection{Study selection}
%%%Katia - Exemplo de descrição de um processo de seleção. Sempre começar descrevendo o total de fases, o objetivo de cada fase, quem fez o que ...
%The study selection activity was conducted in five phases. During phase 1, the first (second ...) author applied the search strategy to identify potentially relevant studies. Duplicate papers were excluded. After this, in phase 2, xx other researchers screened the titles and abstracts to decide whether to include or exclude a study. The full texts of these papers were read independently by the researchers, and the disagreements were resolved by consensus. Therefore, in phase 3, the full text of the primary studies included in the preliminary selection was obtained. The first (second ...) author read in detail the full text of each primary study included in the preliminary selection to decide whether to include or exclude the study. The same studies were analyzed by one other researcher, who independently read the papers, and again disagreements were resolved by discussion and consensus. The studies included in the final selection correspond to the relevant articles that meet the RQ addressed by this SLR. During phase 4, the studies were reviewed to ensure that relevant studies were not eliminated. Finally, during phase 5, the included studies’ quality was assessed.

We utilized the query outlined in Section~\ref{sec:searchdigitallibraries} to retrieve candidate primary studies from the digital library systems in January 2023, as depicted in Figure~\ref{fig:selectionprocess}. Our search across the five selected digital libraries yielded a total of 9,732 primary studies. Subsequently, we removed 2,243 duplicate primary studies, resulting in an initial set of 7,489 unique primary studies to commence the selection process. Notably, we employed the Parsifal~\footnote{https://parsif.al/} tool, developed by~\citet{kitchenham2007guidelines}, to facilitate the SLR process.

\begin{figure}[ht]
\centering
\includegraphics[width=8.5cm]{images/selectionprocess.pdf}
\caption{Paper selection process overview}
\label{fig:selectionprocess}
\end{figure}

Subsequently, we employed the criteria outlined in Section~\ref{sec:criteriaforselectionofstudies} to select the studies. In the following, we provide a comprehensive account of the results obtained through the execution of the study selection steps.

\begin{enumerate}
    \item \textbf{Search in digital libraries:} We initiated our search by querying digital libraries, storing the references of retrieved studies in a local repository for subsequent analysis. The initial set consisted of 7489 primary studies;

    %%%Katia - Não foi mencionado anteriormente os campos que seriam lidos. Nem quantos revisores participariam do processo de seleção. E no caso de dúvidas? O que foi feito?
    \item \textbf{Title, abstract, and keywords analysis:} Titles, abstracts, and keywords of the primary studies were meticulously reviewed to assess their adherence to the inclusion and exclusion criteria. This analysis resulted in the inclusion of 1049 primary studies;

    \item \textbf{Introduction analysis:} The initial sections of the selected studies were evaluated to examine their objectives and results. This analysis allowed us to determine whether the primary studies addressed the research question and met the inclusion and/or exclusion criteria. As a result, 314 primary studies were included;

    \item \textbf{Conclusion analysis:} The closing sections of the studies were scrutinized in terms of their objectives and outcomes. In cases where the assessment based on the introduction and conclusion was inconclusive, the entire paper was thoroughly examined to make a definitive decision regarding its inclusion or exclusion. This process led to the inclusion of 43 primary studies;

    %%%Katia Robustez???
    %%%Katia works? studies? papers? articles? 
    % three experienced researchers, no que é a experiência deles?
    \item \textbf{Quality assessment:} To ensure the robustness of the selected works, meetings were conducted with three experienced researchers who individually reviewed each paper, discussing its objectives and results. Based on this assessment, 25 primary studies were included to meet the desired quality criteria;

    \item \textbf{Author snowballing:} The 25 primary studies selected in the previous step underwent further analysis by investigating the authors associated with them. We searched for other primary studies published by these authors and subjected the candidate primary studies to the same screening process used for primary studies obtained from digital libraries \textit{(steps 2 to 5)}. This iterative author snowballing procedure involved four rounds and as a result five (5) primary studies were included; 

    \item \textbf{Forward and backward snowballing:} The studies obtained through digital library searches and author snowballing were further analyzed with respect to their reference lists. Candidate primary studies identified from these references underwent the same screening process as those obtained from digital libraries and author snowballing \textit{(steps 2 to 5)}. We performed four rounds of forward and backward snowballing and we were able to include 8 primary studies.    
    %%%Katia Author, Backward and Forward snowballing? É isso mesmo? 
\end{enumerate}



\subsubsection{Quality assessment of the studies selected}

After conducting the snowballing process, our research team performed a comprehensive analysis of all 38 primary studies included in the study. The quality assessment of the primary studies was conducted using a predefined set of questions outlined in Table~\ref{tab:qualityassesment}. These questions were carefully designed and tailored to our research objectives, aiming to evaluate various aspects of each study. Each question was answered based on a thorough examination of the paper content. Furthermore, we employed a numeric scale for scoring, where "yes" responses were assigned 1 point and "no" responses received 0 points. This scoring system allowed for a maximum score of 8 points and a minimum score of 0 points to be assigned to each study, reflecting their overall quality assessment.
%%%Katia ... evaluate various aspects of each study. --> Não deixar sentenças vagas. Quais aspectos?

\begin{table}[!ht]\scriptsize
\centering
\caption{Study quality assessment.}
\label{tab:qualityassesment}
\begin{tabular}{l|l|l|l}
\hline
\textbf{ID} & \textbf{Criteria} & \textbf{Y} & \textbf{N} \\
\hline \hline
1  & \begin{tabular}[c]{@{}l@{}}Is there a rationale for why the study was undertaken? \cite{mahdavi2013variability}\end{tabular} & 1 & 0 \\ \hline

2 & \begin{tabular}[c]{@{}l@{}}Is the paper based on research (or is it merely a ``lessons learned'' \\report based on expert opinion)?  \cite{dybaa2008empirical}\end{tabular} & 1 & 0 \\ \hline

3 & \begin{tabular}[c]{@{}l@{}}Is there a clear statement of the goals of the study? \cite{dybaa2008empirical}\end{tabular} & 1 & 0 \\ \hline

4 & \begin{tabular}[c]{@{}l@{}}Is the proposed technological support clearly described? \cite{achimugu2014systematic}\end{tabular} & 1 & 0 \\ \hline

5 & \begin{tabular}[c]{@{}l@{}}Is there an adequate description of the context (industry, \\laboratory setting, products used and so on) in which the \\research was carried out? \cite{dybaa2008empirical,mahdavi2013variability}\end{tabular} & 1          & 0         \\ \hline

6 & \begin{tabular}[c]{@{}l@{}}Is the study supported by a tool? \cite{dermeval2014systematic}\end{tabular} & 1 & 0 \\ \hline

7 & \begin{tabular}[c]{@{}l@{}}Is there a discussion about the results of the study? \cite{dermeval2014systematic}\end{tabular} & 1 & 0 \\ \hline

8 & \begin{tabular}[c]{@{}l@{}}Are the limitations explicitly discussed? \cite{ding2014knowledge}\end{tabular} & 1 & 0 \\ \hline

\multicolumn{4}{l}{\textbf{Key:} Y= Yes; N= Not.} \\ \hline

\end{tabular}
\end{table}

To determine the inclusion of studies, we employed the first quartile approach, setting the cutoff point at 2.0, as recommended by~\citet{usman2014effort}. Consequently, studies scoring below 2 points were excluded due to their lack of quality in the context of this research. As a result of the quality assessment, 7 out of the initial 38 primary studies, which were included after the full-text reading, were eliminated. Consequently, data extraction and analysis were performed on a total of 31 selected studies.
%%%Katia ... Criar uma tabela destacando os estudos excluídos por qualidade.
%(see Table~\ref{tab:liststudies}).

\subsection{Data extraction}

Quantitative and qualitative data were extracted from the selected primary studies to comprehensively analyze the literature on technological support strategies for facilitating newcomers' onboarding in software projects. The quantitative analysis allowed us to examine the findings and trends reported in the literature. Additionally, a qualitative analysis was conducted, employing an inductive approach inspired on open coding and axial coding procedures from Grounded Theory (GT)~\cite{corbin2008techniques} to establish data categories and systematically organize the insights provided by the literature regarding onboarding strategies. Although the purpose of the GT method is the construction of substantive theories, according to Corbin and Strauss~\cite{corbin2008techniques}, the researcher may use only some of its procedures to meet one’s research goals. Throughout the process of addressing each research question, specific data properties were defined and consistently extracted from all relevant publications. Table~\ref{tab:dataextraction} presents a detailed list of the data items that were extracted from the selected primary studies, categorized according to each research question.

\begin{table}[!ht]\scriptsize
\centering
\caption{Data extraction form}
\label{tab:dataextraction}
\begin{tabular}{l}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Information extracted\end{tabular}} \\
\hline \hline

\begin{tabular}[c]{@{}l@{}}Author affiliations and countries\end{tabular} \\ \hline

\begin{tabular}[c]{@{}l@{}}Publication type (journal, conference, or workshop)\end{tabular} \\ \hline

\begin{tabular}[c]{@{}l@{}}Study identifier (PS01, PS02, PS03, ...)\end{tabular} \\ \hline


\begin{tabular}[c]{@{}l@{}}Study metadata (title, authors, year) \end{tabular} \\ \hline


\begin{tabular}[c]{@{}l@{}}Keywords\end{tabular} \\ \hline

\textbf{\begin{tabular}[c]{@{}l@{}}Research question\end{tabular}} \\

\hline \hline

\begin{tabular}[c]{@{}l@{}}Type of technology support\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Onboarding strategies\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Effects of onboarding strategies\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Onboarding barrier\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Onboarding strategies evaluation\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Type of analysis\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Target population\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Focused in diversity and inclusion aspects\end{tabular}  \\ \hline

\begin{tabular}[c]{@{}l@{}}Study findings\end{tabular}  \\ \hline

\end{tabular}
\end{table}

%%%Katia PAREI AQUI!





\subsection{Overview of the studies}

Table~\ref{tab:liststudies} presents the 31 studies that were selected for analysis, along with their respective identifiers. In this paper, we consistently refer to these chosen primary studies using the abbreviation 'PS' (e.g., (PS1)).

\begin{table*}[!ht]\scriptsize
\centering
\caption{List of studies selected}
\label{tab:liststudies}
\begin{tabular}{cllc}
\hline
\textbf{ID} & \textbf{Reference} & \textbf{Title} & \textbf{\begin{tabular}[c]{@{}c@{}}Public. \\year\end{tabular}}\\
\hline \hline

PS01 & \begin{tabular}[c]{@{}l@{}}\citet{PS01azanza2021onboarding}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Onboarding in Software Product Lines: Concept Maps as Welcome Guides \end{tabular} & 2021 \\ \hline

PS02 & \begin{tabular}[c]{@{}l@{}}\citet{PS02canfora2012going}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Who is Going to Mentor Newcomers in Open Source Projects? \end{tabular} & 2012 \\ \hline

PS03 & \begin{tabular}[c]{@{}l@{}}\citet{PS03cubranic2003hipikat}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Hipikat: Recommending pertinent software development artifacts \end{tabular} & 2003 \\ \hline

PS04 & \begin{tabular}[c]{@{}l@{}}\citet{PS04diniz2017using}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Using Gamification to Orient and Motivate Students to Contribute to OSSprojects \end{tabular} & 2017 \\ \hline

PS05 & \begin{tabular}[c]{@{}l@{}}\citet{PS05dominic2020conversational}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Conversational Bot for Newcomers Onboarding to Open Source Projects \end{tabular} & 2020 \\ \hline

PS06 & \begin{tabular}[c]{@{}l@{}}\citet{PS06fu2017expert}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Expert Recommendation in OSS Projects Based on Knowledge Embedding \end{tabular} & 2017 \\ \hline

PS07 & \begin{tabular}[c]{@{}l@{}}\citet{PS07guizani2022attracting}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Attracting and Retaining OSS Contributors with a Maintainer Dashboard \end{tabular} & 2022 \\ \hline

PS08 & \begin{tabular}[c]{@{}l@{}}\citet{PS08he2022gfi}\end{tabular} & \begin{tabular}[c]{@{}l@{}} GFI-bot: automated good first issue recommendation on GitHub \end{tabular} & 2022 \\ \hline

PS09 & \begin{tabular}[c]{@{}l@{}}\citet{PS09kagdi2008can}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Who can help me with this source code change? \end{tabular} & 2008 \\ \hline

PS10 & \begin{tabular}[c]{@{}l@{}}\citet{PS10medeiros2022assisting}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Assisting Mentors in Selecting Newcomers' Next Task in Software ProductLines: A Recommender System Approach \end{tabular} & 2022 \\ \hline

PS11 & \begin{tabular}[c]{@{}l@{}}\citet{PS11nagel2021ontology}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Ontology-Based Software Graphs for Supporting Code Comprehension During Onboarding \end{tabular} & 2021 \\ \hline

PS12 & \begin{tabular}[c]{@{}l@{}}\citet{PS12sarma2016training}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Training the Future Workforce through Task Curation in an OSS Ecosystem \end{tabular} & 2016 \\ \hline

PS13 & \begin{tabular}[c]{@{}l@{}}\citet{PS13serrano2022find}\end{tabular} & \begin{tabular}[c]{@{}l@{}} How to Find My Task? Chatbot to Assist Newcomers in Choosing Tasks inOSS Projects \end{tabular} & 2022 \\ \hline

PS14 & \begin{tabular}[c]{@{}l@{}}\citet{PS14stanik2018simple}\end{tabular} & \begin{tabular}[c]{@{}l@{}} A Simple NLP-Based Approach to Support Onboarding and Retention in Open Source Communities \end{tabular} & 2018 \\ \hline

PS15 & \begin{tabular}[c]{@{}l@{}}\citet{PS15steinmacher2016overcoming}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Overcoming Open Source Project Entry Barriers with a Portal for Newcomers \end{tabular} & 2016 \\ \hline

PS16 & \begin{tabular}[c]{@{}l@{}}\citet{PS16steinmacher2012recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending Mentors to Software Project Newcomers \end{tabular} & 2012 \\ \hline

PS17 & \begin{tabular}[c]{@{}l@{}}\citet{PS17toscani2018gamification}\end{tabular} & \begin{tabular}[c]{@{}l@{}} A Gamification Proposal to Support the Onboarding of Newcomers in the FLOSScoach Portal \end{tabular} & 2015 \\ \hline

PS18 & \begin{tabular}[c]{@{}l@{}}\citet{PS18wang2011bug}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Which bug should I fix: Helping new developers onboard a new project \end{tabular} & 2011 \\ \hline

PS19 & \begin{tabular}[c]{@{}l@{}}\citet{PS19xiao2022recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending Good First Issues in GitHub OSS Projects \end{tabular} & 2022 \\ \hline

PS20 & \begin{tabular}[c]{@{}l@{}}\citet{PS20yin2021automatic}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Automatic learning path recommendation for open source projects using deep learning on knowledge graphs \end{tabular} & 2021 \\ \hline

PS21 & \begin{tabular}[c]{@{}l@{}}\citet{PS21ford2022reboc}\end{tabular} & \begin{tabular}[c]{@{}l@{}} ReBOC: Recommending Bespoke Open Source Software Projects to Contributors \end{tabular} & 2022 \\ \hline

PS22 & \begin{tabular}[c]{@{}l@{}}\citet{PS22liu2018recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending GitHub Projects for Developer Onboarding \end{tabular} & 2018 \\ \hline

PS23 & \begin{tabular}[c]{@{}l@{}}\citet{PS23santos2023designing}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Designing for Cognitive Diversity: Improving the GitHub Experience for Newcomers \end{tabular} & 2023 \\ \hline

PS24 & \begin{tabular}[c]{@{}l@{}}\citet{PS24santos2021can}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Can i solve it? identifying apis required to complete oss tasks \end{tabular} & 2021 \\ \hline

PS25 & \begin{tabular}[c]{@{}l@{}}\citet{PS25minto2007recommending}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Recommending Emergent Teams \end{tabular} & 2007 \\ \hline

PS26 & \begin{tabular}[c]{@{}l@{}}\citet{PS26heimburger2020gamifying}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Gamifying onboarding: How to increase both engagement and integration of new employees \end{tabular} & 2020 \\ \hline

PS27 & \begin{tabular}[c]{@{}l@{}}\citet{PS27malheiros2012source}\end{tabular} & \begin{tabular}[c]{@{}l@{}} A source code recommender system to support newcomers \end{tabular} & 2012 \\ \hline

PS28 & \begin{tabular}[c]{@{}l@{}}\citet{PS28yang2016repolike}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Repolike: personal repositories recommendation in social coding communities \end{tabular} & 2016 \\ \hline

PS29 & \begin{tabular}[c]{@{}l@{}}\citet{PS29zhou2021ghtrec}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Ghtrec: a personalized service to recommend github trending repositories for developers \end{tabular} & 2021 \\ \hline

PS30 & \begin{tabular}[c]{@{}l@{}}\citet{PS30venigalla2022gitq}\end{tabular} & \begin{tabular}[c]{@{}l@{}} GitQ-towards using badges as visual cues for GitHub projects \end{tabular} & 2022 \\ \hline

PS31 & \begin{tabular}[c]{@{}l@{}}\citet{PS31sun2018personalized}\end{tabular} & \begin{tabular}[c]{@{}l@{}} Personalized project recommendation on GitHub \end{tabular} & 2018 \\ \hline

\end{tabular}
\end{table*}



==> OLD_Sections/oldrqs.tex <==

\section{Results}
\label{sec:results}


\subsection{RQ1: Technological support strategies for newcomer onboarding}

Based on the analysis of the selected primary studies, we have identified various technological support strategies proposed to enhance the onboarding process for newcomers in software projects. These strategies have been categorized and presented in Table~\ref{tab:onboardstrategies}.


\begin{table}[!bt]\scriptsize
\centering
\caption{Enhancing technological support strategies for newcomers onboarding}
\label{tab:onboardstrategies}
\begin{tabular}{c|c|l|c}
\hline
\textbf{Categories} & \textbf{Approach} & \multicolumn{1}{c|}{\textbf{Description}} & \textbf{\begin{tabular}[c]{@{}c@{}}Study \\ reference\end{tabular}} \\ \hline \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Redesign \\ environment\end{tabular}} & Gamification & \begin{tabular}[c]{@{}l@{}}Applying gamification to \\ enhance newcomer enga-\\ gement and motivation \\ in software projects.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS04, \\ PS17, PS26\end{tabular} \\ \cline{2-4} 
 & \begin{tabular}[c]{@{}c@{}}Modify \\ GitHub \\ interface\end{tabular} & \begin{tabular}[c]{@{}l@{}}Modifying newcomers' \\ interaction with the OSS \\ project environment.\end{tabular} & PS23, PS30 \\ \hline

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Project \\ knowledge \\ representation\end{tabular}} & Dashboard & \begin{tabular}[c]{@{}l@{}}Dashboard to support \\ community managers to \\ track and acknowledge \\ newcomers’ contributions.\end{tabular} & PS07 \\ \cline{2-4} 
 & \begin{tabular}[c]{@{}c@{}}Dynamic \\ documentation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Guiding newcomers by \\ structuring existing \\ project documents.\end{tabular} & PS15 \\ \cline{2-4} 
 & \begin{tabular}[c]{@{}c@{}}Visualization \\ tool\end{tabular} & \begin{tabular}[c]{@{}l@{}}Graphical tools for \\ organising and repre-\\ senting knowledge.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS01, PS11, \\ PS18, PS20\end{tabular} \\ \hline

\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Recommendation \\ system\end{tabular}} & Issue label & \begin{tabular}[c]{@{}l@{}}Recommending initial \\ tasks or issues for new-\\ comers to work on in \\ OSS projects.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS07, PS08, \\ PS14, PS19, \\PS24\end{tabular} \\ \cline{2-4} 
 & \begin{tabular}[c]{@{}c@{}}Mentor/\\ expert\end{tabular} & \begin{tabular}[c]{@{}l@{}}Facilitating interaction \\ between newcomers \\ and experienced mentors \\ in software projects.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS02, PS06, \\ PS09, PS16, \\ PS25\end{tabular} \\ \cline{2-4} 
 & Project & \begin{tabular}[c]{@{}l@{}}Recommending suitable \\ projects or tasks for \\ newcomers based on \\ their skills and interests.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS05, PS21, \\ PS22, PS28, \\ PS29, PS31\end{tabular} \\ \cline{2-4} 
 & Source files & \begin{tabular}[c]{@{}l@{}}Recommending source \\ code files for newcomers \\ to explore and integrate \\ into projects.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS03, PS10, \\ PS20, PS27\end{tabular} \\ \cline{2-4} 
 & SPL feature & \begin{tabular}[c]{@{}l@{}}Recommending specific \\ features within a software \\ product line for newco-\\ mers to contribute to.\end{tabular} & PS10 \\ \cline{2-4} 
 & Task/bug & \begin{tabular}[c]{@{}l@{}}Recommending relevant \\ tasks or bugs for new-\\ comers to tackle in soft-\\ ware projects.\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS12, \\PS13, PS18\end{tabular} \\ \hline \hline
\end{tabular}
\end{table}


We have identified three primary overarching categories encompassing the technological support strategies for newcomers during the onboarding process:

\textbf{Redesign environment.} This category involves the strategic modification of the project environment to optimize the interactions and experiences of newcomers during the onboarding process. It aimed to create an environment that is conducive to effective integration and engagement. Strategies within this category often include the implementation of gamification (PS04, PS17, PS26), which introduce game-like elements to enhance newcomers' motivation, participation, and learning within the project context. In PS04, the objective was to analyze the use of gamification, to achieve this, the authors selected four game design elements - Rankings, Quests, Points, and Levels - and defined a set of rules to describe the operation of the gamified environment. These elements were implemented on GitLab to provide support and encouragement to students. PS17 proposed and evaluated a gamified version of the FLOSScoach portal, aiming to motivate newcomers to contribute to OSS projects. The authors selected eight game elements - Gameboard, Unlocking, Tips, Badges, Forum, Voting, Profile, and Leaderboard - and strategically integrated them throughout the contribution flow represented in FLOSScoach. PS26 described a mobile onboarding application specifically developed for the younger generations Y and Z, with a focus on gamification. The study analyzed how incorporating game elements into non-gaming situations, such as work contexts, can enhance onboarding processes. By enriching tedious tasks, motivating employees, alleviating stress in social situations, and fostering playful learning, gamification has the potential to positively impact onboarding experiences.

Additionally, this category may encompass alterations to the project infrastructure itself (PS23, PS30), such as platform modifications or interface enhancements, with the goal of creating a more user-friendly and welcoming atmosphere for newcomers. PS23 evaluated GitHub and identify inclusivity bugs that affect newcomers to the platform. The authors analyzed four common tasks that newcomers perform when making their first pull request on GitHub and discovered inclusivity bugs in each of them. To address these issues, a redesign of the GitHub environment was proposed, and a web browser plugin was developed to modify the platform interface and fix the identified bugs. PS30 developed GitQ, which include badges to GitHub providing visual cues related to the project's architecture and maintenance. GitQ displayed metrics related to the repository's source code and maintenance status, offering insights into the activeness and complexity of the repositories. By focusing on redesigning the environment, project teams seek to minimize barriers to entry, promote active participation, and foster a positive initial experience for newcomers as they become acclimated to the project's objectives and dynamics.


\textbf{Project knowledge representation.} The is category involves the use of various tools and techniques to capture, organize, and present knowledge within a project environment, particularly during the onboarding process for newcomers. It focused on enhancing the accessibility and comprehensibility of project-related information. Strategies within this category often include the development of dashboards (PS07), web portals (PS15), and graphical tools (PS01, PS11, PS18, PS20) that provide dynamic and visual representations of project resources, documentation, and contributions. In PS07 a dashboard is presented that assists community managers in monitoring and acknowledging newcomers' contributions. PS15 proposed and evaluated FLOSScoach, a a web portal created to support newcomers in OSS projects. FLOSScoach addresses barriers to entry by providing information and strategies in portal sections that align with different barrier categories. 

Further strategies within this category include the implementation of graphical tools (PS01, PS11, PS18, PS20) for organizing and visually presenting knowledge related to the project. PS01 unveiled SPL Cmaps, serving as sensemaking scaffolds to aid newcomers in comprehending the intricate domain of SPL engineering. By presenting newcomers with pertinent concepts and their interconnections to SPL features and core assets. PS11 offered a solution to comprehend foreign software code by leveraging node-link diagrams to visualize source code. PS18 extended Tesseract, an interactive project exploration environment, this approach captures intricate relationships between code, developers, software bugs, and communication records. It offers cross-linked panes for interactive socio-technical relationship exploration and visualizes socio-technical congruence. PS20 constructed a knowledge graph to integrate program structure data extracted from project code and multi-source information from different project versions. By utilizing these approaches, project teams aim to facilitate efficient navigation, understanding, and engagement for newcomers, enabling them to quickly familiarize themselves with project goals, tasks, and existing knowledge, thereby streamlining the onboarding process and fostering effective collaboration within the project. 


\textbf{Recommendation system.} This a category encompassing a diverse array of approaches aimed at providing personalized suggestions and guidance to individuals, particularly newcomers, within a specific context. In the context of onboarding newcomers to projects, recommendation systems play a crucial role by offering tailored recommendations to assist in various aspects of project engagement. These recommendations can span a wide range of areas, such as suggesting projects that align with newcomers' skills and interests (PS05, PS21, PS22, PS28, PS29, PS31). In PS05, a conversational bot was developed to recommend suitable projects to newcomers and assist them in the onboarding process within the OSS community. PS21 presented ReBOC, a recommendation system suggesting Open Source Software for Social Good (OSS4SG) projects based on contributors' activities and project-related information. PS22 unveiled NNLRank (Neural Network for List-wise Ranking), a learning-to-rank model harnessing developers' extensive OSS project histories on GitHub to suggest projects aligning with their contributions, thus fostering productive collaboration. PS28 presented RepoLike, an approach for recommending repositories to developers by predicting their interests. PS29 proposed GHTRec, an approach for recommending personalized GitHub trending repositories to software developers. PS31 proposed an approach to recommend projects based on developer behavior and the projects in their repository rather than a specific project. This developer-oriented recommendation approach helps developers discover more relevant projects, including those that are less popular.

Some approaches provide recommendations for source code files for integration (PS03, PS10, PS20, PS27). PS03 introduced Hipikat, a tool designed to expedite the productivity of newcomers in OSS projects. Hipikat leverages the archives of a software development project as an implicit group memory, recommending relevant artifacts to newcomers based on the tasks they are attempting. PS10 introduced RecomMentor, a recommender system that assists feature-based onboarding in SPL organizations. PS20 proposed a strategy to expedite learning paths discovery within OSS projects by constructing a knowledge graph. PS27 presented Mentor, a recommender system that aids newcomers in solving change requests.

Other approaches guided newcomers toward relevant tasks/ bugs to tackle (PS12, PS13, PS18), PS12 proposed BugExchange, a system that curates tasks from various OSS projects to facilitate newcomer training. By evaluating and executing these tasks, newcomers gain a comprehensive understanding of the project, its technology, and key concepts. In PS18, the Tesseract tool enable users to identify bugs of interest, resources related to that bug, (e.g., related files, contributing developers, communication records). In PS13, a chatbot was developed to assist newcomers in filtering tasks and selecting assignments that align with their skill sets. 

Concerning to approaches that suggest initial issues or labels to engage with (PS07, PS08, PS14, PS19, PS24). PS07 shifted the focus towards empowering project maintainers the authors developed and evaluated a dashboard that detects if the issue labels the project currently uses include newcomer friendly labels used by other OSS projects and based on the above data, the dashboard suggests adding newcomer friendly labels. PS08 introduced GFI-Bot, which facilitates automated Good First Issue (GFI) recommendations on GitHub. It provides an interactive web portal for newcomers to explore GitHub projects and receive GFI suggestions and project maintainers. PS14 introduced an NLP-based approach for automatically tagging issues as suitable for newcomers. PS19 introduced RecGFI for GFI recommendation. By learning from historical issues resolved by newcomers, RecGFI extracted features from various sources of information, including issue content, background, and dynamics. Moreover, PS24 investigated the feasibility of automatically labeling issues with API domains to facilitate contributors' task selection. 

Other approaches focused on facilitating connections between newcomers and experienced mentors (PS02, PS06, PS09, PS16, PS25). PS09 introduced xFinder, a tool that leverages historical records from software repositories to recommend proficient developers who can offer guidance on specific files to newcomers. Similarly, PS16 addressed newcomer challenges by proposing a mentorship recommendation system, aiding newcomers in identifying the most suitable project member for guidance on technical tasks. Furthermore, PS25 introduced the Emergent Expertise Locator (EEL), which employs emergent team information to suggest experts within the development environment, aiding developers in communicate decisions during programming tasks. Notably, PS02 proposed Yoda, utilizing historical data to recommend mentors for newcomers. In PS06, the authors proposed an expert recommendation method that utilizes knowledge embedding and the random forest algorithm to recommend suitable experts for developers in real time.

The primary objective of recommendation systems is to enhance newcomers' experience by helping them navigate the project landscape, make informed decisions, and quickly become productive contributors. By analyzing available data and applying algorithms, recommendation systems offer insights and guidance that optimize the newcomer's path to effective participation and collaboration within the project.


%%%%% Overview RQ1

\rqone[
    \tcblower
    \textbf{Answer:} Among our findings, we've categorized the technological support strategies for newcomers during onboarding into three main themes: (i) redesigning of the project environment, encompassing gamification strategies (PS04, PS17, PS26) for engagement and modifications to platforms like GitHub (PS23, PS30); (ii) representation of project knowledge, featuring tools like dashboards (PS07), web portals (PS15), and graphical aids for organizing and presenting information (PS01, PS11, PS18, PS20); (iii) the incorporation of recommendation systems, spanning a wide range of approaches, from suggesting projects (PS05, PS21, PS22, PS28, PS29, PS31) aligned with newcomers' skills and interests to providing guidance on source file integration (PS03, PS10, PS20, PS27), task assignment (PS12, PS13, PS18), issue labeling (PS07, PS08, PS14, PS19, PS24), and fostering mentor-newcomer interactions (PS02, PS06, PS09, PS16, PS25) within software projects.
]{}

\subsection{RQ2: Implementation of technological support strategies on newcomers' onboarding}

Through our research, we have successfully identified a set of strategies used to implement the approaches for facilitating the onboarding of newcomers in software projects. The strategies have been described and organized in the taxonomy depicted in Figure~\ref{fig:techstrategies}. By categorizing and presenting these strategies, we aim to provide a comprehensive overview of the available approaches implemented that can effectively support newcomers in their transition and integration into software projects.


\begin{figure*}[h]
    \centering
    \includegraphics[width=17.5cm]{images/rq2new.pdf}
    \caption{Taxonomy of technological support strategies.}
    \label{fig:techstrategies}
\end{figure*}

\textbf{Chatbot.} Among the selected studies, three proposed chatbots to aid onboarding. Each chatbot proposed focuses on different types of recommendations: \textit{issue label} (PS08), \textit{project} (PS05) and \textit{task/bug} (PS13). The objective of this approaches was to alleviate the challenges faced by users when taking their first steps into OSS projects, particularly the difficulty of finding appropriate tasks. PS08, presented GFI-Bot a tangible implementation of a machine learning-powered bot aimed at automating the recommendation of GFI on GitHub. By allowing project maintainers to configure its actions, such as labeling and commenting on issues, the bot contributes to a more welcoming environment for newcomers. The architectural structure, encompassing modules like data collection, model training,  and creates a robust and comprehensive system. 


In PS05, the authors proposed a conversational bot tailored to recommend projects to newcomers and facilitate their onboarding into the open-source community. While still in the development phase, the bot's foundation lies in NLP methods, such as Natural Language Understanding (NLU) and text summarization. The integration of tools like Rasa Open Source, GitHub's REST API, and the Stack Exchange API underscores the commitment to implementing effective features. The envisioned integration with collaboration platforms like Slack signifies a seamless approach to engaging newcomers by tapping into their public GitHub and Stack Overflow information. PS13 introduced a task-finder chatbot designed to guide newcomers in selecting tasks aligned with their skill set within the JabRef project. The authors' innovative workaround to limitations in modifying labels directly on GitHub's issue tracker showcases their commitment to facilitating newcomers' engagement. By creating a mock issue tracker page and deploying the chatbot using the Watson Assistant platform, the authors offer newcomers a streamlined channel to identify tasks suited to their skills.

These three research works collectively demonstrate the growing interest and advancements in implementing chatbots to support newcomers in software development processes. Using chatbots to implement those approaches contributed to enhance the engagement and productivity of newcomers in the software development ecosystem.

 

\textbf{Machine learning.} We have identified seven studies that have harnessed the power of machine learning techniques to address the complexities of newcomers' onboarding strategies. These studies predominantly center on offering recommendations to newcomers, honing in on crucial aspects such as \textit{issue label} (PS08, PS19, PS24), \textit{mentor/expert} (PS06), \textit{projects} (PS28, PS29) and \textit{tasks/bugs} (PS14).

With the overarching goal of enhancing the onboarding process. In PS06 the authors demonstrated the implementation of a recommender system that employs the random forest method to suggest suitable experts for developers. This approach utilizes domain-specific file embeddings generated using node2vec, capturing behavioral patterns of developers, and employs a machine learning model for predictive expertise recommendations. PS08 proposed the GFI-Bot that exemplifies the integration of machine learning into the realm of newcomer onboarding. This prototype showcases the potential of machine learning to facilitate task selection and enhance newcomers' involvement. 

By analyzing the history of resolved issues and utilizing issue titles and descriptions, PS14 presents a dual contribution that emphasizes the role of machine learning in issue categorization. By introducing an NLP-based approach to automatically tag newcomer-friendly issues and establishing a framework for automated evaluation and enhancement of supervised machine learning models, this work streamlines the process of identifying suitable tasks for newcomers. PS19, proposed RecGFI that showcases the power of machine learning in predicting whether an issue qualifies as a Good First Issue. Leveraging extensive feature engineering and the XGBoost classifier, this approach demonstrates how machine learning can contribute to issue categorization by learning from historical ground truth data. PS24 extends the application of machine learning to automatic labeling of issues with APIs' domains. By employing a variety of classifiers in a multilabel classification approach, this work streamlines task selection for contributors by categorizing issues based on their domain associations. The application of machine learning in this context enhances the accuracy of issue categorization and contributes to newcomers' successful onboarding.

In order to explore the diverse applications of machine learning techniques in addressing newcomers' onboarding strategies concerned to project recommendation. PS28 and PS29 introduced machine learning-driven approaches to recommending repositories to developers. Both works leverage historical development activities, technical features, and social connections to predict developers' interests and preferences. By employing machine learning algorithms for repository recommendation, these works enhance developers' engagement and involvement within the software development community.

\textbf{Mobile application.} This category pertains to the specific aspect of onboarding approaches that used mobile applications to focus on guiding and assisting newcomers during the onboarding process. Only one approach was implemented in that sense, in PS26, a mobile app was designed for generations Y and Z entering the workforce. The high-fidelity prototype strategically incorporates gamification elements to enhance onboarding. The app's innovative features, including QR-Hunting, Company-Quiz, Team Bingo, Company-Whisper, and the Onboarding Tree, cater to modern employee preferences and engagement. Additionally, practical features like a newsfeed and communication capabilities reflect a comprehensive approach to newcomers onboarding. This work underscores the app's potential to revolutionize onboarding for tech-savvy professionals and provides valuable insights into the benefits of gamified strategies.

\textbf{Recommendation system.} In the realm of newcomer onboarding strategies, recommender systems play a significant role, covering various categories such as \textit{issue label} (PS08, PS19), \textit{mentor/expert} (PS02, PS06, PS09, PS16, PS25), \textit{project} (PS05, PS21, PS22, PS28, PS29, PS31), \textit{source files} (PS10, PS27) and \textit{SPL feature} (PS10).

%Among the approaches that used machine learning to recommend issue labels. We have PS08 ..<Describe implementation>.. In contrast, PS19 ..<Describe implementation>..

%Concern the use of recommender systems to enhance developer collaboration and mentorship. 
%PS09 ..<Describe implementation>.. 
%PS16 ..<Describe implementation>..
%PS25 ..<Describe implementation>..
%PS02 ..<Describe implementation>..
%PS06 ..<Describe implementation>..

%Focus on the utilization of recommender systems to elevate the effectiveness of project recommendations. PS05, also categorized under chatbot, introduced a conversational bot guiding newcomers in finding OSS projects and navigating the contribution process.  PS21...<Describe implementation>.

%Additionally, PS22..<Describe implementation>. PS28 ..<Describe implementation>..  PS29 ..<Describe implementation>..  PS31 ..<Describe implementation>..

%PS10..<Describe implementation>.. PS27 ..<Describe implementation>..
Each work offers unique perspectives on how these systems can effectively guide and engage developers. Notably, PS02 employs heuristics to recommend mentors based on historical project data, emphasizing relationship building for newcomers. The chatbot in PS05 combines NLP with external APIs to recommend projects and streamline onboarding. PS06 introduces a random forest-based system to guide developers towards experts, enhancing collaboration within projects. Meanwhile, PS08 utilizes machine learning to recommend issues for newcomers, fostering interaction. 

PS09 focused on aiding code modification by suggesting knowledgeable developers based on historical records. In PS10, is utilized topic modeling to assist software product line engineers in selecting relevant features for onboarding. PS16 innovatively suggests mentors based on source code history, email threads, and IDE interactions, tailoring guidance for newcomers. PS19 employs feature engineering and XGBoost to recommend Good First Issues, enhancing newcomers' engagement. 

In PS21, it personalizes OSS project recommendations by considering contributors' activities and project attributes. PS22 employed neural networks to efficiently recommend projects for onboarding. Moreover, PS25 identifies experts in real time through team information, improving communication and decision-making. While PS27 employed the Prediction by Partial Matching (PPM) algorithm to recommend relevant code for addressing change requests, aiding developers' problem-solving. PS28 leverages development activities and social connections to suggest engaging repositories, enhancing developer involvement. Additionaly, PS29 recommends trending GitHub repositories based on developers' historical commit repositories. Finally, PS31 introduces an approach that combines project and developer behaviors to suggest relevant projects, fostering engagement and contribution. This diverse array of works underscores the dynamic evolution of recommendation systems, catering to various aspects of developers' needs and enhancing their overall experience within the software development community.

%These studies contribute to the development of effective recommender systems that support newcomers during the onboarding process, facilitating their integration into OSS projects and promoting knowledge exchange within project communities.

\textbf{Visualization tool.} In our results, we came across six studies that explore visualization strategies in the following domains: \textit{project visualization} (PS01, PS11, PS18, PS20), \textit{issue label} (PS07), and \textit{source files} (PS20). By investigating these studies, our results show that its possible to explore the effectiveness of visualization strategies in supporting newcomers' understanding and engagement in various domains. Using these approaches can leverage and improve newcomers' comprehension of complex concepts, navigate project environments, and facilitate their learning paths within software projects.

In the pursuit of enhancing software understanding and collaboration, some approaches introduced innovative approaches that harness visualizations and knowledge information PS01 assist newcomers in understanding SPL engineering by offering domain-specific visualizations that leverage their existing knowledge. The approach entails Concept Extraction and Relationship Definition, culminating in structured SPL Cmaps that guide newcomers through the intricacies of SPL engineering. In PS07, a dashboard prototype is proposed to empower OSS community maintainers by offering tailored recommendations for attracting and retaining contributors. Created using the GitHub interface in Figma, the dashboard empower maintainers in fostering thriving OSS communities. 

PS11 introduced visualizations for unfamiliar codebases, enhancing code comprehension. These visualizations, integrated into an existing tool, provide a nuanced view of software classes and dependencies, ultimately bolstering collaboration in software projects. In PS18, Tesseract is enhanced with a search functionality using Solr, streamlining bug identification for newcomers. This enables efficient exploration and engagement within software projects. Lastly, PS20 implements an automated method to recommend learning paths for open-source projects. By constructing knowledge graphs and employing deep learning, this approach guides developers towards swift and targeted project exploration, fostering enhanced engagement within open-source communities. These works collectively underscore the significance of visualization tools in easing newcomers' entry into complex software domains, enabling efficient exploration, comprehension, and collaboration.



\textbf{Web environment.} Throughout our research, we identified studies that proposed modifications to the environment to facilitate the success of newcomers during the onboarding process and implemented in a web environment setting, with a focus on \textit{gamification} (PS04, PS17) and the \textit{modification of GitHub interface} (PS23, PS30), \textit{dashboard} (PS07), \textit{dynamic documentation} (PS15), \textit{source files} (PS03) and \textit{task/bug}  (PS12, PS18).

Concerning the gamification strategies for enhancing newcomer engagement in OSS projects to guide and motivating newcomers to overcome onboarding barriers and engage in OSS projects. Two approaches applied game elements in a web environment (PS04, PS17). The integration of gamification elements into the GitLab platform proposed in PS04 enables undergraduate students to navigate open-source projects with enhanced motivation. Meanwhile PS17 proposed a gamified version of the FLOSScoach portal that operates in web environments, offering comprehensive support to newcomers in OSS projects.

Concerning the modification of GitHub interface to enhance inclusivity and usability through the redesign of the OSS environment (PS23, PS30) providing visual elements facilitated newcomers' understanding of the repositories and supported their decision-making process. PS23 tackles inclusivity bugs on the GitHub interface by implementing fixes via a JavaScript plugin, contributing to a more inclusive experience. PS30 developed the GitQ browser extension, providing visual cues through badges, efficiently conveying project information to developers on GitHub repositories. 

Concerning the approach that implemented a dashboard in the web environment PS07 introduced a dashboard prototype designed for OSS community maintainers, offering targeted recommendations to attract and retain contributors, with the dashboard implemented using the GitHub interface in Figma. Moreover, related to dynamic documentation, PS15 designed and assess FLOSScoach, a web portal developed to assist newcomers in OSS projects. FLOSScoach portal was grounded in a conceptual model of barriers, previously proposed by the authors, which categorizes 58 barriers into six distinct categories. This model served as the foundation for the design and structure of the FLOSScoach portal, aiming to address these barriers and provide comprehensive support to newcomers entering the OSS community.

Related to source files PS03 employed a client-server system to create an implicit group memory, facilitating newcomers' access to relevant artifacts within open-source project archives. Concerning to task/bug tools developed in a web environment. PS12 aims to curate tasks from OSS projects for newcomers' training, augmenting their comprehension and engagement within projects.  The expansion of Tesseract proposed in PS18 into an interactive environment with search capabilities strengthens newcomers' ability to explore project bug descriptions. 

By examining these studies, our results show that there are opportunities to explore the effectiveness of gamification and environmental redesign strategies in facilitating newcomers' onboarding experiences. Through these modifications, it would be possible to enhance motivation, engagement, and inclusivity among newcomers in OSS projects, ultimately fostering a welcoming and supportive environment for their integration and growth.


%%%%% Overview RQ2

\rqtwo[
    \tcblower
    \textbf{Answer:} Our findings highlight how the technological support strategies were implemented. We categorized a comprehensive set of strategies aimed at enhancing newcomers' onboarding experiences in software projects. These strategies encompass various domains, including chatbots, machine learning, mobile applications, recommendation systems, visualization tools, and web environment modifications. Some approaches utilize chatbots focused on different types of recommendations: issue label (PS08), project (PS05) and task/bug (PS13) providing assistance to newcomers during the onboarding process. Machine learning techniques are employed to recommend issue labels (PS08, PS19, PS24), mentors/experts (PS06), projects (PS28, PS29) and tasks/bugs (PS14). A mobile application approach was used to support the onboarding (PS26). Recommendation systems play a significant role in recommending issue label (PS08, PS19), mentor/expert (PS02, PS06, PS09, PS16, PS25), projects (PS05, PS21, PS22, PS28, PS29, PS31), source files (PS10, PS27) and SPL features (PS10). Some approaches presented visualization tools to expedite newcomers' productivity, supporting project visualization (PS01, PS11, PS18, PS20), issue label (PS07), and source files recommendation (PS20) to provide assistance and resources during the onboarding process. Modifying the environment through the development of web applications with a focus on gamification (PS04, PS17) and the modification of GitHub interface (PS23, PS30), dashboard (PS07), dynamic documentation (PS15), source files recommendation (PS03) and task/bug recommendation (PS12, PS18) to enhance newcomer engagement and inclusivity.
]{}


\subsection{RQ3: Impact of technological support strategies on newcomers' onboarding}

To address our research question, we have categorized the impact of each selected study into five distinct categories, as presented in Table~\ref{tab:impactcategories}. It is important to note that some studies were classified in multiple categories based on the impact of their proposed technological approaches.

\begin{table}[!ht]\scriptsize
\centering
\caption{Impact categories of strategies on newcomers' onboarding}
\label{tab:impactcategories}
\begin{tabular}{l|c|c|c}
\hline 
\multicolumn{1}{c|}{\textbf{Impact}} & \textbf{\begin{tabular}[c]{@{}c@{}}Study \\ reference\end{tabular}} & \textbf{\# of studies} & \textbf{\%} \\ \hline \hline

\begin{tabular}[c]{@{}l@{}}Contribution process \\ and orientation\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS07, PS10, PS11, PS13, \\ PS15, PS17, PS21, PS22, \\ PS23, PS26, PS28, PS29, \\ PS30, PS31\end{tabular} & 14 & 45\% \\ \hline
\begin{tabular}[c]{@{}l@{}}Improve newcomers \\ experience\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS04, PS05, PS17, \\ PS20, PS23, PS26, PS30\end{tabular} & 6 & 19\% \\ \hline
Improve productivity & PS01, PS03, PS20, PS27, & 4 & 13\% \\ \hline
\begin{tabular}[c]{@{}l@{}}Labeling and \\ task selection\end{tabular} & \begin{tabular}[c]{@{}c@{}}PS08, PS12, PS13, \\ PS14, PS18, PS19, PS24\end{tabular} & 7 & 23\% \\ \hline
Mentoring & \begin{tabular}[c]{@{}c@{}}PS02, PS06, PS09, \\ PS12 , PS13, PS16, PS25\end{tabular} & 7 & 23\% \\ \hline \hline
\end{tabular}
\end{table}

The category with the highest number of studies, consisting of 14 studies (45\%), focuses on the contribution process and orientation. These studies primarily revolve around approaches developed to introduce and guide newcomers through the process of making contributions to OSS projects and emphasize the provision of clear guidelines, documentation, and resources to help newcomers understand the project's objectives, coding standards, version control systems, and collaborative tools (PS07, PS10, PS11, PS13, PS15, PS17, PS21, PS22, PS23, PS26, PS28, PS29, PS30, PS31).

Additionally, we have two categories, each comprising seven studies (23\%), that primarily impact labeling and task selection. These studies focus on the process of categorizing and labeling tasks within an OSS project to assist newcomers in identifying tasks suitable for their skill levels and interests. The aim is to mark tasks with appropriate labels, such as GFI and provide clear descriptions and instructions to ensure newcomers can easily select and engage with tasks aligned with their capabilities (PS08, PS12, PS13, PS14, PS18, PS19, PS24).

Furthermore, we have studies that impact the mentoring process, accounting for seven studies (23\%). Mentoring in the context of software projects refers to the practice of pairing experienced contributors with newcomers to provide guidance, support, and knowledge transfer. The approaches focusing on mentorship support help newcomers navigate the project, understand the community dynamics, learn the technical aspects, and develop their skills. Effective mentoring programs establish constructive learning relationships between mentors and mentees, fostering the growth and integration of newcomers into the OSS community (PS02, PS06, PS09, PS12, PS13, PS16, PS25).

Another set of approaches, comprising six studies (19\%), aims to enhance newcomers' experience within software projects. These approaches encompass strategies and initiatives focused on creating a welcoming and inclusive environment, facilitating communication channels for inquiries and seeking help, and providing mentorship or support programs to assist newcomers in navigating the project successfully (PS04, PS05, PS17, PS20, PS23, PS26).

Lastly, some approaches, totaling four studies (13\%), concentrate on improving productivity by adopting initiatives that maximize the efficiency and effectiveness of newcomers' contributions. These approaches involve providing development tools and infrastructure, offering coding guidelines and best practices, and fostering a culture of collaboration and knowledge sharing among project contributors (PS01, PS03, PS20, PS27).



%%%%% Overview RQ3


\rqthree[
    \tcblower
    \textbf{Answer:} The impact of technology support strategies on newcomers' onboarding was examined, revealing five distinct categories with varying percentages. The highest number of studies (45\%) focused on the contribution process and orientation, providing guidelines and resources for newcomers. Labeling and task selection (23\%) aimed to assist newcomers in identifying suitable tasks, while mentoring (23\%) emphasized guidance and integration into the community. Strategies enhancing newcomers' experience (19\%) and improving productivity (13\%) were also observed. It is evident that technological approaches have a significant impact on newcomers' onboarding, covering various aspects to facilitate their integration and effectiveness in software projects.
]{}







\subsection{RQ4: Evaluation of technological support strategies for onboarding}

The objective of this research question is to investigate the evaluation methods used to assess the effectiveness of technological support strategies for newcomers' onboarding. Table~\ref{tab:evalnewcomersonboarding} presents the types of evaluations identified in the selected primary studies.

\begin{table}[!ht]\scriptsize
\centering
\caption{Evaluation types of technological support strategies}
\label{tab:evalnewcomersonboarding}
\begin{tabular}{l|c|c|c}
\hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Type of \\ analysis\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Study \\ reference\end{tabular}} & \textbf{\# of studies} & \textbf{\%} \\ \hline \hline
Computer evaluation & \textbf{\begin{tabular}[c]{@{}c@{}}PS08, PS09, PS10, \\ PS19, PS20, PS24, \\ PS25, PS27, PS28, PS29\end{tabular}} & 10 & 32\% \\ \hline
Empirical evaluation & \textbf{PS11, PS22, PS23} & 3 & 10\% \\ \hline
No evaluation & \textbf{PS05, PS12, PS16, PS18} & 4 & 13\% \\ \hline
Qualitative analysis & \textbf{\begin{tabular}[c]{@{}c@{}}PS01, PS02, PS03, PS04, \\ PS07, PS10, PS13, PS14, \\ PS15, PS17, PS20, PS21, \\ PS23, PS26, PS29, PS31\end{tabular}} & 16 & 52\% \\ \hline
Quantitative analysis & \textbf{\begin{tabular}[c]{@{}c@{}}PS01, PS02, PS06, \\ PS13, PS14, PS15, PS19, \\ PS22, PS23, PS24, PS30\end{tabular}} & 11 & 35\% \\ \hline \hline
\end{tabular}
\end{table}

More than half of the studies, 16 out of 31 (52\%), employed qualitative analysis to gain insights into onboarding strategies by interpreting data to understand subjective experiences associated with the onboarding process from the perspectives of newcomers (PS01, PS02, PS03, PS04, PS07, PS10, PS13, PS14, PS15, PS17, PS20, PS21, PS23, PS26, PS29, PS31). Additionally, 11 studies (35\%) utilized quantitative analysis to evaluate their proposed approaches to collect and analyzing measurable data related to onboarding, such as success rates, completion times, user satisfaction ratings, or performance metrics (PS01, PS02, PS06, PS13, PS14, PS15, PS19, PS22, PS23, PS24, PS30).

A total of 10 studies (32\%) conducted computer evaluations, which involved analyzing onboarding strategies using automated computational techniques. This type of evaluation relied on computer-based methods to assess the onboarding process aspects and its outcomes (PS08, PS09, PS10, PS19, PS20, PS24, PS25, PS27, PS28, PS29). Four studies (13\%) did not conduct specific analyses of the onboarding strategies proposed. This indicates that the research or study did not involve a systematic investigation or evaluation of the results of the implemented onboarding approaches in software projects (PS05, PS12, PS16, PS18).

Furthermore, three studies (10\%) conducted empirical evaluations by observing, collecting, and analyzing real-world data. These studies aimed to gather empirical evidence from actual users in software projects to assess the impact, effectiveness, and user experience of different onboarding strategies. Empirical evaluation provided valuable insights into the practical application and outcomes of the onboarding approaches (PS11, PS22, PS23).

Based on the analysis of the selected studies, it is evident that a significant proportion of them focused on empirical evaluation, with 27 studies (87\%) incorporating this evaluation component alongside proposing technological support strategies for newcomers' onboarding (PS01, PS02, PS03, PS04, PS06, PS07, PS08, PS09, PS10, PS11, PS13, PS14, PS15, PS17, PS19, PS20, PS21, PS22, PS23, PS24, PS25, PS26, PS27, PS28, PS29, PS30, PS31). Only 4 studies (13\%) that did not include empirical evaluation in their research (PS05, PS12, PS16, PS18).

Out of the total 31 studies, 25 studies (81\%), successfully implemented their proposed approaches (PS01, PS02, PS03, PS04, PS06, PS08, PS09, PS10, PS11, PS13, PS14, PS15, PS18, PS19, PS20, PS21, PS22, PS23, PS24, PS25, PS27, PS28, PS29, PS30, PS31). However, there was one study (3\%) that did not implement the proposed approach (PS16), and five studies (16\%) were still in the development process of their approaches by the time the paper was published (PS05, PS07, PS12, PS17, PS26).

%%%%% Overview RQ4

\rqfour[
    \tcblower
    \textbf{Answer:} The literature utilized different evaluation methods to measure the effectiveness of technology support strategies for newcomers' onboarding. The findings show that 52\% of the studies employed qualitative analysis, 35\% used quantitative analysis, 32\% conducted computer evaluations, and 10\% performed empirical evaluations. The majority of the studies (87\%) incorporated empirical evaluation alongside proposing technological support strategies. Out of the total studies, 81\% successfully implemented their approaches, while 3\% did not implement them and 16\% were still in the development process.
]{}





\subsection{RQ5: Technological support strategies on newcomers' onboarding related to the barriers to joining software projects}

\citet{steinmacher2019overcoming} conducted a qualitative analysis of relevant literature and collected data from practitioners to identify the barriers that hinder newcomers' initial contributions to various domains. As a result of their comprehensive investigation, the authors developed a model comprising 58 distinct barriers. Building upon this foundation, our study focuses on evaluating the existing onboarding strategies proposed in the literature and assessing their efficacy in addressing and mitigating these identified barriers, as illustrated in Figure~\ref{fig:barriersandstrategies}. By examining and highlighting the effectiveness of these strategies, we aim to contribute to the advancement of onboarding practices and facilitate newcomers' successful integration and participation in their respective domains.



\begin{figure*}[h]
    \centering
    \includegraphics[width=17.5cm]{images/rq4-barriers.pdf}
    \caption{Onboarding strategies to overcome barriers.}
    \label{fig:barriersandstrategies}
\end{figure*}

\textbf{Newcomers' orientation.} It is a critical phase in facilitating newcomers' successful integration and contribution to various settings. However, several barriers hinder this process, such as difficulties in finding appropriate tasks to start with and accessing mentors for guidance and support, we will present the papers that address these challenges below.

\begin{itemize}
    \item \textbf{Finding a task to start with:} Among the selected studies some approaches(PS04, PS05, PS07, PS08, PS12, PS13, PS14, PS15, PS17, PS18, PS19, PS24, PS31) addressed the challenge of finding a task for newcomers. These strategies offer insights into effective task selection, providing clear guidelines, utilizing task recommendation systems, and leveraging task complexity levels to match newcomers' skills and interests. By implementing these strategies, organizations, and communities can facilitate newcomers' engagement and help them contribute meaningfully from the beginning;

    \item \textbf{Finding a mentor:} The identified studies (PS02, PS05, PS06, PS09, PS12, PS13, PS14, PS15, PS16, PS19, PS31) shed light on effective approaches to streamline the process of finding a mentor. These strategies underscore the significance of mentorship programs, mentor-mentee matching systems, and establishing efficient communication channels between newcomers and mentors. By adopting these approaches, organizations and communities can cultivate supportive relationships that empower newcomers to seek guidance, acquire valuable knowledge, and navigate challenges encountered during their integration.
\end{itemize}

The following onboarding barriers do not have any specific onboarding strategies approaches proposed in the literature, due to that we highlight them as research opportunities that emerge to be further investigated by the software engineering community,  these barriers are related to newcomers' orientation such as: \textbf{\textit{(i) finding the correct artifacts to fix an issue:}} there is a need for exploring methods to assist newcomers in identifying relevant artifacts needed to fix an issue/task and addressing them effectively. PS03 is the only approach that recommended artifacts from the archives that are relevant to a task that a newcomer is trying to perform; \textbf{\textit{(ii) poor "How to Contribute" availability:}} It is important to call attention and investigate ways to improve the availability and accessibility of comprehensive and user-friendly resources that guide newcomers through the contribution process. This may involve creating well-structured documentation, tutorials, and interactive guides; \textbf{\textit{(iii) outdated list of bugs:}} other opportunities would be developing strategies to ensure that bug lists or issue repositories are regularly updated, providing newcomers with up-to-date and relevant tasks. This may involve implementing mechanisms for tracking the status and activity of reported issues; \textbf{\textit{(iv) reproducing issues:}} Another interesting point would be to explore techniques and tools to assist newcomers in reproducing reported issues, enabling them to understand and address problems effectively. This may involve creating reproducibility guidelines, providing virtualized or sandboxed environments, or offering step-by-step debugging support; \textbf{\textit{(v) newcomers' lack of awareness of the contribution flow:}} would be very important to investigate approaches to provide clear and concise guidance on the contribution flow, ensuring that newcomers understand the steps and expectations involved in their contributions. This may involve creating visual diagrams, interactive workflows, or onboarding tutorials that walk newcomers through the contribution process. 

\textbf{Newcomers' characteristics.} Pose significant challenges during the onboarding process and can lead to different barriers. Newcomers are expected to possess a minimum requirement of previous technical background to perform a development task~\cite{steinmacher2019overcoming}. Characteristics, such as lack of domain experience, knowledge of project processes and practices, and technical background can be very hard to approach. In the following, we discuss the proposed onboarding strategies from the literature that aim to mitigate some newcomers’ characteristics barriers and facilitate newcomers' integration and contribution.

\begin{itemize}
    \item \textbf{Lack of domain experience:} To address the barrier of lack of domain experience (PS01, PS03, PS05, PS07, PS08, PS10, PS11, PS12, PS15, PS20, PS23, PS27, PS29, PS31), various strategies have been proposed. These include broadening newcomers domain knowledge and reducing information overload, forming an implicit group memory from the information stored in a project’s archives, and providing newcomers' support not only during their first contribution, but by acting as an agent to engage them in the project and promoting collaboration between newcomers and domain experts. These approaches aim to bridge the knowledge gap and empower newcomers to acquire domain expertise gradually, enabling them to contribute effectively in their respective domains.
    
    \item \textbf{Lack of knowledge in project process and practices:} To mitigate the barrier of lack of knowledge in project process and practices (PS01, PS02, PS03, PS04, PS05, PS06, PS07, PS08, PS10, PS11, PS15, PS16, PS17, PS20, PS21, PS22, PS23, PS24, PS26, PS27, PS28, PS29, PS30, PS31), several strategies have been proposed. These include providing comprehensive documentation and resources that explain project workflows, coding standards, and communication channels.
    
    \item \textbf{Lack of technical background:} To overcome this barrier (PS01, PS03, PS05, PS07, PS08, PS09, PS10, PS11, PS15, PS18, PS20, PS23, PS25, PS27, PS31), various strategies have been proposed. These include offering guidance during the contribution process, recommendation of project documentation, and pairing newcomers with experienced developers as mentors. These strategies aim to enhance newcomers' technical skills, fill the gaps in their knowledge, and build their confidence to actively contribute to technical projects.    
\end{itemize}

Despite the progress made in developing onboarding strategies for mitigating barriers related to newcomers' characteristics, there are some barriers that can be seen as research opportunities that require further exploration. Among the opportunities we have the following: \textbf{\textit{(i) lack of proactivity:}} investigating approaches to encourage newcomers to take a proactive stance in their onboarding process. This may involve designing interventions, creating platforms for collaboration and engagement, and providing incentives to motivate newcomers to actively seek knowledge and participate in project activities; \textbf{\textit{(ii) lack of commitment:}} exploring strategies to enhance newcomers' commitment levels throughout the onboarding journey. This could involve developing personalized onboarding plans, setting clear goals and expectations, and providing regular feedback and recognition to foster a sense of commitment and accountability; \textbf{\textit{(iii) underestimating the challenge:}} Understanding and addressing the issue of newcomers underestimating the challenges they may face during the onboarding process. This may involve providing realistic expectations, highlighting the learning curve, and offering support mechanisms to help newcomers navigate difficulties and setbacks effectively; and \textbf{\textit{(iv) lack of patience:}} investigating approaches to cultivate patience and resilience among newcomers when encountering obstacles or setbacks during their onboarding journey. This could include mentorship programs, peer support networks, and guidance on managing expectations and building a growth mindset.

\textbf{Communication.} According to \citet{steinmacher2019overcoming}, observed that newcomers are sometimes unaware of community protocol, language, or even the most appropriate communication means to use. We have identified specific approaches from the literature that address these barriers and aim to enhance effective communication between newcomers and existing members of the community or project.

\begin{itemize}
    \item \textbf{Not receiving an answer:} To address this barrier, some strategies were proposed (PS15, PS16, PS25). These include assigning experienced members as mentors to ensure timely responses to newcomers' requests. Additionally, creating designated communication channels, such as dedicated forums or mailing lists, can facilitate better visibility of newcomers' questions and increase the chances of receiving timely answers from the community members.

    \item \textbf{Sending a message that is considered impolite:} To mitigate this barrier, approaches emphasize the importance of providing newcomers with guidelines on appropriate communication (PS15, PS16, PS25). This includes educating newcomers about community norms, promoting respectful and inclusive language, and encouraging them to seek feedback on their communication style to avoid unintentional rudeness or misunderstandings.

    \item \textbf{Need to contact a real person:} To address this barrier (PS02, PS05, PS06, PS09, PS12, PS15, PS16, PS25, PS26), strategies have been proposed to provide effective communication to newcomers. These include mentoring initiatives, such as pairing newcomers with experienced community members, by recommending mentors to newcomers.
\end{itemize}

While existing onboarding strategies have made progress in mitigating communication barriers, there are still research opportunities to further enhance the onboarding process. These opportunities include addressing the following areas: \textbf{\textit{(i) delayed answers:}} investigating approaches to reduce delays in answering newcomers' inquiries. This may involve optimizing response systems, setting response time expectations, and implementing automated or AI-based support to handle common queries and provide timely assistance; \textbf{\textit{(ii) answering with too advanced/complex contents:}} exploring methods to ensure that answers provided to newcomers are understandable and suitable for their level of knowledge and expertise. This may involve creating knowledge resources with varying levels of complexity, encouraging community members to provide clear and concise explanations, and promoting effective communication practices; \textbf{\textit{(iii) not sending a meaningful/correct message:}} investigating strategies to improve the quality and accuracy of communication from both newcomers and existing members. This could include providing communication guidelines, offering templates or examples of effective messages, and encouraging constructive feedback and peer review of communication exchanges; \textbf{\textit{(iv) English level:}} addressing language barriers for non-native English speakers. This may involve providing language support resources, facilitating language exchanges or translation assistance, and promoting inclusive and multicultural communication practices within the community; \textbf{\textit{(v) shyness:}} exploring approaches to support and empower shy or introverted newcomers in their communication efforts. This could include creating safe spaces for interaction, offering communication training, and providing mentorship or peer support specifically tailored to help shy individuals overcome barriers and engage in effective communication; \textbf{\textit{(vi) making useless comments in the mailing list/forum:}} investigating methods to foster meaningful and productive discussions by discouraging irrelevant or low-value comments. This may involve community moderation, setting guidelines for constructive participation, and promoting a culture of mutual respect and relevance in communication platforms; \textbf{\textit{(vii) low responsiveness:}} exploring ways to enhance responsiveness from existing members when interacting with newcomers. This could include incentivizing and recognizing responsive behavior, establishing clear expectations for community participation, and implementing systems to track and measure responsiveness levels; \textbf{\textit{(viii) not acknowledging/thanking answers:}} investigating approaches to encourage newcomers to acknowledge and express gratitude for the assistance they receive. This may involve raising awareness about the importance of appreciation in community dynamics, providing guidance on appropriate ways to express gratitude, and fostering a culture of appreciation and recognition.

\textbf{Documentation problems.} We have identified specific approaches from the literature that address onboarding strategies proposed to mitigate barriers related to documentation problems and aim to enhance the effectiveness and usability of documentation for newcomers.

\begin{itemize}
    \item \textbf{Outdated information:} To address this barrier, approaches emphasize the importance of maintaining up-to-date documentation (PS03, PS11, PS15). Strategies include establishing documentation review processes, involving community members in the documentation and comprehending project source code, as stated in PS11 ``\textit{Comprehending the source code included in a software project allows newly hired software engineers to work on the first tasks in the new project}''. Additionally, creating mechanisms for community members to provide feedback on outdated information can help identify and address inaccuracies more efficiently.    

    \item \textbf{Information overload:} To mitigate this barrier, approaches focused on organizing and structuring documentation in a user-friendly manner (PS03, PS11, PS15, PS23). This includes creating clear and concise documentation, breaking down complex concepts into manageable sections, providing search functionalities or navigation tools, and offering contextual guidance to help newcomers find the most relevant information based on their specific needs.

    \item \textbf{Code comments not clear:} To address this barrier, strategies emphasize the importance of maintaining well-documented code (PS03, PS11, PS15). This includes providing guidelines for writing clear and descriptive comments, encouraging code reviews and feedback, and promoting a culture of code documentation within the development community.

    \item \textbf{Lack of documentation:} To mitigate this barrier, approaches focus on actively creating and improving documentation resources (PS03, PS11, PS15, PS20, PS23). This includes dedicating resources and efforts to document essential aspects of the project and in the code, establishing documentation writing guidelines, and involving community members in the documentation process through collaborative platforms or documentation sprints. In PS20 their approach reduce the time spent by developers on reading and studying the project code, and it can improve the accuracy of developers’ learning correct knowledge.
\end{itemize}

Those existing onboarding strategies have made progress in mitigating documentation problems, but there are still research opportunities to further enhance the onboarding process. These opportunities include addressing the following areas: \textbf{\textit{(i) unclear documentation:}} investigating methods to improve the clarity and comprehensibility of documentation. This may involve conducting usability studies, employing natural language processing techniques to analyze and enhance documentation readability, and incorporating user feedback and testing to identify and address areas of confusion or ambiguity; and \textbf{\textit{(ii) spread documentation:}} exploring approaches to consolidate and centralize documentation resources. It may involve developing unified documentation platforms, implementing knowledge management systems, and establishing clear guidelines for documentation organization and structure to avoid fragmentation and scattered information.

\textbf{Technical hurdles.} We have identified specific approaches from the literature that address barriers related to technical hurdles and aim to facilitate newcomers' understanding and navigation of technical aspects within a project.

\begin{itemize}
    \item \textbf{Local environment setup hurdles:} Some approaches focused on streamlining the setup process and providing comprehensive instructions (PS01, PS03, PS04, PS10, PS11, PS15, PS20, PS25, PS27). Strategies include creating detailed installation guides, and offering pre-configured development environments to ensure a smooth onboarding experience.

    \item \textbf{Code/architecture hurdles:} Other approaches emphasize the importance of documentation and guidance (PS01, PS02, PS03, PS04, PS10, PS11, PS15, PS20, PS23, PS25, PS27). Strategies include providing code walkthroughs, architectural diagrams, and high-level overviews of the project structure. Those strategies can help newcomers navigate the codebase and understand the project's architecture.

    \item \textbf{Change request hurdles:} Among our selected studies we found some strategies focused on providing clear guidelines for submitting and handling change requests (PS01, PS03, PS04, PS10, PS11, PS15, PS19, PS20, PS25, PS27, PS30, PS31). This includes creating templates for change requests, specifying the required information and format, and establishing clear communication channels between newcomers and project contributors. Additionally, offering mentorship where experienced members guide newcomers through the change request process can help address this barrier effectively.
\end{itemize}

While existing onboarding strategies have made progress in mitigating technical hurdles, there are still research opportunities to further enhance the onboarding process. These opportunities include addressing the following areas: (i) code characteristics: investigating the characteristics of code that pose challenges for newcomers, such as code quality, complexity, instability, and adherence to coding standards. This may involve conducting code analysis, developing tools for automated code quality assessment, and exploring methods to simplify complex code structures; and (ii) cognitive problems: exploring the cognitive aspects of understanding and working with code. This may include studying the cognitive processes involved in code comprehension, investigating methods to improve code understanding through visualizations or interactive tools, and identifying common cognitive barriers faced by newcomers. We would like to highlight that PS23 was the only work that mitigated cognitive barriers that newcomers face during the contribution process.

%%%%% Overview RQ5

\rqfive[
    \tcblower
    \textbf{Answer:} Our study aims to assess the effectiveness of various onboarding strategies proposed in the literature, specifically targeting the barriers that hinder the onboarding process. With regards to newcomers' orientation, certain strategies have been suggested to assist them in identifying suitable tasks and connecting with mentors who can offer guidance. To address the unique characteristics of newcomers, strategies have been put forth to bridge the gap in domain experience, project processes and practices knowledge, and technical background. Communication barriers have been tackled through strategies such as mentor assignments and the provision of guidelines for effective communication. Additionally, efforts have been made to alleviate documentation-related issues by maintaining up-to-date and user-friendly documentation, incorporating clear code comments, and actively developing documentation resources. Nevertheless, there are still opportunities for research to enhance the clarity and comprehensibility of documentation, consolidate available documentation resources, and overcome technical obstacles like local environment setup. We also emphasize the significance of further investigation by the research community into these barriers, as it can lead to advancements in the newcomers' onboarding process.
]{}




\subsection{RQ6: Impact of technological support strategies on diversity and inclusion in newcomer onboarding}

The importance of social diversity in software projects has been well-established, with numerous studies showing its positive impact on productivity, teamwork, and the quality of contributions~\cite{horwitz2007effects, vasilescu2015gender}. Conversely, the lack of diversity has significant drawbacks: (i) open-source projects miss out on the benefits of a wider range of contributors and the diverse perspectives they bring; (ii) underrepresented groups miss out on valuable learning and experience opportunities offered by these projects; and (iii) individuals from minority backgrounds may face limited job opportunities when OSS contributions are used in hiring decisions~\cite{marlow2013impression, singer2013mutual, santos2023designing}. Despite the long-standing recognition of the diversity gap in OSS, progress in addressing this issue has been limited~\cite{robles2016women, ford2017someone, trinkenreich2021women}. In our study, we examined the onboarding strategies proposed in the literature to assess their potential for facilitating diversity and inclusion among newcomers in software projects.

Our analysis of the selected studies showed that 30 out of 31 (97\%) proposed onboarding strategies targeting a general newcomer population without considering or validating their effectiveness for integrating different types of users into software projects (PS01, PS02, PS03, PS04, PS05, PS06, PS07, PS08, PS09, PS10, PS11, PS12, PS13, PS14, PS15, PS16, PS17, PS18, PS19, PS20, PS21, PS22, PS24, PS25, PS26, PS27, PS28, PS29, PS30, PS31). Only one study (3\%), PS23, focused on providing support tailored to newcomers with specific cognitive styles that may create barriers to programming for certain populations. Research indicates that cognitive styles often favored by women are frequently unsupported, leading to entry barriers for female newcomers. PS23 specifically addressed the needs of minority newcomers.

Regarding the explicit focus on diversity and inclusion, 29 studies (94\%) did not mention any specific emphasis in this regard (PS01, PS02, PS03, PS04, PS05, PS06, PS08, PS09, PS10, PS11, PS12, PS13, PS14, PS15, PS16, PS17, PS18, PS19, PS20, PS21, PS22, PS24, PS25, PS26, PS27, PS28, PS29, PS30, PS31), while only two studies (6\%) addressed diversity and inclusion concerns (PS07, PS23). In PS07, the authors explained that they selected participants from OSS4SG projects, including their maintainers, for evaluation as these projects tend to attract contributors from underrepresented groups, offering an excellent opportunity to recruit participants from diverse backgrounds. In PS23, the focus was on mitigating cognitive barriers faced by newcomers due to inclusivity bugs. The study revealed that platforms like GitHub, which newcomers use to contribute to OSS, create barriers for users with different characteristics, disproportionately impacting underrepresented groups. By addressing these barriers, the study shed light on how newcomers' performance can be improved when their cognitive styles are supported, thereby contributing to overall community diversity.

It is worth noting that the majority of studies proposing technological onboarding strategies predominantly focused on newcomers in general. This finding highlights the need for more research in the software engineering field that specifically targets increasing diversity and inclusion in software communities to increase and facilitate more inclusive onboarding strategies.

%%%%% Overview RQ6

\rqsix[
    \tcblower
    \textbf{Answer:} Our study evaluated the extent to which technology support strategies prioritize diversity and inclusion among newcomers. We found that 97\% of proposed onboarding strategies targeted a general newcomer population without considering different user types, while only 3\% addressed the specific needs of minority newcomers. Additionally, 94\% of the studies did not mention any emphasis on diversity and inclusion, whereas 6\% explicitly addressed these concerns. These findings highlight the need for more research and inclusive onboarding strategies to increase diversity in software communities.
]{}




%
\begin{table*}[ht!]
	\caption{Research questions and their rationales} \label{table:conductionRQ}
	\vskip 0.3cm
	\centering
	\begin{tabular}{p{0.7cm}||p{7cm}|p{9cm}}
		\hline
		\textbf{N$^{o}$} & \textbf{Research question} & \textbf{Rationale} \\ \hline \hline

            \textbf{RQ1} & \textit{What software solutions are proposed in the literature to facilitate newcomers' onboarding in software projects?} & We intend to highlight the existing software solutions that minimizes the human participation to help newcomers onboarding. \\ 
		\hline

            \textbf{RQ2} & \textit{How were the software solutions implemented?} & We intend to provide details of how the software solutions were implemented to guide new solutions that want to create or improve the existing software solutions. \\ 
		\hline	

            \textbf{RQ3} & \textit{How do the proposed software solutions improve newcomers' onboarding?} & We intend to deliver empirical evidence of the outcomes achieved by the software solutions to highlight the benefits of using each software solution.  \\ 
		\hline

            \textbf{RQ4} & \textit{What research strategies were employed to assess the software solutions?} & We intend to verify the research strategies most used to assess software solutions for onboarding to guide future evaluation of software solutions development.  \\
		\hline

            \textbf{RQ5} & \textit{How do the software solutions can mitigate newcomers' barriers to joining software projects?} & We intend to comprehend which proposed software solutions mitigated contribution barriers to explore possible research gaps. \\ 
		\hline

            \textbf{RQ6} & \textit{How do the software solutions address diversity and inclusion of newcomers?} & We intend to investigate which diversity and inclusion aspects are explored to make software solutions for onboarding more inclusive. \\ 
		\hline
	\end{tabular}
\end{table*}


==> OLD_Sections/proposal.tex <==

\section{Proposal}
\label{sec:proposal}

%**** bem alto nivel proposta de trabalho do que vai ser feito ate o qualifying
%**** dentre todas essas estrategias eu identifiquei essas aqui de gamification e vou abordar ele por causa disso e disso, vou fazer isso e isso, seguir neste metodo aqui, fazer 2 paginas pra descrever o plano de trabalho
%**** linkar os resultados com a proposta do projeto

\subsection{Problem characterization}

The Open Source Software (OSS) movement has attracted a globally distributed community of volunteers, and the increasing demand for professionals with OSS knowledge has prompted students to contribute to OSS projects~\cite{goduguluri2011kommgame}. By engaging in OSS projects, students gain real-world skills, experiences, and confidence, making them more competitive in the job market~\cite{nascimento2013using, morgan2014lessons}. Additionally, exposing students to OSS projects benefits the OSS communities by increasing the number of potential contributors and fostering collaboration.

To enhance student engagement and motivation in OSS projects, gamification has gained attention. Gamification applies game elements in non-gaming contexts to motivate and engage participants~\cite{deterding2011game}. In the context of OSS, gamification techniques have been successful in incentivizing contributions, fostering healthy competition, and providing a sense of achievement~\cite{sheth2012increasing, bertholdo2016promoting}. By incorporating gaming elements, students remain engaged, persist in their contributions, and derive satisfaction from their involvement. Furthermore, gamification offers opportunities for learning and skill development, as students acquire new technical skills, learn collaboration, and gain insights into project management practices~\cite{pedreira2015gamification, dicheva2015gamification, bartel2016gamifying}.

Overall, the integration of students into OSS projects brings mutual benefits, empowering students with valuable skills and contributing to the growth and sustainability of OSS communities~\cite{goduguluri2011kommgame}. By leveraging gamification techniques, educators and OSS communities can enhance student engagement, motivation, and learning outcomes, fostering a collaborative environment that nurtures the next generation of software developers.

Through our analysis of the primary studies, we have identified a range of technological interventions proposed in the literature to improve the onboarding process for newcomers in software projects. Notably, one strategy that captured our attention is gamification. Gamification involves integrating game mechanics and elements into specific tasks to enhance user engagement, motivation, and performance. This approach has been recognized for its ability to improve developer engagement and outcomes, as highlighted in previous research~\cite{pedreira2015gamification}.

The use of gamification in onboarding interventions for software projects offers several compelling reasons. Gamification can address the challenge of newcomer engagement and motivation, which are crucial for their integration and long-term success in software projects. In addition to motivation and engagement, gamification can contribute to fostering inclusivity in OSS projects by creating a more welcoming and supportive environment for newcomers. This can help mitigate the challenges and barriers they may face, making them feel valued and encouraged to contribute.

Our findings indicate that gamification and environmental redesign interventions offer promising opportunities for enhancing newcomers' onboarding experiences in software projects. There is a growing interest in leveraging gamification techniques (PS04, PS17, PS26) and modifying the OSS environment (PS04, PS17, PS23, PS30) to improve newcomer engagement and motivation. For instance, in PS04, gamification elements such as rankings, quests, points, and levels have been successfully implemented to guide and motivate newcomers. Additionally, the redesign of the OSS environment, incorporating plugins and web portals, aims to address inclusivity issues (PS23), provide assistance and resources (PS17), and offer visual cues for better understanding project architecture and maintenance (PS30). These modifications have the potential to enhance motivation, engagement, and inclusivity among newcomers in OSS projects, thereby creating a welcoming and supportive environment for their integration and growth.

Overall, the use of gamification and environmental redesign interventions in onboarding can enhance newcomer engagement, motivation, and inclusivity in software projects. By leveraging game elements and modifying the project environment, these interventions offer an innovative and effective approach to facilitate the onboarding process and create a positive experience for newcomers.

In this sense, this project intends to build a sandbox environment that mirrors real projects, providing scaffolding, engagement, and incentives for learners. We aim to develop an inclusive tool that enables individuals with different backgrounds to contribute to OSS projects, ultimately enriching their resumes and promoting the sustainability of OSS.

Our proposal will leverage OSS projects as online learning spaces to engage STEM students early in their careers. Through in-depth investigations and the use of game elements, such as quests, the project aims to facilitate the learning of the OSS contribution process and provide scaffolding for individuals with limited knowledge of project structures. By addressing challenges associated with creating a learning environment, the project aims to contribute novel approaches to teaching contribution procedures and provide hands-on experience in real software engineering projects. Successful participation in OSS projects not only benefits students in terms of visibility, career prospects, and societal impact but also supports the adoption and improvement of widely used software projects.


\subsection{Goals}

Overall, our investigation will involve analyzing the feasibility of gamification elements and designing a sandbox environment, considering inclusivity through an intersectional lens, and evaluating the effectiveness of our approach in engaging newcomers to contribute to real OSS projects.


\subsection{Research activities}

The planned activities for this PhD project are organized into the following steps to achieve the project's goal:

\begin{enumerate}
    \item \textbf{Comprehensive exploration of the research area:} In this step, we conducted a systematic literature review to thoroughly investigate the existing body of knowledge regarding technological interventions for onboarding in software projects. The review aimed to identify, gather, and analyze primary studies that focused on onboarding interventions in order to provide valuable insights and inform our research. This step has been successfully completed, providing a solid foundation for the subsequent phases of the project.

    \item \textbf{Design learning environment:} Our goal is to understand how to create a scaffolded learning environment to help novice students participate in an OSS project and learn the underlying OSS processes, environments, and conventions.

    \item \textbf{Define research thrusts:} In this proposal, we will focus on the following research thrusts:

        \textbf{ - Research thrust 1:} Investigate the feasibility of incorporating gamification elements, such as quests, and a sandbox environment to support the learning of the OSS contribution process. This thrust aims to determine which gamification elements can effectively teach the OSS contribution model and how to create an inclusive and safe learning environment. 

        \textbf{ - Research thrust 2:} Perform investigations through an intersectional lens to evaluate the implications of our tools and OSS projects for minorities in programming novices' learning. This thrust aims to assess how our tools and the OSS context impact inclusivity. 

    \item \textbf{Address research questions:} Based on the previous research thrusts we will answer the following research questions:

        \textbf{ - RQ1:} How can novices in programming learn the contribution process of an OSS project through quests?

        \textbf{ - RQ2:} How can we design a tool that promotes inclusivity in supporting novices' learning in the context of OSS?

        \textbf{ - RQ3:} How effective is our approach in engaging novices to start contributing to a real OSS project?

    \item \textbf{Evaluation of the proposed approach:} We will conduct our investigation iteratively by collecting data, designing tools, and assessing them through formative and summative evaluations. This iterative approach allows us to refine our tools based on user feedback and improve their effectiveness.
\end{enumerate}

\subsection{Research schedule}

This section provides a description of the key activities that form the core of this PhD research project. Each activity is outlined below, we aim to provide a clear roadmap for the successful execution of the project and ensure its alignment with the research goals.

\begin{enumerate}
    \item \textbf{Completion of graduate program disciplines:} As a mandatory requirement for credit acquisition within the SICCs Graduate Program, the candidate diligently attended the prescribed disciplines. Adhering to the program's regulations, the accumulation of credits is required to take place during the initial year of the PhD degree program. By fulfilling this requirement, the candidate ensures compliance with the program's guidelines and demonstrates their commitment to academic progression within the designated timeframe.

    \textbf{ - Period:} Fall 2021 - Fall 2023.

    \item \textbf{Systematic literature review of onboarding technological interventions:} In this stage, a comprehensive SLR will be undertaken to examine the proposed onboarding technological interventions in the literature. The primary focus is to identify interventions that facilitate the onboarding process for newcomers in OSS projects. By meticulously analyzing the literature, this review aims to gather valuable insights into the approaches and interventions employed to assist newcomers during their transition into OSS projects. The findings will contribute to the existing body of knowledge on onboarding interventions and provide valuable guidance for practitioners and researchers seeking effective ways to support newcomers in the OSS community.

    \textbf{ - Period:} Fall 2022 - Summer 2023.

    \item \textbf{Writing and defending the comprehensive exam:} According the regulations of the SICCs graduate program, it is mandatory for every PhD student to successfully complete a comprehensive examination. This examination is typically conducted within 24 months from the commencement of the course. The student will undertake the task of writing a monograph based on their research findings, which will serve as the foundation for the comprehensive exam. The monograph will encompass an in-depth literature review describing: methodology, results, and discussions. The student will then defend their monograph before a panel of examiners, showcasing their knowledge, expertise, and contribution to the field of study. Successful completion of the comprehensive exam signifies the student's readiness to proceed with their doctoral research and signifies a significant milestone in their academic journey.

    \textbf{ - Period:} Spring 2023 - Summer 2023.

    
    \item \textbf{Proposal and implementation of an OSS learning environment:} In this crucial phase, we will focus on the design and implementation of an innovative OSS learning environment. Our primary objective is to create a sandbox environment that accurately mirrors a real-world project, providing learners with a practical platform to develop their skills and understanding of OSS practices. To support effective learning, we will incorporate various mechanisms that offer scaffolding and guidance throughout the learning process. Additionally, we will introduce gamification engaging elements and incentives to enhance learner motivation and participation.

    \textbf{ - Period:} Fall 2023 - Spring 2024.

    \item \textbf{Definition of the empirical study:} This critical phase involves comprehensive planning for the empirical study, where the candidate will establish all necessary parameters to conduct the research. The primary focus will be on defining clear objectives, formulating hypotheses, and identifying dependent and independent variables, among other essential factors crucial for the experiment's success. By dedicating attention to the definition of the empirical study, the candidate aims to establish a robust and well-structured research plan. This planning phase will provide a solid foundation for conducting the study, enabling accurate data collection, analysis, and ultimately contributing to the advancement of knowledge in the chosen research area.

    \textbf{ - Period:} Summer 2024.

    \item \textbf{Preparation and execution of the empirical study:} During this pivotal phase, meticulous preparation and execution of the empirical study will take place. The primary focus will be on setting up the experimental environment, ensuring the availability of all necessary resources and tools.

    \textbf{ - Period:} Fall 2024 - Spring 2025.

    \item \textbf{Elaboration of reports and scientific articles:} As a crucial step in the research process, the candidate will undertake the task of preparing comprehensive reports based on the partial and final results of the study. Furthermore, the candidate will also focus on disseminating the research outcomes to the wider scientific community. To achieve this, scientific articles will be written and prepared for submission to reputable events and journals within the research area.

    \textbf{ - Period:} Fall 2024 - Spring 2025.

    \item \textbf{Writing and defense of the PhD dissertation:} In this phase, the candidate will embark on the task of meticulously crafting the PhD dissertation, which will encapsulate and present the culmination of the research conducted in the previous stages. The dissertation will serve as a comprehensive document, showcasing the results, insights, and contributions derived from the SLR, as well as the foundational principles that underpin the research.

    \textbf{ - Period:} Spring 2025 (April).
    
\end{enumerate}

\subsection{Expected results}

The conduction of this PhD project is expected to yield significant contributions and results in several key areas:

\begin{enumerate}
    \item Introduces and engage students to contribute in real software development processes;

    \item Enhances newcomers learning experience, participation in projects, and resume enrichment;
    
    \item Prepares a future workforce of contributors;

    \item Contributes to the state-of-the-art in learning the OSS contribution process;

    \item Reduces barriers and provides appropriate tools for fostering learning;
    
    \item Increases participation in projects and generates interest in software engineering;

    \item Empowers new contributors to OSS projects;

    \item Enhances diversity in contributions;

    \item Positively impacts society by leveraging the potential of a broader range of contributors.
\end{enumerate}

==> Protocol/protocol-Example.tex <==
%%%SLR protocol
%This document is based on ``Kitchenham, B. SEGRESS: Software Engineering Guidelines for REporting Secondary Studies. IEEE Transactions on Software Engineering, Vol. 49, NO. 3, March 2023.''

%Title -- The title should identify the article's objective and specify whether the article is. Examples:
%...: A Systematic Review
%...: A Systematic Literature Review
%...: A Systematic Mapping Study 
%...: A Metaanalysis
\textbf{...: A Systematic Literature Review}

%######################################
%Description of the rationale for the review in the context of existing knowledge (the current state of knowledge and its uncertainties).
%Why is it essential to perform the review?
%What the findings from the review might add to existing knowledge?
\vspace{0.1cm}
\textbf{1. Introduction} 

%-----------------------------
\textbf{1.1 Rationale} 

Given the importance of knowing ..., we will conduct a Systematic Literature Review (SLR) to ...

%-----------------------------
\textbf{1.2 Objectives} 

The aim of this SLR is to ...

To determine ... our research questions (RQs) are:

\begin{itemize}
    \item [] \textbf{(RQ1)} -- \textit{``What evidence is there that ...?''}
    \item [] \textbf{(RQ2)} -- \textit{``...?''}  
    \item [] \textbf{(RQx)} -- \textit{``...?''}  
\end{itemize}

We considered our RQx suitable for investigation by SLR because ... 
Initial research shows ... in the area of ... Our work relates more closely to the ...
However, before answering our RQx we need to know the ... This is because we need to understand ... in terms of ...

%######################################
\vspace{0.1cm}
\textbf{2. Methods}

%-----------------------------
\textbf{2.1 Eligibility Criteria}

This SLR aims to identify and classify papers related to ... in the context of ..., including papers related to ... The inclusion criteria (IC) are, therefore:

\begin{enumerate}
    \item (\textbf{IC1}) -- The study's main objective may be ... or to discuss or investigate the ....
    \item (\textbf{IC2}) -- Studies discussing how ...
    \item (\textbf{IC3}) -- The study must have a ... context.
    \item (\textbf{IC4}) -- The study must be published in English.
    \item (\textbf{ICx}) -- ...
\end{enumerate}
    
%Note that different papers related to the same study will be kept in the selected papers but identified as linked.

The exclusion criteria (EC) are:

\begin{enumerate}
    \item (\textbf{EC1}) -- Papers whose main objective is to ... Thus, we exclude papers that comment on ... 
    \item (\textbf{EC2}) -- Methodological papers with general (i.e. non-...) context.
    \item (\textbf{EC3}) -- Papers for which only PowerPoint presentations or extended
abstracts are available.
    \item (\textbf{ECx}) -- Papers that describe ...
    \item (\textbf{ECx}) -- Papers reporting studies that ...
    \item (\textbf{ECx}) -- Papers discussing ...
\end{enumerate}

%-----------------------------
\textbf{2.2 Information Sources}
%Specification of all databases, registers, websites, organizations, reference lists, and other sources searched or consulted to identify studies together with the date each source was last searched or consulted.

To address our RQs, we needed to identify papers that reported the ..., and were published in high-quality journals. To achieve our search process strategy, we decided to limit our search to the following x journals:

\begin{enumerate}
    \item (\textbf{Source 1}) -- ... http://www
    \item (\textbf{Source 2}) -- ... http://www
    \item (\textbf{Source x}) -- ... http://www
\end{enumerate}    

We restricted ourselves to these journals because they all publish papers on ... and have relatively high impact factors (among ... journals). These are, therefore, highly respected journals, and we should expect the quality of the papers they publish to be correspondingly high.

%-----------------------------
\textbf{2.3 Search Strategy}
%Presenting full search strategy, including, as appropriate, electronic search strings, snowballing, manual search, finding unpublished materials, etc
%Explaining how the search string(s) were developed linking the explanation to the SR goals and eligibility criteria as necessary.
%Reporting any search filters used for specific databases.
%Explaining how the search strings were validated
%Reporting the full search string used for each digital library, platform

As represented in Figure \ref{fig:search}, we will adopt a search strategy as a x-stage process defined as:

%We will conduct a x-stage search, as shown in Figure \ref{fig:search}, to identify the current literature on ...

\begin{enumerate}
    \item \textbf{Stage 1} -- First, during Stage 1, we will create our search string, presented in Table \ref{tab:searchStringFinal}. It will be applied in \textit{...., ..., ... and ...}, the most commonly used electronic databases in Computer Science \cite{Maplesden15}. Inclusion and Exclusion criteria will be applied as defined in \ref{sub:selection} to define our initial set of studies (SetA).         
    \item \textbf{Stage 2} -- With an objective to expand our set of studies, during Stage 2, we will use the studies selected for inclusion in Stage 1 as our seed set (start set) for performing iterations in snowballing, where each iteration will contain forward and backward snowballing. The citations (forward snowballing) will be extracted with the help of \textit{Google Scholar}.     
    In the first interaction of backward snowballing, the references of the studies of the start set will be screened to identify more papers to include in the SLR. The papers citing the included studies as the start set will be evaluated in forward snowballing. The new papers identified go into the second iteration, and so on, to compose Set B. 
\end{enumerate}

The final list of included studies will be formed by combining the findings of the two stages (Stage 1: Set A + Stage 2: Set B).

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=18cm]{Protocol/images/search.png}
    \caption{Search Strategy}
    \label{fig:search}
\end{figure*}

%Search process documentation
We will use the ``export'' feature available in the electronic database (i.e., title, author(s), abstract, keywords, year of publication, and the name of the data source) to export bibliometric data. In addition, all candidate papers will be stored using the ... x.x software. 

%The concept of population, intervention, and outcomes is not well-suited to the Software Engineering area

%The following details of the population, intervention, and outcomes of relevance to the SLR will form the basis for the construction of suitable search terms.
%\begin{itemize}
    %\item [] \textbf{(Population)} -- ...
    %\item [] \textbf{(Intervention)} -- ...
    %\item [] \textbf{(Outcomes of relevance)} -- ...
%\end{itemize}

%The detailed strategy for developing search strings are:

%\begin{enumerate}
    %\item Derive major terms from the RQs by identifying the population, intervention and outcome.
    %\item Identify alternative spellings and synonyms for major terms.
    %\item Check the keywords in any relevant papers we already have.
    %\item When database allows, use the Boolean OR to incorporate alternative spellings and synonyms.
    %\item When database allows, use the Boolean AND to link the major terms from population, intervention and outcome.
%\end{enumerate} 

The detailed strategy for developing search strings are:

\begin{enumerate}
    \item Derive major terms from the SLR topic area (Table \ref{tab:searchString}).
    \item Identify alternative spellings and synonyms for major terms (Table \ref{tab:searchString}).    
    \item When databases allow, use the Boolean \textbf{OR} to incorporate alternative spellings and synonyms (Table \ref{tab:searchStringBoolean} -- Line 3).
    \item When databases allow, use the Boolean \textbf{AND} to link the major terms (Table \ref{tab:searchStringFinal}).
\end{enumerate} 

\begin{table*}[!ht]
\centering
\caption{Search String}
\label{tab:searchString}
\begin{tabular}{p{8.5cm}|p{8.5cm}}
\hline

{\textbf{Major terms}} & {\textbf{Alternative spellings and synonyms}} \\ \hline

\multirow{3}{*}{\textbf{... ... ... ... ... ... ... ... ... ...}} & ... ... ... ... ... ... ... ... ...\\
 & ... ... ... ... ... ... ... ... ...\\
 & ... ... ... ... ... ... ... ... ...\\ \hline

\multirow{3}{*}{\textbf{... ... ... ... ... ... ... ... ... ...}} & ... ... ... ... \\
& ... ... ... ... ... ... ... ... ...\\
 & ... ... ... ... ... ... ... ... ...\\ \hline

\end{tabular}
\end{table*}

\begin{table*}[!ht]
\centering
\caption{Search String -- Boolean}
\label{tab:searchStringBoolean}
\begin{tabular}{p{9.5cm}|p{7.5cm}}
\hline

\multirow{3}{*}{\textbf{Boolean OR to incorporate alternative spellings and synonyms}} & ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \\
& ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \\
& ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \\ \hline

\end{tabular}
\end{table*}

\begin{table*}[!ht]
\centering
\caption{Final Search String}
\label{tab:searchStringFinal}
\begin{tabular}{l}
\hline

(... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ...) \textbf{AND} (... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ... \textbf{OR} ...) \\ \hline

\end{tabular}
\end{table*}

%-----------------------------
\textbf{2.4 Selection Process}\label{sub:selection}
%Stating the process for selecting studies, including the specific phases of the selection process, the number of assessors per study, methods of handling disagreements, any tools used, and any methods of assessing agreement rates.

As represented in Figure \ref{fig:selection}, we will adopt a selection process as a x-stage process defined as:

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=18cm]{Protocol/images/search.png}
    \caption{Selection Process}
    \label{fig:selection}
\end{figure*}

\begin{enumerate}
    \item \textbf{Stage 1} -- The initial selection will be based on reviewing each article’s title, abstract, and keywords.
    %\item \textbf{Stage 1} -- ... %Identify candidate studies by searching ... Exclude studies on the basis of titles and Abstracts.
    \item \textbf{Stage 2} --  Final inclusion/exclusions will be based on the x reviewers independently assigning the full papers. 
    %\item \textbf{Stage 2} -- ... %Obtain full text of studies and critically appraise them, excluding ...     
\end{enumerate}

xxx reviewers (one expert in ..., one in ..., and ) will screen all the potential papers independently. Meetings will be performed to solve conflicts. 

%We will consider conducting the bibliometric data extraction (e.g., title, abstract, authors, year, source, among others) while deciding whether the paper should be included.

%-----------------------------
\textbf{2.5 Data Collection Process}
%Describing how many reviewers collected data from each report, whether multiple reviewers worked independently or not, and any process used to resolve disagreements.
%Describing software tool that was used to support data collection.

All included studies will go into data extraction, which will be conducted in accordance with the RQs posed in our SLR.

The studies will be proportionally assigned to xx researchers, x (x) acting as extractors and x (x) as reviewers. Therefore, all researchers will be responsible for extracting and verifying the data, besides completing the data extraction form, as shown in Table \ref{tab:dataExtractoin} 

\begin{table*}[!ht]
\centering
\caption{Data Extraction Form}
\label{tab:dataExtractoin}
\begin{tabular}{p{5cm}|p{12cm}}
\hline

{\textbf{Data Item}} & {\textbf{Value}} \\ \hline
\textbf{Study ID} & A unique identifier in the format: $<$number$>$ \\ \hline
\textbf{Title} & Study’s title: $<$string$>$ \\ \hline
\textbf{Year} & Year of study publication: $<$number$>$ \\ \hline
\textbf{Reference type} & Journal/Conference $<$one of the listed options$>$: $<$string$>$ \\ \hline
\textbf{Journal/conference name} & Journal/conference’s name: $<$string$>$\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... $<$...$>$ \\ \hline

\multicolumn{2}{l}{\textbf{RQ1}} \\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline

\multicolumn{2}{l}{\textbf{RQ2}} \\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline
\textbf{.... .... .... ... ... ... ... ...} & .... .... .... ... ... ... ... ... .... .... .... ... ... ...  .... .... .... ... ... ... ... ... .... .... .... ... ... ...\\ \hline

\end{tabular}
\end{table*}

%-----------------------------
\textbf{2.6 Study Risk of Bias Assessment}
%The goal is to assess the risk of methodological bias for each primary study (primary study risk of bias (RoB)). However, RoB is optional for mapping studies.
%The aim is to have an overall assessment of risk of bias for each domain and the primary study. One approach is to assess each domain regarding the options: Very Low RoB, Low RoB, Moderate RoB, High RoB, No Information.

We will use the following questions to assess the risk of bias (RoB) in our studies: 

\begin{enumerate}
    \item ... Yes (Low RoB), Probably Yes (Moderate RoB), No (High RoB).
    \item ... No (Low RoB), Yes (High RoB).
    %Examples \cite{Dyba08}
    %\item Is the study based on research (or merely a ``lessons learned'' report based on expert opinion)? No (Low RoB), Yes (High RoB).
    %\item Is there a clear statement of the aims of the research? No (Low RoB), Yes (High RoB).
    %\item Is there an adequate description of the context in which the research was carried out? No (Low RoB), Yes (High RoB).
    %\item Was the research design appropriate to address the aims of the research? No (Low RoB), Yes (High RoB).
    %\item Was the recruitment strategy appropriate to the aims of the research? No (Low RoB), Yes (High RoB).
    %\item Was the data collected in a way that addressed the research issue? No (Low RoB), Yes (High RoB).
    %\item Was the data analysis sufficiently rigorous? No (Low RoB), Yes (High RoB).
    %\item Has the relationship between researchers and participants been adequately considered? No (Low RoB), Yes (High RoB).
    %\item Is there a clear statement of findings? No (Low RoB), Yes (High RoB).
    %\item Is the study of value for research or practice? No (Low RoB), Yes (High RoB).
\end{enumerate}

The questions (x--x) relating to the validity of the ... used by each study will be used to assess the risk of study bias. Other questions (x--xx) will help assess the ...

The first x questions are ``screening questions''. If the answer to those questions is ``No'' it is not worth continuing with the other questions. 

X two of the X authors will be assigned to extract the criteria at random. We will perform our assessments independently and discuss disagreements until we reach an agreement.

%-----------------------------
%%%%%Effect Measures - if applicable (quantitative studies)

%-----------------------------
\textbf{2.7 Analysis and Synthesis of Bias Assessment}

Regarding analysis and synthesis methods issues, we will split our included studies into subsets that address similar issues. Studies that address ... will be separated from studies that address ... 

%General
Since we investigate outcome patterns in the data, we will adopt 
presentation of study results using tabulation and visual representations.

%For quantitative studies
%Forest plots will be used to summarise the effect sizes and their variance for each study and the overall summary effect size from ...
%We will summarize the outcome data along with studies characteristics in Tables with primary studies grouped according to whether the effect sizes are positive, inconclusive, or negative. 

%For mapping/qualitative studies
The main results will be presented as the categories assigned to the studies. The categories will be displayed as tables of categories and their values for each study. In addition, we will display the outcome data as conceptual models comprising bubbles linked by lines, where the bubble names will identify concepts, and the lines will represent the relationships among the concepts. 

We will synthesize the data by identifying themes from the findings reported in each accepted study. These identified themes will
gave us the categories reported in our results section.

%-----------------------------
\textbf{2.8 Reporting of Bias Assessment}

To assess the reliability of the search and selection processes, we will ...

The process used to construct and refine our search string is described in ... to guarantee the transparency of our search process. It is also worth mentioning that our search string was generated considering terms ... 

We will describe all the limitations placed in the search process. Moreover, we will adopt two methods to search relevant literature, one based on search strings and the other on references and citations.

Similarly, aiming at the transparency of our selection process, X or more researchers will be assessing each candidate study ... In addition, x researcher(s) will check ... Finally, ... will be used as an indication of missing data or missing studies.

%-----------------------------
\textbf{2.9 Certainty Assessment}

In addition to the previously mentioned criteria, Study Risk of Bias, and Analysis and Synthesis of Bias Assessment, we will assess our body of evidence's Relevance, Coherence, and Adequacy. 

For Relevance, we will assess whether data is (or not) well described or define concepts in different ways. Additionally, we will analyze plausible alternative descriptions, interpretations, or explanations that could be used to synthesize the data.

For Coherence, we will verify the extent to which data from the individual studies are consistent with or contradict the finding being assessed. 

For Data Adequacy, two issues will be considered: whether there were possible missing studies and significant gaps in the data obtained from the studies. We will check the number of studies from which each finding originated, such as information about the context of each study, including, ...

==> Tables/references_primary_studies.tex <==
\begin{table*}[!btb]
\centering
%\scriptsize
\caption{References of the Primary Studies (PS)}
\label{tab:appendix}

\begin{tabularx}{\textwidth}{XX|XX|XX|XX}
\toprule
\textbf{ID} & \textbf{Reference} & \textbf{ID} & \textbf{Reference} & \textbf{ID} & \textbf{Reference} & \textbf{ID} & \textbf{Reference}\\
\hline \hline

PS1 & \cite{PS01azanza2021onboarding} & 
PS11 & \cite{PS11nagel2021ontology} & 
PS21 & \cite{PS21ford2022reboc} & 
PS31 & \cite{PS31sun2018personalized} \\


PS2 & \cite{PS02canfora2012going} & 
PS12 & \cite{PS12sarma2016training} & 
PS22 & \cite{PS22liu2018recommending} & 
PS32 & \cite{PS32sarma2009tesseract} \\


PS3 & \cite{PS03cubranic2003hipikat} & 
PS13 & \cite{PS13serrano2022find} & 
PS23 & \cite{PS23santos2023designing} & \\


PS4 & \cite{PS04diniz2017using} & 
PS14 & \cite{PS14stanik2018simple} & 
PS24 & \cite{PS24santos2021can} & \\


PS5 & \cite{PS05dominic2020conversational} & 
PS15 & \cite{PS15steinmacher2016overcoming} & 
PS25 & \cite{PS25minto2007recommending} & \\


PS6 & \cite{PS06fu2017expert} & 
PS16 & \cite{PS16steinmacher2012recommending} & 
PS26 & \cite{PS26heimburger2020gamifying} & \\


PS7 & \cite{PS07guizani2022attracting} & 
PS17 & \cite{PS17toscani2018gamification} & 
PS27 & \cite{PS27malheiros2012source} &  \\


PS8 & \cite{PS08he2022gfi} & 
PS18 & \cite{PS18wang2011bug} & 
PS28 & \cite{PS28yang2016repolike} & \\



PS9 & \cite{PS09kagdi2008can} & 
PS19 & \cite{PS19xiao2022recommending} & 
PS29 & \cite{PS29zhou2021ghtrec} & \\


PS10 & \cite{PS10medeiros2022assisting} & 
PS20 & \cite{PS20yin2021automatic} & 
PS30 & \cite{PS30venigalla2022gitq} & \\ \hline

\bottomrule

\end{tabularx}
\end{table*}
